Astrochemical modelling of infrared dark clouds

Infrared dark clouds (IRDCs) are cold, dense regions of the interstellar medium (ISM) that are likely to represent the initial conditions for massive star formation. It is thus important to study the physical and chemical conditions of IRDCs to provide constraints and inputs for theoretical models of these processes. We aim to determine the astrochemical conditions, especially cosmic ray ionisation rate (CRIR) and chemical age, in different regions of the massive IRDC G28.37+00.07 by comparing observed abundances of multiple molecules and molecular ions with the predictions of astrochemical models. We have computed a series of single-zone astrochemical models with a gas-grain network that systematically explores the parameter space of density, temperature, CRIR, and visual extinction. We have also investigated the effects of choices of CO ice binding energy and temperatures achieved in transient heating of grains when struck by cosmic rays. We selected 10 positions across the IRDC that are known to have a variety of star formation activity. We utilised mid-infrared (MIR) extinction maps and sub-mm emission maps to measure the mass surface densities of these regions, needed for abundance and volume density estimates. The sub-mm emission maps were also used to measure temperatures. We then used IRAM-30m observations of various tracers to estimate column densities and thus abundances. Using estimates of the abundances of CO, HCO$^+$ and N$_2$H$^+$ we find consistency with astrochemical models that have relatively low CRIRs of $\zeta \sim10^{-18}$ to $\sim10^{-17}\:{\rm s}^{-1}$, with no evidence for systematic variation with the level of star formation activity. Astrochemical ages are found to be < 1 Myr. We discuss potential sources of systematic uncertainties in these results and the overall implications for IRDC evolutionary history and astrochemical models.(abridged for arXiv)

==> chapters/Conclusion.tex <==
\section{Conclusion}\label{final}

In this work we have used the astrochemical model provided by \cite{2015A&A...582A..88W} to predict the evolution of molecular abundances with respect o Hydrogen nuclei, as a function of H nuclei density, temperature, visual extinction and CRIR, while the initial abundances of species has been defined before. Hence, we compared the grid of obtained models with molecular abundance estimated by using IRAM30m data, previously obtained toward the IRDC G28.\\


comparison has been performed using different methods and progressively increasing the number of molecular species. Below, we summarise the obtained results:

1) We have compared model predictions and observations by following method: \textit{Restricted}. IN this method we restricted the parameters in a way that the the models cover n(H) being in the range 1.0e4-1.0e6 cm$^{-3}$, T in 5-50 K and A$_v$ in 5-100 mag. We have applied the mentioned method to the abundances of narrow velocity (N) range, HCO$^+$ obtained from HC$^{18}$O$^+$ (18) and N$_2$H$^+$. Applying mentioned method constrain $\zeta$ associated with $\chi^2$<3 to be 1.0e-19-2.2e-19 s$^{-1}$ at p8, 1.0e-19-4.6e-19 s$^{-1}$ at p2,p3,p4,p10, 2.2e-19-1.0e-18 s$^{-1}$ at p7, 4.6e-19-2.2e-18 s$^{-1}$ at p9, 1.0e-18-1.0e-17 s$^{-1}$ at p5, 2.2e-18-2.2e-17 s$^{-1}$ at p1, and the highest range 4.6e-16-2.2e-15 s$^{-1}$ at p6. The age of the clouded has been estimated older than 1.0e6 years at p2,p3,p4,p6,p8,p10 and younger than 1.0e6 years for the remaining positions. At p1, the age has been estimated even younger $\sim$ 8e4 years.\\

2) We have performed fitting in restricted region using ratio abundances of HCO$^+$ and N$_2$H$^+$ with respect to CO. Estimated range of $\zeta$ with this method is broader than the \textit{Restricted} fitting method.

3) We continued to find the best models using abundances of positive charges (\textit{ions} fitting method), CO together with HCO$^+$ and CO together with N$_2$H$^+$. 



4) Hence, we have progressively increased the number of species. We added C-bearing species including CH$_3$OH and H$_2$CO. Even though the high values of $\chi^2$ ($\sim$ >10) indicates that the models fail to reproduce the real data at all positions, still it can be seen a solution at later time, after 1 Myrs. Considering the possibility that CH$_3$OH is thick, we removed it from C-bearing species to reduced the uncertainty. The fitted models have been obtained with better $\chi^2$. Then we repeated the same method by adding N-bearing species and all species with and without CH$_3$OH as well, for which the best fitting gives $\chi^2$>14.\\


We have considered all uncertainties in the calculation of physical parameters of the positions and further restricted the range of parameters to search through the models to find the best one. We have noted that CO might be overestimated and thus selected a narrow velocity range based on the N$_2$H$^+$ transition line to obtain abundances of species. Also, assuming that H$^{13}$CO$^+$ could be optically thick, we obtained HCO$^+$ from HC$^{18}$O$^+$. The final CRIR distribution shows relatively low CRIR for all positions. We can conclude that in general accepted range for $\zeta$ for $\chi$<3 at quiescent positions p7,p8,p9,p10 and three of active star forming regions p2,p3,p4 (approximately 1.0e-19-1.0e-18 s$^{-1}$), is lower than that obtained at active star forming regions i.e. p1,p5 which is approximately 1.0e-18-1.0e-17 s$^{-1}$. Estimated age of the Cloud varies from position to position and it does not show a similar pattern between regions. Future observations and obtaining more accurate abundances of CO without environmental contamination and detecting more ionized molecular transitions, may lead to find better estimation of CRIRs.

 




==> chapters/main_file.tex <==
\section{Introduction}

%The relatively well known scenario, collapsing dense core under its own gravity and accretion by the surrounded material \citep{1969MNRAS.145..271L,2018IAUS..332..249T,1987ARA&A..25...23S,leblanc2011introduction,2012A&A...537A.122K}, that leads to the formation of low-mass stars (M<8M$_{\odot}$), fails to predict the birth of more massive stars, whose formation mechanism remains under debate \citep{2014prpl.conf..149T}. Despite the key role that high-mass stars (M>8M$_{\odot}$) play in regulating the energy content and interstellar medium and evolution of galaxies, it has not been identified yet a mechanism that allows to gather together the large amount of material necessary to form massive stars, in the relatively short time-scale \citep{kennicutt2005role,motte2018high}. \\

%In addition to the theoretical difficulties, high-mass stars pose observational challenges as well. Their large distances (>few kpc), strong stellar feedback, crowded environments (massive stars are usually born in clusters) and relatively short evolutionary time-scales \citep{2018ARA&A..56...41M}, make the direct observations of forming massive stars challenging. Hence, a parallel theoretical and observational approach has been undertaken and it is to study the regions in which massive stars are seen to form \citep{2006ApJ...641..389R}. These regions are known as Infrared Dark Clouds (IRDCs).\\

Infrared Dark Clouds (IRDCs) are cold ($T<25\:$K) \citep[e.g.,][]{2006A&A...450..569P,peretto2010mapping,lim2016distribution}
%,2020ApJ...897..136M} 
and dense ($n_{\rm H} \gtrsim 10^3\:{\rm cm}^{-3}$) 
\citep[e.g.,][]{2013A&A...549A..53K,lim2016distribution}
%\citep{2014prpl.conf..149T} 
regions of the Interstellar Medium (ISM) %\citep{2009Ap&SS.324..155R,2013MNRAS.428.3425H} 
that have the potential to host the formation of massive stars and star clusters \citep[for a review, see, e.g.,][]{2014prpl.conf..149T}.
%\citep{hernandez2012virialized,2012MNRAS.423.2342F}. Indeed, IRDCs shows H column densities similar to those regions in which massive stars are known to be formed and host cold cores i.e., the earliest phase in massive star formation. 
Thus, it is essential to study the physical and chemical properties of IRDCs to understand the initial conditions for the formation of these massive stellar systems.
%\citep{2009Ap&SS.324..155R}.

%Based on the studies focused on inferring physical conditions of temperature and density toward massive cores, these cores located within IRDCs can host different evolutionary stages of massive star formation, so that the cold and massive quiescent region may be the best candidate for pre-prorostellar phase, an earlier stage of massive star formation \citep{2011ApJ...741..120R,2010ApJ...715..310R}. Hence, studying both active and quiescent regions in IRDCs, can reveal the initial conditions for massive stars to be born.

%The physical properties of IRDCs i.e. temperature \citep{peretto2010mapping,lim2016distribution}, volume density of Hydrogen \citep{2013A&A...549A..53K} and visual extinction have been studied so far \citep{lim2016distribution}. 

Regarding astrochemical studies of IRDCs, the CO depletion factor ($f_{\rm D,CO}$), i.e., the ratio of the CO abundance if all C was present as gas phase CO compared to the actual abundance, has been measured to be $\sim 3$ on parsec scales in a filamentary IRDC by \cite{hernandez2012virialized}. High CO depletion factors are generally expected in cold conditions, i.e., when $T\lesssim 20\:$K. Widespread enhanced deuteration of $\rm N_2H^+$, which is expected in cold, dense conditions where CO is depleted from the gas phase, has been seen in another filamentary IRDC by \cite{barnes2016widespread}. More localised, highly deuterated regions have been reported in the massive IRDC G28.36+00.07 by \cite{kong2016deuterium}.

%CO depletion factor, the Deuterium fractionation \citep{2015ApJ...804...98K} and consequently Ionization fraction X(e)=$\frac{\rm n(e)}{\rm n(H_2)}$ \citep{2002P&SS...50.1133C}, may be another parameters leading to obtain information about the age and the evolution of IRDCs. The studies by \cite{1999ApJ...523L.165C} and \cite{ceccarelli2014deuterium} shows a very high degree of CO ($\sim 10$) depletion factor and deuteration as well, at a dense region of IRDCs where the formation of massive stars begins.\\

%Another study by \cite{2003A&A...403L..37C} indicates that at the earliest stage prior to the formation of protostellar core, the major molecular ion dominating the chemistry evolution is H$_2$D$^+$ (the deuterated forms of the main ion H$_3$ $^+$). On the other side, the formation of ions are produced by Cosmic rays (CRs) and the molecules in ISM are formed mainly by ion-molecule gas phase reactions \citep{2002P&SS...50.1133C}.\\

Much of interstellar chemistry is driven by cosmic ray (CR) ionization, and the cosmic ray ionization rate (CRIR), $\zeta$, (defined as the rate of ionizations per H nucleus) is an important parameter of astrochemical models. Examples of inferred values of CRIR include the study of the $\rm H^{13}CO^+$ emission and $\rm H_3^+$ absorption towards seven massive protostellar cores by \cite{2000A&A...358L..79V}, who estimated $\zeta \sim (2.6\pm 1.8) \times 10^{-17}\:{\rm s}^{-1}$. More recent studies of hot cores with more sophisticated chemical networks include the work of Barger \& Garrod (2020), who derived more elevated levels of CRIRs.
%jct - we need to give some more quantitative info here; and make sure definition of \zeta is the same.
Studies of the diffuse ISM have found values of $\zeta\simeq 2\times 10^{-16}\:{\rm s}^{-1}$ \citep[e.g.,][]{neufeld2017cosmic}. In regions of active star formation, such as OMC-2 FIR 4, much higher values of CRIR, 
$\gtrsim 10^{-15}\:{\rm s}^{-1}$, 
%jct - we should check this number
have been reported \citep{ceccarelli2014herschel, fontani2017seeds,favre2018solis}, which may be explained by local production in protostellar accretion and/or outflow shocks \citep{padovani2016protostars, gaches2018exploration}.
Another region where the CRIR is inferred to be very high is the Galactic Centre, with values of $\zeta\gtrsim10^{-15}\:{\rm s}^{-1}$ \citep{carlson2016cosmic}.
%Carlson et al. 2016, PRD, 94, 3504

Lower energy CRs, which dominate the CRIR, are expected to be absorbed by high column densities of gas and more easily shielded by magnetic fields, whose strength increases in denser regions \citep{crutcher2012magnetic}. Thus, it is possible that the CRIR in IRDCs may be smaller than that of the diffuse ISM in which they reside. To date, there have been relatively few studies of the CRIR in IRDCs. 

IRDCs have the advantage of being probed by mid-infrared (MIR) extinction (MIREX) mapping methods \citep[e.g.,][]{butler2012mid, 2013A&A...549A..53K}, which yield measurements of cloud mass surface density, $\Sigma$. {\it Herschel} sub-mm emission maps also constrain $\Sigma$ and additionally provide a measure of the dust temperature, although careful subtraction of contributions from the diffuse Galactic plane are important \citep{lim2016distribution}. IRDCs are expected to be at a relatively early evolutionary stage, which may simplify their modeling. However, studies with ALMA and {\it Herschel} do indicate that active star formation can be proceeding even in MIR-dark regions of the clouds  \citep[e.g.,][]{tan2014kinematics, 2018ApJ...867...94K, moser2020high}.

%(e.g., Tan et al. 2016; Kong et al. 2019; Moser et al. 2020).

%Bron et al.???

%CRs can penetrate through the cloud and start a chain of reactions producing tracers such as HCO$^+$ and N$_2$H$^+$.
%Even though the formation of atomic ions (i.e C$^+$, Mg$^+$) by CRs is like list, it is difficult to measure atomic abundances directly and hence the studies carries on by molecular abundances \citep{caselli1998ionization}. In the recent study reported by \cite{2020arXiv200713593B}, using an astro-chemical model has led to predict the best observable tracers of ionization fraction rather than DCO$^+$/HCO$^+$, in both translucent and dense regions of ISM.\\


%Since CRs are counted as the main source of ionization, constraining cosmic ray ionization rate (CRIR),denoted $\zeta$ (the total number of
%H$_2$ ionization per molecule, per sec) can lead us to better understanding of the initial phases of massive star formation. The results obtained by \cite{2002P&SS...50.1133C} shows that, DCO$^+$/HCO$^+$ ratio provides information about ionization degree, only in the regions in which CO depletion is negligible (non-dense area). Whereas, in the central core in which CO is depleted significantly, the ratio of N$_2$D$^+$/N$_2$H$^+$ measurement is a better tracer of ionization degree. 

%A theoretical study by \cite{bialy2020cold} shows that detecting H$_2$ vibrational transition from cold dense molecular cloud, may lead to constrain CRIR inside clouds as well. Another study by \cite{2020MNRAS.495L...7B} who has tried to define a relation to calculate CRIR based on the observed column densities, results CRIR to be $\zeta\sim(2-3)\times 10^{-17}s^{-1}$ in a dense core.
%Comparing observed column densities of H$_3$ $^+$ and HCO$^+$ with a model of young massive stars \citep{2000ApJ...537..283V}, constrains CRIR to be $\zeta_{\rm CR}=(2.6\pm1.8)\times 10^{-17} s^{-1}$ \citep{2000A&A...358L..79V}.\\ 

In this paper, we aim to constrain the astrochemical conditions, including CRIR and chemical age, in ten different positions in the massive IRDC G28.36+00.07. We first present a grid of astrochemical models, based on the work of \cite{2015A&A...582A..88W}, that cover a wide range of physical conditions, including those relevant to IRDCs (\S\ref{astrochemical_model}). We next measure the physical properties of mass surface density ($\Sigma$), number density ($n_{\rm H}$) and temperature ($T$) of the IRDC regions (\S\ref{observations}.1), followed by measurements of the column densities and thus abundances of various molecules and molecular ions from IRAM-30m telescope observations (\S\ref{observations}.2). Then, in \S\ref{comparison}, we determine which parts of the multi-dimensional astrochemical model parameter space, including CRIR and time, are consistent with the observations. We discuss the implications of our results in \S\ref{discussion}. We present our conclusions in \S\ref{final}.

%For this purpose, we present the comparison of molecular abundances observed by IRAM 30m telescope, with the astrochemical model provided by \cite{2015A&A...582A..88W}, to be able to find the best models with associated cosmic ray ionization rate. The paper is structured as follows. In sections \ref{astrochemical_model} we describe the model and its properties and interpret its results. In section \ref{observations}, the properties of the observed cloud, detected lines and their obtained abundances is presented. In section \ref{comparison}, the comparison between observation and the model is made. Finally, a summery of our work and obtained results comprise section \ref{final}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Astrochemical model}\label{astrochemical_model}

\subsection{Overview of the Model}

We use the astrochemical model developed by \cite{2015A&A...582A..88W} to predict the evolution of abundances of different species in the gas and grain ice mantle phases. 
%The model, initially used to reproduce molecular abundances in T-tauri type protoplanetary disks, is used here to reproduce chemical compositions of IRDCs in physical property parameter space \citep{2015A&A...582A..88W}.
The model uses a gas-phase network extracted from the UMIST 2012 Database for Astrochemistry \citep{2013A&A...550A..36M}, complemented by both thermal and non-thermal gas-grain processes, including CR-induced desorption, photodesorption, 
X-ray desorption, 
and grain-surface reactions. The reaction types included in the astrochemical code are described in \cite{walsh2010chemical} and the subsequent works \citep{walsh2012chemical,walsh2013molecular,2014A&A...563A..33W,2015A&A...582A..88W}.

However, of these extended reactions, we have switched off CR-induced thermal desorption reactions, since their rates are highly uncertain \citep{cuppen2017grain}. Still, CR-induced photoreactions are included, including those that lead to desorption of species from grain surfaces. In our modeling we do not include any X-ray background, so the reactions involving X-rays do not play any role.
%In the main code of the model, the reactions of direct X-ray ionization has not been considered as well. 
Overall the network includes a total of 8763 reactions following the time evolution of the abundances of 669 species. The elements that are followed in the network and their assumed initial abundances are shown in Table~\ref{tab:initial_abundances}. All elements are initially in atomic form, except for: H, which is almost entirely in the form of $\rm H_2$; C, which is entirely in the form of CO; and 44\% of O that is in the form of CO. This choice is made given that IRDCs are expected to typically be structures within larger-scale molecular clouds.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{chapters/tables/initial_abundances}
\begingroup
\setlength{\tabcolsep}{10pt} % horizontal space
\renewcommand{\arraystretch}{1.3} % vertical space


\begin{table}[H]
\caption{Fiducial Initial Abundances}
\centering
\begin{tabular}{c c}
      \hline
      \hline
      Species & Abundance ($n_{\rm X}/n_{\rm H}$)\\
      \hline
      H$_2$ & 5.00e-01\\
      H & 5.00e-05 \\
      He & 9.75e-02 \\
      CO & 1.40e-04 \\
      O & 1.80e-04 \\
      N & 7.50E-05 \\
      S &  8.00e-08 \\
      F & 2.00e-08 \\
      Si & 8.00e-09 \\
      Cl & 4.00e-09 \\
      P & 3.00e-09 \\
      GRAIN & 1.30e-12\\
    \hline 
    \end{tabular}
    %\vspace{2mm}
    %\caption{Fiducial initial elemental abundances.}
    \label{tab:initial_abundances}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In order to produce the grid of models 
We have adopted the standard parameter values of a Draine FUV radiation field equal to $6.4\times 10^{-3}\:{\rm erg\: cm^{-2}\:s^{-1}}$ and a Habing FUV field equal to $4.0\times 10^8\:{\rm cm^{-2}\:s^{-1}}$. Other standard parameters are the assumed dust particle radius of $a_0=0.1\:{\rm \mu m}$, so that the grain surface area per H nucleus is $1.63\times 10^{-19}\:{\rm cm}^2$.
%jct - this needs to be checked.

%In addition, we have set the initial abundances as reported in Table \ref{tab:initial_abundances}. We note that, for the adopted initial abundances, all the carbon is the form of CO, and corrected to Oxygen abundance accordingly. This assumptions indicates that the chemical evolution in our models occurs after the cloud is formed i.e., when the material is mainly in the molecular form.

Each astrochemical model is run for a fixed set of values of number density of H nuclei ($n_{\rm H}$), gas temperature ($T$), CRIR ($\zeta$), visual extinction ($A_V$), and FUV radiation field intensity ($G_0$). 
%The models are evolved in time for $10^8$~years. 
The range of the parameter space of the grid of the models for this work is presented in Table \ref{tab:initial_parameters}. This parameter space is sampled at a resolution of 3 values per decade for density and CRIR. For temperatures, with a focus on lower values, we run models at 5, 10, 15, 20, 25, 30, 40, 50, ..., 100, 120, ..., 200, 250, 300, ..., 500, 600, ..., 1000 ~K. For $A_V$, we run models at 1, 2, 3, 4, 5, 7, 10, 20, 50, 100~mag.
%focusing on lower temperatures and reducing the resolution as temperature raises, higher resolution of A$_V$s below 10 mag and 
We only run models with one value of external FUV radiation field, i.e., $G_0 = 4$, which is the value expected in the inner Galaxy relevant to most IRDCs \citep{wolfire2010dark}.
%(Wolfire et al. 2010). 
In any case, the typical values of extinctions in IRDCs are very high, so that the external FUV radiation field is expected to play a negligible role in the chemical evolution.

With the above choices, we have a total of 137,750 different physical models. Each of these is evolved in time for $10^8$~years, with a sampling of 100 outputs per decade in time (after $10^3$~years). We note that while we have developed here a relatively wide range of models for a first general exploration, when modeling IRDCs, we will focus on a much narrower range of conditions that are constrained by observational data on the clouds.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{chapters/tables/initial_parameters}
\begingroup
\setlength{\tabcolsep}{10pt} % horizontal space
\renewcommand{\arraystretch}{1.3} % vertical space


\begin{table}[H]
\caption{Model Grid Parameter Space}
\centering
\begin{tabular}{c c c}
      \hline
      \hline
      Parameter & Explored Range \\
      \hline
      $n_{\rm H}$ (cm$^{-3}$) & 10 - $10^9$\\
      $T$ (K) & 5 - 1000\\
      $\zeta$ (s$^{-1}$) & $10^{-19}$ - $10^{-13}$\\
      $A_V$ (mag) & 1 - 100\\
%      t & time & 1.0e3-1.0e8~~year \\
      $G_0$ (Habings) & 4\\
%      a$_0$ & dust particle radius & 0.1 $\mu$m \\
    \hline 
    \end{tabular}
    \label{tab:initial_parameters}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\large CO Depletion Factor}
\label{co depletion factor}

In this section we study how the CO depletion factor, $f_{D}$, varies with astrochemical conditions. CO is typically the second most abundant molecule in molecular clouds after $\rm H_2$ and so it is important to understand its behaviour.
%The physical and chemical properties of different regions in the IRDCs may be reflected in the abundance of CO, causing variation in the CO abundance and consequently its depletion factor across the cloud \citep{2011ApJ...738...11H}. 
One of the main expectations is that CO freezes out rapidly from the gas phase at temperatures $\lesssim 20$~K, but then with eventual abundances set by a balance of the non-thermal desorption processes from the grains.

%jct - maybe we will discuss the comparison to observational data later.
%Previous works have shown that the CO depletion factor (f$_D$) depends on the density of the Hydrogen and in particular it is higher in the regions with high densities \citep{2011ApJ...738...11H} which is consistent with the study by \cite{2016A&A...587A..96P}. At this work f$_D$ has been estimated to lie between 16-31 towards IRDC G28 (C1) at which density is set to 5e4 cm$^{-3}$, whereas CO depletion factor has been estimated lower (5-9) towards IRDC G34, at which the density is lower approximately by the factor of 2 (2e4 cm$^{-3}$).
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htb!]
    \centering
     \includegraphics[width=\textwidth]{chapters/images/fD.pdf}
     \vspace*{-12mm}
     \caption{Time evolution of CO depletion factor, $f_D$, as a function of the environmental variables of: (a) top left - number density of H nuclei, $n_{\rm H}$; (b) top right - temperature, $T$; (c) bottom left - cosmic ray ionization rate, $\zeta$; (d) bottom right - visual extinction, $A_V$. In each panel the three remaining variables are held fixed at their fiducial level, i.e., $n_{\rm H}=10^5\:{\rm cm}^{-3}$, $T=20\:$K, $\zeta=10^{-16}\:{\rm s}^{-1}$, $A_V=100$~mag. Each time-evolving model is shown by a horizontal line with $f_D$ indicated by the color scale.
     }
     \label{fig:fD}
   %\end{subfigure}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!htb]
    \centering
     \includegraphics[width=\textwidth]{chapters/images/fD_15K.pdf}
     \vspace*{-12mm}
     \caption{Time evolution of CO depletion factor, $f_D$, as a function of the environmental variables of: (a) top left - number density of H nuclei, $n_{\rm H}$; (b) top right - temperature, $T$; (c) bottom left - cosmic ray ionization rate, $\zeta$; (d) bottom right - visual extinction, $A_V$. In each panel the three remaining variables are held fixed at their fiducial level, i.e., $n_{\rm H}=10^5\:{\rm cm}^{-3}$, $T=15\:$K, $\zeta=10^{-16}\:{\rm s}^{-1}$, $A_V=100$~mag. Each time-evolving model is shown by a horizontal line with $f_D$ indicated by the color scale.
     }
     \label{fig:fD_15K}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
 \begin{figure*}[!htb]
    \centering
     \includegraphics[width=\textwidth]{chapters/images/fD_values.pdf}
     \vspace*{-1.5cm}
     \caption{CO depletion factor, $f_D$, at fixed times of $10^5$ (circles), $10^6$ (triangles), $10^7$ (squares) and $10^8$~yr (stars) as a function of the environmental variables of: (a) top left - number density of H nuclei, $n_{\rm H}$; (b) top right - temperature, $T$; (c) bottom left - cosmic ray ionization rate, $\zeta$; (d) bottom right - visual extinction, $A_V$. In each panel the three remaining variables are held fixed at their fiducial level, i.e., $n_{\rm H}=10^5\:{\rm cm}^{-3}$, $T=20\:$K, $\zeta=10^{-16}\:{\rm s}^{-1}$, $A_V=100$~mag.
     }
     \label{fig:fD_values}
 \end{figure*}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{figure*}[!htb]
    \centering
     \includegraphics[width=\textwidth]{chapters/images/fD_values_15K.pdf}
     \vspace*{-1.5cm}
     \caption{CO depletion factor, $f_D$, at fixed times of $10^5$ (circles), $10^6$ (triangles), $10^7$ (squares) and $10^8$~yr (stars) as a function of the environmental variables of: (a) top left - number density of H nuclei, $n_{\rm H}$; (b) top right - temperature, $T$; (c) bottom left - cosmic ray ionization rate, $\zeta$; (d) bottom right - visual extinction, $A_V$. In each panel the three remaining variables are held fixed at their fiducial level, i.e., $n_{\rm H}=10^5\:{\rm cm}^{-3}$, $T=15\:$K, $\zeta=10^{-16}\:{\rm s}^{-1}$, $A_V=100$~mag.
     }
     \label{fig:fD_values_15K}
 \end{figure*}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the following, we define $f_{D}$ via: %(\ref{rel:fd}) and will discuss its variation as a function of the model parameters.
\begin{equation}
    f_{D}(t) = \frac{1.4 \times 10^{-4}}{X[{\rm CO}](t)},
    \label{rel:fd}
\end{equation}
where $1.4 \times 10^{-4}$ is the initial gas phase abundance of CO with respect to H nuclei in our models (i.e., assuming all C is in this form) and $X[{\rm CO}](t)$ is the actual gas phase abundance of CO with respect to H nuclei, which evolves in time.

To explore the time evolution of $f_D$ and its dependence on density, temperature, CRIR and $A_V$, we choose a fiducial reference case with $n_{\rm H}=10^5\:{\rm cm}^{-3}$, $T=20\:$K, $\zeta=10^{-16}\:{\rm s}^{-1}$ and $A_V=100\:$mag. We then vary each of these variables systematically, while holding the others constant. The results are shown in Figures~\ref{fig:fD}a-d. Simple profiles of $f_D$ versus these environmental variables at several fixed times are shown in Figure~\ref{fig:fD_values}a-d. The time evolution of the abundances of CO, $\rm HCO^+$ and $\rm N_2H^+$ are shown in Figures~\ref{fig:CO_evolution_fD}a-d. We now discuss these results in the following four sub-sections.



%Figure~\ref{fig:fD} shows the time evolution of $f_D$, with respect to CRIR (panel a), visual extinction (panel b), gas temperature (panel c) and hydrogen density (panel d). The different colors correspond to different f$_D$ values. For each panel, the remaining parameters have been set to the value of our fiducial model as listed in Table~\ref{tab:fiducial_parameters}.



%Figure ~\ref{fig:fD_values} and Figure ~\ref{fig:CO_evolution_fD} show f$_D$ at different time steps with respect to different parameters and evolution of CO, together with two other species (HCO$^+$, N$_2$H$^+$) respectively.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\begin{figure*}[!htb]
\centering
\includegraphics[width=\textwidth]{chapters/images/CO_HCO_N2H_evolution.pdf}
     \vspace*{-20mm}
     \caption{\tiny Time evolutions of the abundances of CO (left column), HCO$^+$ (middle column) and N$_2$H$^+$ (right column), exploring the effects of the environmental variables of: (a) top row - number density of H nuclei, $n_{\rm H}$; (b) second row - temperature, $T$; (c) third row - cosmic ray ionization rate, $\zeta$; (d) bottom row - visual extinction, $A_V$. In each row the three remaining variables are held fixed at their fiducial level, i.e., $n_{\rm H}=10^5\:{\rm cm}^{-3}$, $T=20\:$K, $\zeta=10^{-16}\:{\rm s}^{-1}$, $A_V=100$~mag.
     }
     \label{fig:CO_evolution_fD}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!htb]
\centering
\includegraphics[width=\textwidth]{chapters/images/CO_HCO_N2H_evolution_15_K.pdf}
     \vspace*{-20mm}
     \caption{\tiny Time evolutions of the abundances of CO (left column), HCO$^+$ (middle column) and N$_2$H$^+$ (right column), exploring the effects of the environmental variables of: (a) top row - number density of H nuclei, $n_{\rm H}$; (b) second row - temperature, $T$; (c) third row - cosmic ray ionization rate, $\zeta$; (d) bottom row - visual extinction, $A_V$. In each row the three remaining variables are held fixed at their fiducial level, i.e., $n_{\rm H}=10^5\:{\rm cm}^{-3}$, $T=15\:$K, $\zeta=10^{-16}\:{\rm s}^{-1}$, $A_V=100$~mag.
     }
     \label{fig:CO_evolution_fD_15K}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\begin{figure*}[!ht]
%    \centering
%    \addtolength{\leftskip} {-2.3cm}
%    \addtolength{\rightskip}{-1cm}
%     \includegraphics[width=23cm, height=4cm]
%     {chapters/images/n_rates.pdf}
%     \caption{\tiny Evolution of the rates of multiple reactions with the highest rates, in the models with different n(H). The rest of the parameters have been set to the value of fiducial model (Fig~\ref{tab:fiducial_parameters})}
%     \label{fig:n_rates}
% \end{figure*}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}[!ht]
%    \centering
%    \addtolength{\leftskip} {-2.3cm}
%    \addtolength{\rightskip}{-1cm}
%     \includegraphics[width=23cm, height=4cm]
%     {chapters/images/T_rates.pdf}
%     \caption{\tiny Evolution of the rates of multiple reactions with the highest rates, in the models with different T. The rest of the parameters have been set to the value of fiducial model (Fig~\ref{tab:fiducial_parameters}).}
%     \label{fig:T_rates}
% \end{figure*}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{figure*}[!ht]
%    \centering
%    \addtolength{\leftskip} {-2.3cm}
%    \addtolength{\rightskip}{-1cm}
%     \includegraphics[width=23cm, height=4cm]
%     {chapters/images/CRIR_rates}
%     \caption{Evolution of the rates of multiple reactions with the highest rates, in the models with different CRIRs. The rest of the parameters have been set to the value of fiducial model (Fig~\ref{tab:fiducial_parameters}).}
%     \label{fig:CRIR_rates}
% \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Dependence on Density}

In the high density regime, $n_{\rm H}\gtrsim 10^5\:{\rm cm}^{-3}$, the general trend shown in Figure~\ref{fig:fD}a is that the CO depletion factor increases with time and can reach very high values, $f_D\gtrsim20$, within a few Myr. As expected, the evolution proceeds more quickly at higher densities, which lead to higher rates of CO molecules hitting and sticking to the dust grains.

At low densities, $n_{\rm H}\lesssim 10^2\:{\rm cm}^{-3}$, the freeze-out rates become very low and competing processes that destroy CO, e.g., via interaction with CR-produced He$^+$ or CR-induced FUV photons, become more important. Note that since $A_V=100\:$mag, the destruction of CO via external FUV photons is unimportant. The system evolves to having most of the C in atomic or ionized form, and hence the CO abundance is lowered and $f_D$ appears large.

Focusing on the density range that is relevant to IRDCs, i.e., $n_{\rm H}\sim 10^4$ to $10^5\:{\rm cm}^{-3}$, we see from Fig.~\ref{fig:fD_values}a that after 1~Myr $f_D$ is still quite small ($\lesssim 2$), but by 10~Myr it has reached near equilibrium values of about 5 to 100 from the low to high ends of this density range. However, note that this time evolution is very sensitive to the temperature, since the rate of thermal desorption reduces dramatically for $T\leq20\:$K. Thus for models at 15~K, relatively high levels of CO depletion of $f_D\sim5-10$ can be achieved even within $\sim10^5\:$yr at typical IRDC densities.

%When the number density of H nuclei ($n_{\rm H}$) is very low (1.0e2 cm$^{-3}$), thermal desorption and freeze-out rates are unimportant. Due to the low density, CRs can penetrate easily through the medium to ionize the main component (H$_2$) and consequently form H$_3$ $^+$ so that CO is formed and destructed dominantly by mentioned reactions previously (reactions~\ref{rel:top_rates_zeta}) (panel a in Figure~\ref{fig:n_rates}). In this case, C is depleted mostly due to the reaction below. Thus most of C, can be found in atomic or ionized form (C, C$^+$):
 
%\begin{equation}
%\begin{split}
%    \rm CO + CRPHOT \longrightarrow \rm C + \rm O\\
%    \rm He^{+} + \rm CO \longrightarrow \rm O + \rm C^{+} + \rm He \\
%\end{split}
%\end{equation}
 
 
%As the density increases the rate of the reactions increase as well (panel b in Figure~\ref{fig:n_rates}) and when the density reaches $\sim$ 1.0e4 cm$^{-3}$ (panel c in Figure~\ref{fig:n_rates}) , thermal desorption becomes the second dominant reaction to form CO gas phase. As n(H) gets bigger (panel d and e in Figure~\ref{fig:n_rates}), the rate freeze-out raises as well and it becomes the main reaction to destruct CO, before 1.0e6 years.


%Figure~\ref{fig:fD} and \ref{fig:CO_evolution_fD} shows that, as number density of Hydrogen increases up to 1.0e3 cm$^{-3}$, f$_D$ decreases. After that, by increasing density, CO is depleted more and begins its depletion at earlier times. The results of our model (Figure~\ref{fig:fD_values}) shows that, f$_D$ is $\approx$ 15-33, when the density is in the range of (2.2-4.6)e4 cm$^{-3}$, with the age of above 10Myear, which is in agreement with the studies by \cite{2016A&A...587A..96P} and \cite{2011ApJ...738...11H}.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subsubsection{Dependence on Temperature}
 
Time dependant evolutions of $f_D$ at different temperatures are shown in Figures~\ref{fig:fD}b and \ref{fig:fD_values}b. The actual gas phase abundances of CO versus time for these models are shown in Figure~\ref{fig:CO_evolution_fD}b, along with similar evolutions of $\rm HCO^+$ and $\rm N_2H^+$. The strong dependence of $f_D$ evolution with $T$ in the range from $\sim10-50$~K is clearly illustrated, i.e., above this temperature range, gas phase CO remains the main reservoir of C. At temperature $\gtrsim500\:$K, C is still mostly in the gas phase, but not in the form of CO.



%CO (see figure \ref{fig:CO_evolution_fD}) at different temperatures shows that as temperature increases, CO depletion decreases. After 50 K, CO remains in gas phase and f$_D$ stays below 2 (Figure \ref{fig:fD} (panel c)) , until the temperature exceeds a limit(>500 K). In the Figure~\ref{fig:T_rates} (panel a), it is clearly seen that at low temperature (T=15 K), thermal desorption mechanism is not the dominant reaction and CO is formed mainly by:
 
%\begin{equation}
%\begin{split}
%    \rm HCO^+ + \rm e \longrightarrow \rm CO + \rm H\\
%\end{split}
%\end{equation}

%While in the same model, CO is depleted mostly with freeze out at earlier times, as we move forward in time, CO destruction with H$_3^+$ and producing HCO$^+$ and H$_2$ becomes the dominant ones after 1.0e5 years. As temperature raises, CO molecules are released from the surface of the grains meaning the increasing of thermal desorption rate which is seen from Figure~\ref{fig:T_rates} (panel b). By increasing temperature (Figure~\ref{fig:T_rates} (panel c and d) thermal desorption and freeze-out become the dominant reaction of CO formation and destruction, independent of the time scale. At higher temperatures (Figure~\ref{fig:T_rates} (panel e),whereas  thermal desorption and freeze-out are still the main reactions, majority of C is found in HCN gas phase which is formed mostly via the below reactions:

%\begin{equation}
%\begin{split}
%    \rm GHCN \longrightarrow \rm HCN\\
%    \rm H_2 + \rm CN \longrightarrow \rm HCN + \rm H \\
%\end{split}
%\end{equation}
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\subsubsection{Dependence on Cosmic Ray Ionization Rate}

Time dependant evolutions of $f_D$ at different CRIRs are shown in Figures~\ref{fig:fD}c and \ref{fig:fD_values}c. The actual gas phase abundances of CO versus time for these models are shown in Figure~\ref{fig:CO_evolution_fD}c, along with similar evolutions of $\rm HCO^+$ and $\rm N_2H^+$. {\bf NE: In this figure, we see oscillation in the abundances of CO, HCO$^+$ and N$_2$H$^+$ at early times, in the model at which the CRIR is in highest level and the value of $\frac{n(H)}{\zeta}$ is 1.0e18 cm$^{-3}$s. Figures~\ref{fig:os_n} and \ref{fig:os_cr} indicates that the oscillatory feature appears in the models at which this ratio is between 1.0e18 and 2.2e18 cm$^{-3}$ s$^{-1}$, the models with lower densities and higher CRIR consistenting with previous studies \citep{maffucci2018astrochemical}, which probably corresponds to the High Ionization Phase (HIP) \citep{roueff2020sustained}.} 
%In upper left panel in figure \ref{fig:fD} and the upper left panel in figure ~\ref{fig:CO_evolution_fD} the variation of f$_D$ with respect to $\zeta$ is shown. 
These figures indicate that as $\zeta$ increases, CO depletion begins earlier in time, but reaches a lower equilibrium value. A different mode of evolution occurs at the highest value of CRIR ($\zeta = 10^{-13}\:{\rm  s}^{-1}$), in which C is mostly in the form of $\rm C^+$.

%Figure~\ref{fig:CRIR_rates} demonstrates that at very low CRIR (panel a), CO is formed and destructed dominantly by thermal desorption and freeze-out respectively.

%As $\zeta$ increases ($\zeta$=1.0e-17 s$^{-1}$) (panel b in Fig~\ref{fig:CRIR_rates}), thermal desorption and freeze-out reactions are still the most dominant reactions up to about 10 million years. But after that, CO major production and destruction rates via reactions~\ref{rel:top_rates_zeta}, decrease by the factor of approximately 2 orders of magnitude which causes the drastic grow of f$_D$ by the factor of approximately 2 orders of magnitude (\ref{fig:CRIR_rates}). 

%As $\zeta$ gets bigger (panel c and d in Fig~\ref{fig:CRIR_rates}, the high level of CRIR bursts the abundance of molecular ions such as H3$^+$ and HCO$^+$. Reactions of molecular ions thus became the main routes of CO production and destruction. In the first 1.0e3 years, CO abundance is mainly regulated by the following reactions of H3$^+$ and HCO$^+$, while at later time, CO is mainly destructed by reactions with He$^+$.

%\begin{equation}
%\begin{split}
%    \rm HCO^+ + \rm e^- \longrightarrow CO + H\\
%    \rm H3^+ + CO \longrightarrow \rm HCO^+ + \rm H_2\\
%    \label{rel:top_rates_zeta}
%\end{split}
%\end{equation}

%In the models with values of CRIR higher than our fiducial one, CO is more efficiently destructed at later times (<1.0e6 years), except the model with the highest $\zeta\:=\:1.0e-13\:s^{-1}$. At this model, CO depletion begins even earlier than 1.0e3 years with the gas phase Carbon being mostly in the form of C+, which is the result of higher CRIR directly and indirectly as bellow:


%\begin{equation}
%\begin{split}
%    \rm He^+ + \rm CO \longrightarrow \rm O + \rm C^{+} + \rm He\\
%    \rm C + \rm CRPHOT \longrightarrow \rm C^{+} + \rm e\\
%\end{split}
%\end{equation}

%and,

%\begin{equation}
%\begin{split}
%    \rm C^{+} + \rm e \longrightarrow \rm C + \rm PHOTON\\
%    \rm H + \rm CH \longrightarrow \rm C + \rm H2\\
%\end{split}
%\end{equation}
%Where CRPHOT is defined as cosmic rays photons.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Dependence on Visual Extinction}

%\begin{figure*}[!ht]
%    \centering
%    \addtolength{\leftskip} {-2.7cm}
%    \addtolength{\rightskip}{-1.8cm}
%     \includegraphics[width=17cm, height=4cm]
%     {chapters/images/Av_rates.pdf}
%     \caption{\tiny Evolution of the rates of multiple reactions with the highest rates, in the models with different A$_v$. The rest of the parameters have been set to the value of fiducial model (Fig~\ref{tab:fiducial_parameters}).}
%     \label{fig:Av_rates}
% \end{figure*}

Time dependant evolutions of $f_D$ at different CRIRs are shown in Figures~\ref{fig:fD}d and \ref{fig:fD_values}d. The actual gas phase abundances of CO versus time for these models are shown in Figure~\ref{fig:CO_evolution_fD}d, along with similar evolutions of $\rm HCO^+$ and $\rm N_2H^+$.
These figures show that in the models with $A_V>5$~mag, CO evolution has little dependency on the level of visual extinction so that CO depletion becomes large after about 1 Myr, no matter the value of $A_V$.

%It is demonstrated in Figure~\ref{fig:Av_rates} (panel a) that at very low A$_v$, CO remains in gas phase and f$_D$ stays below 2, which is the result of equilibrium between thermal desorption and freeze-out.

%As A$_v$ increases (panel b and c in Figure~\ref{fig:Av_rates}), the rates of thermal desorption and freeze-out decreases, but instead the rates of the reactions~\ref{rel:top_rates_zeta}, which are responsible of CO formation and destruction, increases Figure~\ref{fig:Av_rates} (panel b and c) and Figure~\ref{fig:fD} shows that in the model with the highest A$_v$ (100 mag), CO starts to be depleted since $\approx$ 1.0e6 years and reaches equilibrium before $\approx$ 1.0e7 years.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Observational Data and Abundance Estimates} \label{observations}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{chapters/tables/table2}
\setlength{\tabcolsep}{7pt} % horizontal space
\renewcommand{\arraystretch}{1.4} % vertical space

\begin{table*}[t]\centering
\caption{Observed molecular species, rest frequencies, rotational quantum numbers of the transitions, rotational constants, rotational partition function, Einstein $A$ coefficients, energy of lower state, degeneracy of upper state, velocity resolution, $B_{\rm eff}$ and HPBWs.}
  \begin{tabular}{c c c c c c c c c c c}
  \hline
  \hline
  molecule & $\nu$ (GHz) & $J$ & $B$~(Hz) & $Q_{\rm rot}$($T_{\rm ex}$=7.5K) & $A$~(s$^{-1}$) & $E_{L}$~(K) & $g_{u}$ & $dv$~(km s$^{-1}$) & $B_{\rm eff}$ & $\theta(\arcsec)$ \\
  \hline
   HC$^{18}$O$^+$ & 85.1621570 & 1-0 & 4.26e10 & 3.90  & 3.6450E-05 & 0.00 & 3 &  0.6876 & 0.81 & 28.89\\
    \hline
    H$^{13}$CO$^+$ & 86.7542884 & 1-0 & 4.34e10 & 3.83 & 3.8539E-05 & 0.00 & 3 &  0.6749 & 0.81 & 28.36 \\
    \hline
    %SiO & 86846.96 & Q($T_{ex}$) = 1.010600$\times T^{0.990020}$ & 2.9275E-05 & 2.08 & 5 & 0.6742 & 83.39\\
    %\hline
     HN$^{13}$C & 87.0908500 & 1-0 & 4.35e10 &  3.82 & 2.3840E-05 & 0.00 & 3 & 0.6723 & 0.81 & 28.25\\
    \hline
     %CCH & 87316.925 & Q($T_{ex}$) = 2.106200$\times T^{0.981580}$ & 1.5314E-06 & 0.00216 & 3 & 0.6706 & 83.30\\
    %\hline
    HNCO & 87.9250443 & 4-3 & 1.11e10 & 36.90 & 8.7801E-06 & 6.33 & 9 & 0.6659 & 0.81 & 27.98\\
    \hline
    HCN & 88.6304160 & 1-0 & 4.43e10 & 3.88 & 8.0884E-06 & 0.00 & 3 & 0.6606 & 0.81 & 27.76\\
    \hline
    N$_2$H$^+$ & 93.1761300 & 1-0 & 4.66e10 & 3.71 & 3.6300E-05 & 0.00 & 3 & 0.0628 & 0.80 & 26.40\\
    \hline
    C$^{18}$O & 109.7821734 & 1-0 & 5.49e10 & 3.11& 6.2661E-08 & 0.00 & 3 & 0.0533 & 0.78 & 22.41\\
    \hline
     %DCO+ & 144077.2144 & Q($T_{ex}$) = 1.842760$\times T^{0.991545}$ & 2.1184E-04 & 3.46 & 5 & 0.4064 & 72.82 \\
    %\hline
     CH$_3$OH & 145.1031850 & 3-2 & 2.47e10 & 13.25 & 1.2323E-05 & 6.96 & 7 & 0.4035 & 0.73 & 16.95\\
    \hline
    H$_2$CO & 145.6029490 & 2-1 & 3.88e10 & 10.52 & 7.8127E-05 & 3.49 & 5 & 0.4021 & 0.73 & 16.90\\
    \hline
    %\dots & \dots
  \end{tabular}
  \vspace*{1mm}
  
  \label{tab:modelcules_parameters_Ntot}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Molecular Line Data}
The rotational transitions listed in Table~\ref{tab:modelcules_parameters_Ntot} were mapped toward the IRDC G28.37+00.07 (hereafter Cloud C, Butler \& Tan \citeyear{butler2009mid,butler2012mid}) in August 2008, May 2013 and September 2013 using the IRAM (Instituto de Radioastrom\'ia Milim\'etrica) 30m telescope in Pico Velata, Spain. Observations were performed in On-The-Fly mode with map size $264\arcsec\times252\arcsec$; central coordinates $\alpha = 18^{h}42^{m}52.3^{s}$, $\delta =-4^{\circ}02\arcmin26.2\arcsec$; and off position (-370$\arcsec$, 30$\arcsec$). 
An angular separation in the direction perpendicular to the scanning direction of 6$\arcsec$ was adopted.

The FTS spectrometer was used for observations of $\rm C^{18}O(1-0)$ and $\rm N_2H^+(1-0)$, which provided a spectral resolution of 200 kHz, corresponding to a velocity resolution of 0.053 and 0.063~$\rm km\:s^{-1}$, respectively. For the other transitions, the data have velocity resolutions of $\sim0.4$ to $0.7\:{\rm km\:s}^{-1}$.
%jct - more information is needed about this observing mode
In the worst case, i.e., at the lowest frequency of 81.5~GHz, the angular resolution of the molecular line data has a HPBW of $32\arcsec$.
Peak intensities were measured in units of antenna temperature, $T^{\star}_{A}$, and converted into main-beam temperature, $T_{\rm mb}$. Beam and forward efficiencies of 0.73 and 0.95, respectively, for $\nu\sim145\:$GHz, and 0.86 and 0.95 for $\nu\sim86\:$GHz were used. The final data cubes were produced using the {\sc CLASS} and {\sc MAPPING} software within the {\sc GILDAS} package\footnote{https://www.iram.fr/IRAMFR/GILDAS/}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mass Surface Density and Temperature Data}

The MIR extinction (MIREX) map of \cite{butler2012mid}, derived from 8~$\rm \mu m$ {\it Spitzer}-IRAC imaging data, with the NIR correction of \cite{2013A&A...549A..53K}, was used as a first method to estimate the mass surface density, $\Sigma$, of selected regions in the IRDC. The advantage of this map is that it has a high angular resolution of 2\arcsec\ and the derivation of $\Sigma$ does not depend on the temperature of the cloud. The disadvantages of the map are that it cannot make a measurement in regions that are MIR bright. Furthermore, the map saturates at values of $\Sigma\sim 0.5\:{\rm g\:cm}^{-2}$, i.e., in regions with $\Sigma$ approaching this value the map underestimates the true value of $\Sigma$.

An independent measure of $\Sigma$ for the IRDC has been derived by \cite{lim2016distribution} based on {\it Herschel}-PACS and SPIRE sub-mm emission imaging data, with this analysis also simultaneously yielding an estimate of the dust temperature. These maps have an angular resolution of $18\arcsec$ for the $\Sigma$ map and $36\arcsec$ for the $T$ map, i.e., much lower than that of the MIREX map. As discussed by \cite{lim2016distribution}, there are significant effects due to Galactic plane foreground and background emission that contaminate that arising from the IRDC itself. In our analysis, we make use of the map derived from the Galactic Gaussian (GG) foreground-background subtraction method.

%Finally, we have made use, in our analysis, of the dust temperature and H$_2$ mass surface density ($\Sigma$) maps obtained by \cite{lim2016distribution} and \cite{2013A&A...549A..53K}, from Herschel and a combination of NIR and MIR data, respectively.
%of cloud C (see Figure\ref{fig:sigma_T_map}), obtained by \citep{lim2016distribution}, from a combination of Herschel images at 70 $\mu$m and Spitzer images at 8 $\mu$m and 24 $\mu$m. We also extracted $\Sigma$ values from the map obtained by \citep{2013A&A...549A..53K} (see table\ref{tab:physical_parameters_IRDC}), although we will continue with the data obtained by \citep{lim2016distribution}.

\subsection{Ten Selected IRDC Regions}

From the final data cubes, we extracted molecular line spectra from ten regions in the IRDC (see Figure \ref{fig:sigma_T_map}). Each region has a circular aperture of radius $16\arcsec$, which was set so that the angular resolution of the HPBW of the lowest frequency transition, i.e., from $\rm HC^{18}O^+(1-0)$, fits within the region. At the 5~kpc distance of the IRDC, the radius of each region corresponds to 0.39~pc.

The locations of the ten positions were selected for having relatively high values of $\Sigma$ and for having a range of star formation activities. In particular, positions P1 to P6 (shown with red circles in Figure \ref{fig:sigma_T_map}) are known to be sites of active star formation based on the presence of CO outflows \citep{kong2019widespread} and containing {\it Herschel}-Hi-GAL 70~$\rm \mu m$ point sources \citep{moser2020high}. However, these positions are still dark structures at $8~{\rm \mu m}$: indeed the P1 to P6 positions correspond approximately to the MIREX $\Sigma$ peaks of C1, C2, C4, C5, C6 and C8, respectively, identified and characterised by \cite{butler2012mid}.

\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.9cm}
    %\addtolength{\rightskip}{-1.5cm}
     \includegraphics[width=\textwidth]{chapters/images/H2_map.pdf}
    \vspace*{-14mm}
    \caption{(a) Left: MIREX derived mass surface density map of IRDC G28.37+00.07 from \cite{2013A&A...549A..53K} (scalebar is in $\rm g\:cm^{-2}$). The ten regions selected for our astrochemical study are marked with circles, labelled 1 to 10. Regions 1 to 6 (red) are known to harbor some star formation activity, while regions 7-10 have been specifically selected to avoid known protostellar sources. (b) Right: Sub-mm emission derived mass surface density map of the IRDC from \cite{lim2016distribution} using the Galactic Gaussian method of foreground-background subtraction (scalebar is in $\rm g\:cm^{-2}$). Note, it is of significantly lower angular resolution than the MIREX map (see text). The analysed positions are marked as in (a).}
    \label{fig:sigma_T_map}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.9cm}
    %\addtolength{\rightskip}{-1.5cm}
     \includegraphics[width=\textwidth]{chapters/images/T_map.pdf}
    \vspace*{-14mm}
    \caption{Sub-mm emission derived dust temperature map of IRDC G28.37+00.07 from \cite{lim2016distribution} using the Galactic Gaussian method of foreground-background subtraction (scalebar in K). The ten regions selected for our astrochemical study are marked with circles, labelled 1 to 10, as in Fig.~\ref{fig:sigma_T_map}.
    }
    \label{fig:T_map}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

The positions from P7 to P10 (shown with black circles in Figures~\ref{fig:sigma_T_map} and \ref{fig:T_map}) are not directly associated with massive condensations previously identified within the cloud \citep{rathborne2006infrared,butler2009mid,butler2012mid} and have been selected for being relatively quiescent in terms of their star formation activity \citep{2018ApJ...867...94K,moser2020high}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{chapters/tables/table1}
%\input{chapters/tables/table3_positions_abundances}

%\input{chapters/tables/landscape}
\begin{landscape}
\setlength{\tabcolsep}{9pt} % horizontal space
\renewcommand{\arraystretch}{1.8} % vertical space

\begin{table}[htpb!]\centering
 \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{c c c c c c c c c c c c c c c c c c c c c c}
  \hline
  \hline
          position & R.A. & Dec. &  $\Sigma$ & $N_H$ & $n_H$ & $A_{V,{\rm tot}}$ & $\bar{A}_V$ & T & [C$^{18}$O] & [CO] & [H$^{13}$CO$^{+}$] & [HCO$^+$] & [HC$^{18}$O$^{+}$] & [HCO$^+$] & [N$_2$H$^+$] & [HN$^{13}$C] & [HNC] & [HCN] & [HNCO] & [H$_2$CO] & [CH$_3$OH] \\
           & (J2000) & (J2000) & [gcm$^{-2}$] & [10$^{23}$ cm$^{-2}$] & [10$^{4}$ cm$^{-3}$] & [mag] & [mag] & [K] & [10$^{-8}$] & [10$^{-5}$] & [10$^{-11}$] & [10$^{-10}$] & [10$^{-12}$] & [10$^{-10}$] & [10$^{-10}$] & [10$^{-11}$] &  [10$^{-10}$] & [10$^{-11}$] & [10$^{-10}$] & [10$^{-11}$] & [10$^{-9}$] \\
         \hline
         \rule{0pt}{2ex}
         P1 & 18:42:46.687 & -4:04:08.830 & 0.394 & 1.68 & 10.50 & 88.4 & 22.1 & 11.8 & $4.77\pm$1.47 & $1.52\pm$0.56 & $1.02\pm$0.31 & $4.11\pm$1.51 & $1.96\pm$0.69 & $6.23\pm$2.54 & $0.55\pm$0.17 & $1.41\pm$0.43 & $5.65\pm$2.08 & $11.10\pm$3.44 & $2.17\pm$0.74 & $3.89\pm$1.26 & $0.52\pm$0.18\\
         & & & 0.270 & 1.15 & 7.19 & 60.7 & 15.2 & \\
         \hline
         P2 & 18:42:50.709 & -4:03:14.763 & 0.438 & 1.87 & 11.70 & 98.4 & 24.6 & 13.1 & $4.31\pm$1.33 & $1.37\pm$0.51 & $1.11\pm$0.34 & $4.48\pm$1.64 &$1.84\pm$0.67 & $5.84\pm$2.43 & $1.79\pm$0.56 & $1.61\pm$0.50 & $6.47\pm$2.37 & $10.30\pm$3.22 & $4.29\pm$1.45 & $10.40\pm$3.33 & $1.73\pm$0.60\\
         & & & 0.296 & 1.26 & 7.88 & 66.6 & 16.6\\
         \hline
        P3 & 18:42:49.490 & -4:02:21.514 & 0.330 & 1.41 & 8.84 & 74.2 & 18.6 & 13.5 & $4.86\pm$1.50 & $1.54\pm$0.57 & $0.87\pm$0.27 & $3.49\pm$1.28 &$1.88\pm$0.74 & $5.96\pm$2.64 & $1.53\pm$0.47 & $1.85\pm$0.57 & $7.43\pm$2.73 & $5.86\pm$1.88 & $4.15\pm$1.41 & $7.33\pm$2.37 & $1.74\pm$0.61\\
        & & & 0.265 & 1.13 & 7.06 & 59.6 & 14.9 \\
        \hline
        P4 & 18:42:52.583 & -4:02:44.647 & 0.322 & 1.38 & 8.65 & 72.6 & 18.2 & 13.4 & $5.19\pm$1.60 & $1.65\pm$0.61 & $0.97\pm$0.30 & $3.89\pm$1.43 &$1.64\pm$0.65 & $5.23\pm$2.31 & $1.52\pm$0.47 & $1.64\pm$0.51 & $6.59\pm$2.43 & $8.16\pm$2.57 & $3.45\pm$1.18 & $7.66\pm$2.47 & $1.33\pm$0.46\\
        & & & 0.267 & 1.14 & 7.12 & 60.1 & 15.0\\
        \hline
        P5 & 18:42:53.970 & -4:02:31.320 & 0.336 & 1.44 & 9.02 & 75.8 & 19.0 & 13.8 & $5.58\pm$1.72 & $1.77\pm$0.65 & $1.02\pm$0.32 & $4.10\pm$1.52 &$2.19\pm$0.78 & $6.98\pm$2.86 & $1.10\pm$0.34 & $1.24\pm$0.39 & $4.97\pm$1.84 & $8.53\pm$2.69 & $2.74\pm$0.94 & $6.98\pm$2.25 & $1.26\pm$0.44\\
        & & & 0.259 & 1.11 & 6.94 & 58.3 & 14.6\\
        \hline
        P6 & 18:43:00.610 & -4:01:32.639 & 0.130 & 0.56 & 3.48 & 29.2 & 7.3 & 14.1 & $11.00\pm$3.40 & $3.51\pm$1.29 & $1.52\pm$0.48 & $6.11\pm$2.27 & & & $2.62\pm$0.81 & $2.85\pm$0.89 & $11.40\pm$4.24 & $26.60\pm$8.29 & $1.91\pm$0.72 & $3.31\pm$1.19 & $0.49\pm$0.18 \\
        & & & 0.187 & 0.80 & 4.99 & 42.1 & 10.5\\
        \hline
        P7 & 18:42:54.636 & -4:00:52.451 & 0.239 & 1.02 & 6.39 & 53.7 & 13.4 & 14.9 & $6.68\pm$2.06 & $2.12\pm$0.78 & $0.84\pm$0.26 & $3.37\pm$1.25 & & & $0.91\pm$0.28 & $0.94\pm$0.30 & $3.79\pm$1.43 & $10.10\pm$3.28 & $1.78\pm$0.64 & $2.76\pm$0.94 & $0.45\pm$0.16\\
        & & & 0.193 & 0.83 & 5.16 & 43.4 & 10.9\\
        \hline
        P8 & 18:42:55.289 & -4:01:21.835 & 0.270 & 1.15 & 7.21 & 60.5 & 15.1 & 13.6 & $5.79\pm$1.79 & $1.84\pm$0.68 & $0.69\pm$0.22 & $2.77\pm$1.04 & & & $0.80\pm$0.25 & $0.91\pm$0.29 & $3.67\pm$1.38 & $10.50\pm$3.33 & $1.40\pm$0.51 & $2.19\pm$0.73 & $0.33\pm$0.12\\
         & & & 0.195 & 0.83 & 5.21 & 43.9 & 11.0\\
        \hline
        P9 & 18:42:50.591 & -4:02:47.469 & 0.315 & 1.35 & 8.46 & 71.1 & 17.8 & 13.3 & $5.13\pm$1.58 & $1.63\pm$0.60 & $0.96\pm$0.30 & $3.84\pm$1.41 & & & $1.14\pm$0.35 & $1.41\pm$0.44 & $5.66\pm$2.09 & $7.66\pm$2.40 & $3.47\pm$1.18 & $9.16\pm$2.95 & $1.54\pm$0.54\\
        & & & 0.164 & 0.70 & 4.38 & 36.9 & 9.2\\
        \hline
        P10 & 18:42:47.860 & -4:03:08.458 & 0.171 & 0.73 & 4.58 & 38.5 & 9.6 & 13.6 & $6.43\pm$1.98 & $2.05\pm$0.75 & $1.36\pm$0.42 & $5.45\pm$2.01 & $1.40\pm$0.36 & $4.45\pm$1.45 & $1.47\pm$0.46 & $1.88\pm$0.59 & $7.54\pm$2.80 & $10.00\pm$3.32 & $4.32\pm$1.49 & $9.94\pm$3.21 & $1.93\pm$0.67\\
        & & & 0.116 & 0.50 & 3.11 & 26.1 & 6.5\\
        \hline
        \hline
    \end{tabular}
  \end{adjustbox}
  \vspace*{1mm}
  \caption{Estimated physical properties and molecular abundances observed by IRAM 30m towards IRDC G28.37+00.0, at 10 different positions.}
  \label{tab:landscape-tab}
  
\end{table}
\end{landscape}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


From the two mass surface density maps shown in Figure~\ref{fig:sigma_T_map}, we have measured the average values of $\Sigma_{\rm MIREX}$ and $\Sigma_{\rm sub-mm}$ in each of the ten regions P1 to P10 (see Table~\ref{tab:landscape-tab}). This also allows an estimate of $N_{\rm H}$, assuming a mass per H of $\mu_{\rm H}=1.4 m_{\rm H} = 2.34\times 10^{-24}\:$g (i.e., approximately due to $n_{\rm He}=0.1 n_{\rm H}$ and ignoring contributions from other species). We assume an uncertainty of $\sim$30\% in the measurements of $\Sigma$ and $N_{\rm H}$ \citep{2013A&A...549A..53K,lim2016distribution}.

We have then estimated the average total amount of visual extinction, $A_V$, through each region using the standard dust model assumptions of \cite{2013A&A...549A..53K}, i.e.,
%By using Equation 4 in \cite{2013A&A...549A..53K}, we have used the N(H) measurements to calculate the visual extinction level, A$_v$, at each position:
\begin{equation}
   N_{\rm H} = 1.9\times 10^{21} \: {\rm cm}^{-2} \:\left(\frac{A_{V,{\rm tot}}}{\rm mag}\right).
   \label{eq:N_av}
\end{equation}
However, we then divide this estimate of the total extinction through the region by a factor of 4 in order to obtain an estimate of the typical extinction from the nearest boundary of the IRDC, i.e., $\bar{A}_V=A_{V,{\rm tot}}/4$.



%we have measured the dust temperature T, Hydrogen column density, N(H), Hydrogen volume density n(H), and visual extinction, A$_v$, toward the ten positions across cloud C.

%For each position, we obtained the mass surface density, $\Sigma$, as the mean value within a beam aperture, calculated across all pixels within a beam. Hence, we have converted the obtained $\Sigma$ values into Hydrogen column density values, N(H), using Equation 5 in \cite{2013A&A...549A..53K}:
%\begin{equation}
 %   \Sigma_{\rm H} = 1.4\rm m_{H}\rm N_{H}
  %  \label{rel:Hydrogen density}
%\end{equation}
%where, m$_{H}$ is the Hydrogen mass ($1.6735\times 10^{-24} g$) and the 1.4 factor takes into account a 40$\%$ helium contribution to the column density (implying the H:He number ratio of 10:1).\\

We have estimated the average number density of H nuclei, $n_{\rm H}$, in each region by assuming the material is distributed in a spherical volume with radius equal to the circular aperture radius of the region projected on the sky. These values are also listed in Table \ref{tab:landscape-tab}.

%converted the Hydrogen column density N(H) into Hydrogen volume density, n(H), assuming that the Hydrogen nuclei are distributed in a sphere of the same radius of the beam aperture. The obtained values of $\Sigma$, N(H) and n(H) are listed in Table \ref{tab:physical_parameters_IRDC}.\\

Finally, by using the dust temperature map from \cite{lim2016distribution}, we have estimated the $\Sigma$-averaged $T$ values for the ten selected positions.
These values are also listed in Table \ref{tab:landscape-tab}. The uncertainties in $T$ are assumed to be at the level of $30\%$ \citep{lim2016distribution}.

%Toward each position, we have measured the mean weighted T , averaged across the pixels within the 32$^{\prime\prime}$ beam aperture and using as weight the corresponding $\Sigma$ value at that pixel (we note that the two maps have the same pixel size and shape).\\

%The obtained values of $\Sigma_{\rm H}$, T, N(H), n(H) and A$_v$ are listed in Table \ref{tab:physical_parameters_IRDC}. For the $\Sigma_{\rm H}$ and T measurements, we have assumed an uncertainty of $\sim$30\% \citep{2013A&A...549A..53K,lim2016distribution} and calculated the uncertainty in the other quantities following statistical error propagation rules. 

%\input{chapters/molecular_abundances}

\subsection{Molecular Abundances}

%All spectra have been extracted over a beam-aperture of 32$^{\prime\prime}$ HPBW, corresponding to the poorest angular resolution for the observed transitions (81.5 GHz). In some cases, spectra were smoothed to improve the signal-to-noise- ratio and the final velocity resolution of the lines are reported in Table~\ref{tab:modelcules_parameters_Ntot}.

We now estimate column densities of the nine observed species listed in Table~\ref{tab:modelcules_parameters_Ntot} in the 10 regions of the IRDC and use these results to calculate their abundances with respect to the total H nuclei, i.e., $N_X/N_H$. For the column density estimation we have used Equation A4 of \cite{caselli2002molecular}:
% \begin{equation}
 \begin{eqnarray}
 %\begin{split}
  N_{X} & = & \frac{8 \pi \nu^{2}}{A g_{u}c^{3}}\frac{k}{h} \frac{1}{J_{\nu}(T_{\rm ex})-J_{\nu}(T_{\rm bg})}\nonumber\\
     & \times & \frac{Q_{\rm rot}}{1-{\rm exp} (\frac{-h\nu}{kT_{\rm ex}})} \frac{1}{{\rm exp}(\frac{-E_{L}}{kT_{\rm ex}})} \int T_{\rm mb} dv,
     \label{rel:N_tot}
 %\end{split}
\end{eqnarray}
% \end{equation}
where $\nu$ is the frequency of the observed transition, $A$ is the Einstein coefficient obtained from the CDMS catalog\footnote{https://cdms.astro.uni-koeln.de/classic/}, $g_{u}=2J+1$ is the statistical weight of the upper level, $E_{L}$ is the energy of the lower level, and
%in unit of temperature (K), 
$J_{\nu}(T_{\rm ex})$ and $J_{\nu}(T_{\rm bg})$ are the %Rayleigh-Jeans 
excitation and background temperatures, respectively. For these we set $T_{\rm ex}$= 7.5 K based on the multi-transition CO study of an IRDC by \cite{hernandez2012virialized}, while $T_{\rm bg}$=2.73 K from the CMB. Finally, $Q_{\rm rot}$ is the rotational partition function at the assumed $T_{\rm ex}$. For each molecule, $Q_{\rm rot}$ has been calculated by fitting its values from JPL catalogue, except in the case of N$_2$H$^+$ and HCN for which, since their main rotational transitions split into hyperfine components, the partition function reported in the JPL catalogue includes an additional factor and it does not coincide with the pure rotational partition function. Hence, for N$_2$H$^+$ and HCN, we have calculated Q$_{\rm rot}$ as:
\begin{equation}
 %\begin{split}
  Q_{\rm rot} = \sum_{J=0}^{\infty} (2J+1) {\rm exp} \left(\frac{-E_{J}}{kT}\right),
  \label{rel:Q_rot}
 %\end{split}
 \end{equation}
where, $E_{J}=J(J+1)hB$ is the energy of the $J$ level and $B$ is the rotational constant of the molecule.
The various parameters used to derive the abundances of the species are listed in Table \ref{tab:modelcules_parameters_Ntot}.
Finally, we note that $N_{\rm N_2H^+}$ and $N_{\rm HCN}$ obtained from Equation~\ref{rel:N_tot} have been corrected for the transition statistical weights of 0.11 and 0.3333, respectively, since only one of the hyperfine lines was used in each case to derive total abundances. %to take into account the presence of hyperfine structures, i.e., $\approx$ 0.11 for N$_2$H$^+$ \citep{henshaw2014dynamical} and $\approx$ 0.3333 for HCN. All used spectroscopic quantities are reported in Table \ref{tab:modelcules_parameters_Ntot}.

In deriving column densities from the observed spectra, which are shown in Figures~\ref{fig:spectra_A} and \ref{fig:spectra_B}, we must make a choice of the velocity range over which to integrate the line intensities. From inspection of the spectra, this range is chosen to have a common extent of 77 to 82 km~s$^{-1}$, motivated by the goal of covering the dense gas tracers of $\rm H^{13}CO^+(1-0)$, $\rm HC^{18}O^+(1-0)$ and $\rm N_2H^+(1-0)$. Examining the spectra of Figures~\ref{fig:spectra_A} and \ref{fig:spectra_B}, we see that C$^{18}$O(1-0) generally shows emission from several components that span a broader velocity range than the above dense gas tracers. In our analysis, we will only measure the CO column density from the part of C$^{18}$O(1-0) emission that falls in the velocity range from 77 to 82 km~s$^{-1}$.

%Looking at the spectra of C$^{18}$O, H$^{13}$CO$^{+}$, HC$^{18}$O$^{+}$  and N$_2$H$^+$ (Figures~\ref{fig:spectra_A} and \ref{fig:spectra_B}) for all positions, the C$^{18}$O emission likely shows multiple velocity components and shows a broader velocity range compared to the other species. Due to the ubiquitousness of CO along the line of sight, the CO abundance may be overestimated. On the other hand, H$^{13}$CO$^{+}$, HC$^{18}$O$^{+}$ and N$_2$H$^+$ show much narrower line widths. Thus, comparing the velocities of H$^{13}$CO$^{+}$, HC$^{18}$O$^{+}$ and N$_2$H$^+$ transition and choosing the narrowest range of velocity (77-82 km.s$^{-1}$), mostly based on N$_2$H$^+$ spectra, extracted abundance are demonstrated in Table \ref{tab:abundances}.\\

%We estimated the area under the curve of all spectra, in the range of 77-82 km.s$^{-1}$. Since resolution of the spectra is different for each molecule, we defined a condition for the channels chosen in 77-82 km.s$^{-1}$. For lower boundary (77 km.s$^{-1}$), if the central velocity of the channel (V$_c$) is bigger than 77 (V$_c$ > 77), the channel is included to calculate the area of the spectrum, otherwise it is excluded. For upper boundary (82 km.s$^{-1}$), if the central velocity of the channel is smaller than 82 (V$_c$ < 82), the channel is included, otherwise is excluded.\\

To estimate the uncertainties in the total column densities, we consider the following factors. First is the uncertainty in the integrated intensity of each line, which we assess to be equal to the noise integrated in a line-free spectral range and calculated as:
\begin{equation}
    %\sigma_{area}=\sqrt{\rm N}\times rms \times dv,
    \int T_{\rm mb,noise} dv = \sqrt{n} \Delta T_{\rm mb,noise} dv
    \label{rel:Uncertainty}
\end{equation}
where $n$ is the number of channels, each of velocity width $dv$, that are summed in the integration and $\Delta T_{\rm mb,noise}$ is the noise in an individual channel.

Second is the systematic uncertainty due to the need to assume a value of $T_{\rm ex}$. We note that $T_{\rm ex}=7.5\:$K has been adopted for all the species. If $T_{\rm ex}$ is varied by $\pm30\%$ about this value, the estimated total column density changes by $\sim 7-28\%$. For most species, this systematic error dominates over that due to the noise in the integrated intensity. In our analysis, we estimate the overall uncertainty in total column densities by summing the above two sources of uncertainties in quadrature. However, we note that there are other potential sources of systematic error, such as the assumption that the emission in the particular chosen velocity range is a good representation of the physical component of the molecular cloud that is being modelled.

For some of the species, like CO, $\rm HCO^+$ and HNC, the column density is estimated by conversion from a rarer isotopologue. This involves another source of systematic uncertainty. For these conversions, we assume $\rm [^{12}C]/[^{13}C]=40.2\pm 8.0$ \citep{zeng201715n} and $\rm [^{16}O]/[^{18}O]=318\pm 64$ \citep{hezareh2008simultaneous} and these levels of uncertainty are also propagated in quadrature for the final column density estimate.

We note that, since no significant signal is detected for the HC$^{18}$O$^{+}$(1-0) transition toward the positions p6, p7, p8, p9, and p10, we have estimated their HC$^{18}$O$^{+}$ column density from the average of their spectra. Then, we have apportioned this column density among the five positions in proportion to their H column densities.

%divided obtained value by the average Hydrogen column density toward the five positions p6-p10. The obtained HC$^{18}$O$^{+}$ abundance has been used for the 5 positions, p6 to p10.

%The CO and HCO$^+$ molecular abundances have been obtained by converting the abundances of C$^{18}$O and H$^{13}$CO$^{+}$ (or HC$^{18}$O$^{+}$) respectively. 

The final step of the analysis is to estimate abundances of species with respect to H nuclei that are assumed to be present in the same molecular cloud component. For this we simply divide the above estimates of total species column density by the estimate of H nucleus column density obtained previously either via {\it Herschel}-observed sub-mm dust emission or via MIR extinction. Each of these methods is assumed to have a 30\% uncertainty, which is summed in quadrature for the final abundance estimate. The obtained results are summarised in Table \ref{tab:landscape-tab}. Note, the H column densities obtained by both methods are themselves quite similar (see above) and, for simplicity, in the remaining analysis we will adopt those estimates based on the sub-mm dust continuum emission.

%Finally, we have obtained molecular abundances, as the ratio between molecular and hydrogen column density, at each position and for each molecule. 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
    \centering
    %\includegraphics[width=\textwidth]{chapters/images/both_maps_16_arsec.pdf}
    %\addtolength{\leftskip} {-3.1cm}
    %\addtolength{\rightskip}{-1.5cm}
     \includegraphics[height=25cm,width=15cm,]{chapters/images/spectra_A.pdf}
    \vspace*{-21mm}
    \caption{Spectra of observed species at positions p1-p5. The dashed lines indicate the velocity range 77 to 82 km~s$^{-1}$, which has been selected to cover the dense gas as traced by N$_2$H$^+$ and H$^{13}$CO$^+$. 
    {\bf JCT - There is some mistake here in the description, I think.}
    {\bf NE In the left-side panels}, the signals of species are amplified by three times, except C$^{18}$O.} 
    \label{fig:spectra_A}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
    \centering
    %\includegraphics[width=\textwidth]{chapters/images/both_maps_16_arsec.pdf}
    %\addtolength{\leftskip} {-3.1cm}
    %\addtolength{\rightskip}{-1.5cm}
     \includegraphics[height=25cm,width=15cm,]{chapters/images/spectra_B.pdf}
    \vspace*{-21mm}
    \caption{Spectra of observed species at positions p6-p10. The dashed lines indicate the narrower range of velocity 77-82 km.s$^{-1}$ which has been selected based on the spectra of N$_2$H$^+$ and H$^{13}$CO$^+$. In the left-side panels, the signals of species are amplified by three times, except C$^{18}$O.} 
    \label{fig:spectra_B}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Spectra of ch3oh, hcn, hnc, h2co and hnco

%\begin{figure*}
    %\centering
    %\includegraphics[width=\textwidth]{chapters/images/both_maps_16_arsec.pdf}
    %\addtolength{\leftskip} {-4.5cm}
    %\addtolength{\rightskip}{-1.cm}
     %\includegraphics[height=25cm,width=15cm,]{chapters/images/remaining_spectra.pdf}
    %\vspace*{-21mm}
    %\caption{Spectra of CH$_3$OH, H$_2$CO, HN$^{13}$C, HCN and HNCO at all positions. The dashed lines indicates the narrower range of velocity 77-82 km.s$^{-1}$ which has been selected based on the spectra of N$_2$H$^+$ and H$^{13}$CO$^+$}. 
    %\label{fig:remaining_spectra}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%To obtain the velocity range of the detected signal, first the line peak velocity is identified. Then, the line is integrated at blue (lower) and red-shifted (higher) velocities until the lowest positive temperature is reached.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Results}
\label{S:results}

\subsection{Abundances, including density dependence}

Here we summarise the abundances of the various species obtained in the IRDC positions (see also Table~\ref{tab:landscape-tab}). For CO, we find a typical value of ${\rm [CO]} \equiv N_{\rm CO}/N_{\rm H} \sim 2 \times 10^{-5}$, which corresponds to a CO depletion factor of $f_D\sim7$. In Figure~\ref{fig:fd_n}a we plot $f_D$ versus $n_{\rm H}$, which reveals a trend of increasing depletion factor (i.e., smaller gas phase CO abundance) with increasing density. While correlated uncertainties are present in the measurements of $f_D$ and $n_{\rm H}$ (estimated via $N_{\rm H}$), the trend is significant, given a Pearson correlation coefficient of $r=0.93$. ({\bf some check here from Negar, Giuliana on this description.})
%jct - Pearson correlation coefficient?
For completeness, the same information about the trend of [CO] with $n_{\rm H}$ is also shown in Figure~\ref{fig:species_nH}a.

Theoretically, for a given set of conditions including cloud age, one expects higher CO depletion factors at higher densities, i.e., due to higher rates of freeze-out leading to shorter freeze-out timescales. To illustrate this quantitatively, Figure~\ref{fig:fd_n}a shows some example models of the time evolution of $f_D$ versus $n_{\rm H}$, with other parameters set to values of $T=15\:$K, $A_V=10\:$mag, and two values of $\zeta=10^{-18}$ and $10^{-16}\:{\rm s}^{-1}$ explored. The observed trend of $f_D$ versus $n_{\rm H}$ can be explained by a model in which the 10 positions have fairly similar ages of $2\times 10^5\:$yr. We note that this result is quite insensitive to certain choices of the astrochemical models, such as $\zeta$, $A_V$ (for values $>5\:$mag) and $T$ (for values $<20\:$K).

%(see Fig.~\ref{fig:fd_n}b {\bf NE:dotted line}) and $A_V$ (see Fig.~\ref{fig:fd_n}c {\bf NE:dashed-dotted line}).

Figure~\ref{fig:fd_n}b plots $f_D$ versus $\bar{A}_{V}$. While we see a trend of increasing observed $f_D$ versus $\bar{A}_{V}$, we note that $\bar{A}_{V}\propto N_{\rm H} \propto n_{\rm H}$. At a given age and volume density, the astrochemical models do not predict a significant variation of $f_D$ with $A_V$ (at least for $A_V>5\:$mag, which is the relevant range). Thus, we consider that trend we observe here is more likely to be caused by variations in density in the regions.

%Note, that the measurements that deviate from this value by the largest amount are still consistent with it, given the uncertainties. However, there is a slight trend for higher CO depletion factors to be found in regions P1 to P5. These regions have higher measured values of $N_{\rm H}$ and $n_{\rm H}$ compared to the other regions (see Table~\ref{tab:landscape-tab}), so this could indicate a systematic increase in $f_D$ with $n_{\rm H}$  



%{\bf NE:, which is consistent with the results of theoretical model shown in panel a of Figure~\ref{fig:fD_values_15K}}. We plot $f_D$ versus $n_{\rm H}$ in Figure~\ref{fig:fd_n}.{\bf NE: In figure~\ref{fig:fd_n}, the parameters of the fiducial model have been chosen for the remaining parameters. As it is indicated in relation~\ref{eq:N_av}, due to a correlation between $N_H$ and $A_v$, we see in panel b of Figure~\ref{fig:fd_n} that as $A_v$ increases, $f_D$ is raised up as well. Exploring the effects of other parameters indicated in Figures~\ref{fig:fd_n_CRIR} and \ref{fig:fd_n_av}, shows that $f_D$ is not very sensitive to $\zeta$ and $A_v$, for the time between 1.0e5-1.0e7 years, which is also obvious from panel c and d of Figure~\ref{fig:fD_values_15K}. But exploring varying of density indicated in Figure~\ref{fig:fd_av_n}, shows that as $n_H$ decreases, $f_D$ is decreased and observed $f_D$s tend to match with the models with older ages. The only Dependency of abundance on $n_H$ is detected for $f_D$ ([CO]) which is positively correlated to $n_H$ with correlation parameter r = 0.93, and for other species there is not a significant correlation (r<0.8) (Figure~\ref{fig:species_nH}). }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{chapters/images/fd_n.pdf}
\vspace*{-5mm}
\caption{{\it (a) Left:} CO depletion factor ($f_D$) versus number density of hydrogen nuclei ($n_{\rm H}$). The data for each position are shown, along with their uncertainties. Astrochemical models are shown for ages ranging from $10^5\:$yr to $10^7\:$yr and for $\zeta= 10^{-18}\:{\rm s}^{-1}$ (dotted lines) and $10^{-16}\:{\rm s}^{-1}$ (solid lines), with other parameters set to be $T=15\:$K and $A_V=10\:$mag.
%
{\it (b) Right:} CO depletion factor ($f_D$) versus visual extinction ($A_V$). The data for each position are shown, along with their uncertainties. Astrochemical models are shown here for $n_{\rm H}=10^{5}\: {\rm cm}^{-3}$, $T=15\:$K and $\zeta=10^{-16}\:{\rm s}^{-1}$ {\bf (solid lines), and $n_{\rm H}=10^{4}\: {\rm cm}^{-3}$ (dotted lines)}.}
     \label{fig:fd_n}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[!ht]
%\centering
     %\addtolength{\leftskip} {-8cm}
    %\addtolength{\rightskip}{-8.5cm}
     \hspace{-2cm}
    \includegraphics[width=1.2\textwidth]{chapters/images/allspecies_vs_n.pdf}
     \vspace*{-8mm}
     \caption{Observed abundances of (a) CO, (b) HCO$^+$, (c) $\rm N_2H^+$, (d) HCN, (e) HNC, (f) HNCO, (g) H$_2$CO and (h) $\rm CH_3OH$ versus $n_{\rm H}$. Astrochemical model results are also shown for $\zeta= 10^{-18}\:{\rm s}^{-1}$ (dotted lines) and $10^{-16}\:{\rm s}^{-1}$ (solid lines), with other parameters set to be $T=15\:$K and $A_V=10\:$mag.}
     \label{fig:species_nH}
 \end{figure*}


%with 37$\%$ uncertainty in all positions except P6, with relatively higher abundance at starless positions (p7-p10). As it can be seen from Figure\ref{fig:sigma_T_map}, and estimated in table~\ref{tab:physical_parameters_IRDC} as well, P2 is located in the center of mass condensation and it contains the highest Hydrogen volume density. Estimated CO abundance at P2 is 1.37$\times$ 10$^{-5}$, which is the lowest value with respect to the other regions which consequently implies that at P2, we see the higher value of CO depletion factor ($\simeq$ 10). Contrariwise, at P6 that we see the lowest Hydrogen density, the highest CO abundance is estimated. It can be said that as hydrogen density reduces, CO abundance increases.

%... discussion of the estimated abundances and the implied CO depletion factors... is there any trend of CO depletion factor with density, T, spatial location in the IRDC?


For HCO$^+$, using emission from H$^{13}$CO$^+$ we infer typical abundances of [HCO$^+$]~$\sim 4 \times 10^{-10}$. The abundances inferred from  HC$^{18}$O$^+$ are systematically larger by about 30$\%$. However, such a difference is within the isotopologue ratio uncertainties. While the two lowest density regions, P6 and P10, are seen to have the highest abundances, $\sim 6 \times 10^{-10}$, the overall correlation with density is not as strong as in the case of [CO] (see Figure~\ref{fig:species_nH}b).

%As examples, we estimated [HCO$^+$]~$\sim 4 \times 10^{-10}$ 
%with $\sim$ 37$\%$ uncertainty obtained 
%from H$^{13}$CO$^+$, with the highest abundance at P6 and the lowest one at P8.

%and 6~$\times$ 10$^{-10}$ with $\sim$ 40$\%$ uncertainty obtained from HC$^{18}$O$^+$. 

We estimate [N$_2$H$^+$] $\sim 10^{-10}$ on average (see Figure~\ref{fig:species_nH}c). Again, the lowest density region has the highest abundance, but, as with HCO$^+$, there is no significant trend with density. Similar results are seen for HCN, with typical abundance of [HCN]~$\sim 10^-{10}$ (Fig.~\ref{fig:species_nH}d), and HNC, with typical abundance of $6\times 10^{-10}$ (Fig.~\ref{fig:species_nH}e).

Finally, we find [HNCO]$\sim 3\times 10^{10}$, [H$_2$CO]$\sim 5\times 10^{-11}$ and [CH$_3$OH]$\sim 10^{-9}$ as typical values. Here there are hints of a bifurcation in the regions, with P1, P6, P7 and P8 having relatively low values, and the other six regions having abundances that are several times larger. 

We note that P7 and P8 were specifically chosen to be in regions that are relatively quiescent with respect to star formation activity as traced by CO(2-1) outflows (Kong et al. 2019), while still containing relatively dense structures. P1 also includes the candidate C1-N and S massive pre-stellar cores (Tan et al. 2013), i.e., significant quantities of dense, quiescent gas, although there are two protostellar sources (C1-Sa and C1-Sb) also in the region. P6 also appears to be quiescent, e.g., not containing a $70\:{\rm \mu m}$ detected protostar (Moser et al. 2020), but is outside the region mapped for CO(2-1) outflows. Thus, we tentatively conclude that regions with relatively low star formation activity also have relatively low abundances of the relatively complex species of HNCO, H$_2$CO and CH$_3$OH. Such a result could be due to requirement of protostellar warming or outflow shock activity to liberate these species efficiently from dust grain ice mantles.



%We estimated [N$_2$H$^+$] approximately 2~$\times$ 10 $^{-10}$, with approximately 30$\%$ uncertainty. The highest [N$_2$H$^+$] has been estimated at P6, the less dense region and the lowest abundance has been estimated at P1, the coldest region.

%For other species, the abundances with~30-35$\%$ uncertainties, are varied from position to positions. for HNC and HCN, the highest abundance has been estimated at P6. Although for HNCO, CH$_3$OH and H$_2$CO, relatively lower abundances has been estimated at P6, the highest abundance of HNCO and and H$_2$CO has been estimated at P2.

%It is clear that, at p2 with the highest volume density and P6 with the lowest hydrogen density, we see outstanding values of abundances which are related to the the properties of these positions.


%... typical value and dispersion? Which region has highest/lowest abundance.

%Follow similar pattern for other species... does any region stand out?... 

\subsection{Astrochemical Implications for Cosmic Ray Ionization Rate and Cloud Age}

In this section we use the abundance measurements of the IRDC positions to constrain conditions in the clouds, especially $\zeta$ and $t$, via the astrochemical models described in \S\ref{astrochemical_model}. In general we will compare a set of the observed abundances, $[X_i]_{\rm obs}$, in a given position with those of theoretical model abundances, $[X_i]_{\rm theory}$. We will search the model grid parameter space $(n_{\rm H}, T, A_V, \zeta, t)$ to minimize a $\chi^2$ metric of the following form
\begin{equation}
    \chi^2=\sum_i W_i [({\rm log}_{10} [X_i]_{\rm obs} - {\rm log}_{10} [X_i]_{\rm theory}) / {\rm log}_{10}(\sigma_i)]^2,
    \label{rel:chi-square}
\end{equation}
where $\sigma_i$ is an estimate of the uncertainty in the abundance, including the basic observational uncertainty and any allowed theoretical model uncertainty, and $W_i$ is a weighting factor, which allows certain species to be given greater or lesser importance in the analysis.


%Below we describe the method used to identify the model that best reproduces the observed molecular abundances and that provides us with an estimate of the cosmic ionization rate across the ten positions. For each positions, the best model is considered the one that minimizes the reduced $\chi^2$ in logarithmic scale, defined as:\\

%where \textit{X[obs]} and \textit{X[model]} refers to the abundances of the observed and astrochemical model data respectively and \textit{X[obs]$_{error}$} is the uncertainty of the observed abundances.\\


As first step, we only consider the abundances of CO, HCO$^+$ (obtained from H$^{13}$CO$^+$) and N$_2$H$^+$, i.e., CO and the two molecular ions in our set of species. 
%
We have first searched the entire model grid parameter space to find best fitting models and map out the $\chi^2$ landscape.
However, unrealistic solutions can be found with low values of $\chi^2$, e.g., at high temperatures ($\gtrsim 500\:$K), where low values of [CO] are matched by gas-phase chemical processing of the CO, rather than by CO freeze out onto dust.
%
Thus, we focus on a restricted (R) search over the ranges: $n_{\rm H} = 10^4 - 10^6\: {\rm cm}^{-3}$; $T= 10 - 50\:$K and $A_V = 5 - 100\:$mag. We also consider ultra-restricted (UR) searches in which $n_{\rm H}$ and $A_V$ are set to the closest values in the model grid to those of the observed region and with only adjacent values also considered. For this UR case we limit the search to $T=10 - 20\:$K. Finally, we have an extreme-restricted (XR) case where we only search the $\zeta$-$t$ parameter space in the best physically matched model for $n_{\rm H}$, $A_V$ and $T$ (note, in this case we always set $T=15\:$K: this is always the closest match, except for P1, where $T=11.8\:$K, but even here for simplicity we will consider 15~K for the XR case).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htb!]
    \centering
    \addtolength{\leftskip} {-1.2cm}
    \addtolength{\rightskip}{-1cm}
     \includegraphics[width=20cm, height=16cm]
     {chapters/images/p2_n_T.pdf}
     \vspace*{-14mm}
     \caption{$\chi^2$ landscape in the $n_{\rm H}$ versus $t$ plane for Extra-restricted (XR) fitting of the abundances of CO, HCO$^+$ and N$_2$H$^+$ at the P2 position. For these models, $A_{\rm v}$ has been set to be 20~mag and the location of the minimum $\chi^2$ has been marked with a white cross.}
     \label{fig:p2_n_T}
 \end{figure*}


\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-2.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_case1_XR.pdf}
     \vspace*{-6mm}
     \caption{Evolution of the main species, in the best models shown in the central panels of Figure~\ref{fig:p2_n_T}. The density of the models is $n_{\rm H}$=1.0e5 cm$^{-3}$ and $A_{\rm v}$ = 20 mag. $\zeta$ of the best models has been marked with a white  and black crosses in the location of minimum $\chi^2$. The same locations have been shown with colored crosses at each panel of the evolution of the species. The dotted colored lines show the gas phase and solid lines the grain phase of the species. In the panel of [CO], colored solid lines show the C-bearing species with the highest amount of C, at each model. The horizontal band indicates observed species with associated uncertainties.}
     \label{fig:p2_n_T_evolution}
 \end{figure*} 
 
 
 
 \begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-2.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_case1_4.pdf}
     \vspace*{-6mm}
     \caption{Evolution of the main species, in the best model shown in the central panels of Figure~\ref{fig:p2_n_T}, showing for T=15 and 10~K.The density of the models is $n_{\rm H}$=1.0e5 cm$^{-3}$ and $A_{\rm v}$ = 20 mag. $\zeta$ of the best models has been marked with a white crosses in the location of minimum $\chi^2$. The same locations have been shown with colored crosses at each panel of the evolution of the species. The dotted colored lines show the gas phase and solid lines the grain phase of the species. The horizontal band indicates observed species with associated uncertainties.}
     \label{fig:p2_n_T_evolution_10K}
 \end{figure*}
 
 
 \begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-2.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_case1_7.pdf}
     \vspace*{-6mm}
     \caption{Evolution of the main species, in the best model shown in the central panels of Figure~\ref{fig:p2_n_T}, showing for T=15 and 20~K.The density of the models is $n_{\rm H}$=1.0e5 cm$^{-3}$ and $A_{\rm v}$ = 20 mag. $\zeta$ of the best models has been marked with a white crosses in the location of minimum $\chi^2$. The same locations have been shown with colored crosses at each panel of the evolution of the species. The dotted colored lines show the gas phase and solid lines the grain phase of the species. The horizontal band indicates observed species with associated uncertainties.}
     \label{fig:p2_n_T_evolution_20K}
 \end{figure*}
 
 
 
 
 \begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-2.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_case1_2.pdf}
     \vspace*{-6mm}
     \caption{Evolution of the main species, in the best model shown in the central panel of Figure~\ref{fig:p2_n_T}, as well as two other models with higher and lower CRIR. The density of the models is $n_{\rm H}$=1.0e5 cm$^{-3}$, $A_{\rm v}$ = 20 mag and T=15~K. $\zeta$ of the best model has been marked with a white cross in the location of minimum $\chi^2$. The same locations have been shown with colored crosses at each panel of the evolution of the species. The horizontal band indicates observed species with associated uncertainties.}
     \label{fig:p2_n_T_evolution_high_low_CRIR}
 \end{figure*}
 
 
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htb!]
    \centering
    \addtolength{\leftskip} {-1.2cm}
    \addtolength{\rightskip}{-1cm}
     \includegraphics[width=20cm, height=16cm]
     {chapters/images/p2_n_T_case2.pdf}
     \vspace*{-14mm}
     \caption{$\chi^2$ landscape in the $n_{\rm H}$ versus $t$ plane for Extra-restricted (XR) fitting of the abundances of all observed species, at the P2 position. For these models, $A_{\rm v}$ has been set to be 20~mag and the location of the minimum $\chi^2$ has been marked with a black cross.}
     \label{fig:p2_n_T_case2}
 \end{figure*}
 
 
 
\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_XR_case2.pdf}
     \vspace*{-7mm}
     \caption{Evolution of the all species, in the best models indicated in the middle panel of Figure~\ref{fig:p2_n_T_case2}. The density of the models is $n_{\rm H}$=1.0e5 cm$^{-3}$ and $A_{\rm v}$ = 20 mag. $\zeta$ of the best models has been indicated with black cross at each panel in Figure~\ref{fig:p2_n_T_case2}. The colored crosses at each panel shows the location of the minimum $\chi^2$  at each model. The dotted colored line indicates gas phase species and the straight lines in the panel of [CO], shows the grain C-bearing species at each model with the highest amount of C. The horizontal band indicates observed species with associated uncertainties at P2.}
     \label{fig:p2_n_T_evolution_case2}
 \end{figure*}  
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htb!]
    \centering
    \addtolength{\leftskip} {-1.2cm}
    \addtolength{\rightskip}{-1cm}
     \includegraphics[width=20cm, height=16cm]
     {chapters/images/p6_n_T.pdf}
     \vspace*{-14mm}
     \caption{$\chi^2$ landscape in the $n_{\rm H}$ versus $t$ plane for Extra-restricted (XR) fitting of the abundances of CO, HCO$^+$ and N$_2$H$^+$, at the P6 position. For these models, $A_{\rm v}$ has been set to be 7~mag and the location of the minimum $\chi^2$ has been marked with a white cross.}
     \label{fig:p6_n_T_case1}
 \end{figure*}
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p6_case1_XR.pdf}
     \vspace*{-7mm}
     \caption{Evolution of the main species, in the best models shown in the central panels of Figure~\ref{fig:p6_n_T_case1}. The density of the models is $n_{\rm H}$=4.6e4 cm$^{-3}$ and $A_{\rm v}$ = 7 mag. $\zeta$ of the best models has been marked with a white and black crosses in the location of minimum $\chi^2$. The same locations have been shown with colored crosses at each panel of the evolution of the species. The dotted colored lines show the gas phase and solid and dashed-dotted lines the grain phase of the species. In the panel of [CO], colored solid lines show the C-bearing species with the highest amount of C, at each model. The horizontal band indicates observed species with associated uncertainties.}
     \label{fig:p6_n_T_evolution_case1}
 \end{figure*}  



\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p6_case1_10K.pdf}
     \vspace*{-7mm}
     \caption{Evolution of the main species, in the best model shown in the central panels of Figure~\ref{fig:p6_n_T_case1}, showing for T=15 and 10~K.The density of the models is $n_{\rm H}$=4.6e4 cm$^{-3}$ and $A_{\rm v}$ = 7 mag. $\zeta$ of the best models has been marked with crosses in the location of minimum $\chi^2$. The same locations have been shown with colored crosses at each panel of the evolution of the species. The dotted colored lines show the gas phase and solid lines the grain phase of the species. The horizontal band indicates observed species with associated uncertainties.}
     \label{fig:p6_n_T_evolution_case1_10K}
 \end{figure*} 


\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p6_case1_20K.pdf}
     \vspace*{-7mm}
     \caption{Evolution of the main species, in the best model shown in the central panels of Figure~\ref{fig:p6_n_T_case1}, showing for T=15 and 20~K.The density of the models is $n_{\rm H}$=4.6e4 cm$^{-3}$ and $A_{\rm v}$ = 7 mag. $\zeta$ of the best models has been marked with a white crosses in the location of minimum $\chi^2$. The same locations have been shown with colored crosses at each panel of the evolution of the species. The dotted colored lines show the gas phase and solid lines the grain phase of the species. The horizontal band indicates observed species with associated uncertainties.}
     \label{fig:p6_n_T_evolution_case1_20K}
 \end{figure*} 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htb!]
    \centering
    \addtolength{\leftskip} {-1.2cm}
    \addtolength{\rightskip}{-1cm}
     \includegraphics[width=20cm, height=16cm]
     {chapters/images/p6_n_T_case2.pdf}
     \vspace*{-14mm}
     \caption{$\chi^2$ landscape in the $n_{\rm H}$ versus $t$ plane for Extra-restricted (XR) fitting of the abundances of all observed species, at the P6 position. For these models, $A_{\rm v}$ has been set to be 7~mag and the location of the minimum $\chi^2$ has been marked with a black cross.}
     \label{fig:p6_n_T_case2}
 \end{figure*}


\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p6_XR_case2.pdf}
     \vspace*{-8mm}
     \caption{Evolution of the all species, in the best models indicated in the middle panels of Figure~\ref{fig:p6_n_T_case1}. The density of the models is $n_{\rm H}$=4.6e4 cm$^{-3}$ and $A_{\rm v}$ = 7 mag. $\zeta$ of the best models has been indicated with black crosses at each panel in Figure~\ref{fig:p6_n_T_case2}. The colored crosses at each panel shows the location of the minimum $\chi^2$  at each model. The dotted colored line indicates gas phase species and the straight lines in the panel of [CO], shows the grain C-bearing species at each model with the highest amount of C. The horizontal band indicates observed species with associated uncertainties at P6.}
     \label{fig:p6_n_T_evolution_case2}
 \end{figure*}  
 





Examples of the $\chi^2$ landscape in the $\zeta$ versus $t$ plane are shown in Figure~\ref{fig:p2_n_T} for UR fitting of [CO], [HCO$^+$] and [N$_2$H$^+$] of the P2 position. These nine panels are centered around the case with $n_{\rm H}=2.2\times10^4\:{\rm cm}^{-3}$ {\bf I recreated the image, now the central n(H)=1.0e5} and $T=15\:$K (with the other main variable of $A_V$ set equal to 20~mag for all nine panels). Then in each panel we see which values of $\zeta$ and $t$ give relatively low values of $\chi^2$, with values of $\chi^2<30$ illustrated via the color scale.

We notice several main features in the results of Figure~\ref{fig:p2_n_T}. First, the best result in the central panel that is best matched to the physical conditions of P2 has $\zeta=???8\times 10^{-19}\:{\rm s}^{-1}$ ({\bf 2.2e-18 s-1})and $t=???9\times10^5\:$yr ({\bf 2.00e5 yr}) and yields a value of $\chi^2=???$ ({\bf chi $\chi^2=0.69$}). These values are listed in Table~\ref{tab:gen_table}, along with those {\bf obtained for UR and R cases, using observed abundances of main and all species separately as case 1 and case 2, for all positions.}\\

{\bf Second, in the central panel we notice two different solution islands, one is the best with minimum $\chi^2$ indicating with with cross associated with lower CRIR, and the other one marked with black square in Figure~\ref{fig:p2_n_T}, related higher CRIR, the $\chi^2$ is become worse though. 


\subsubsection{15 K}
To understand the nature of the extracted solutions in the central panel of Figure~\ref{fig:p2_n_T}, we tried to look at the time evolution of the main species shown in Figure~\ref{fig:p2_n_T_evolution}. In this Figure, abundances of gas-phase and grain-phase particles are shown with dotted and straight lines, respectively. In the model resulted in minimum $\chi^2$, at lower CRIR and early times, the model is in good match with observed abundances. But in high CRIR model, obviously due to higher CRIR, we see that abundances of HCO$^+$ rises up which leads to get further away from the observed value. In the panel of [CO], higher CRIR makes CO to reach equilibrium while it has been depleted less and the best position to be matched with the observed data is where at which CO is already in equilibrium. Higher CRIR boosts N$_2$H$^+$ to go up faster and then get down and be in good match with observation. Thus, in the model with higher CRIR, in spite the fact that the extracted model is able to reproduce [N$_2$H$^+$], but the main uncertainty comes from failing to reproduce [CO] and [HCO$^+$].


\subsubsection{10 K}
In the left middle panel of Figure~\ref{fig:p2_n_T}, it is shown than if temperature is 10~K, the best model will have higher CRIR, with higher $\chi^2$. In this panel, another green island at later time is also extracted which comes from the evolutionary path of HCO$^+$ and N$_2$H$^+$.

To compare the difference between the extracted solutions for T=10 and 15~K, we look at the evolution of the molecules in these two models in Figure~\ref{fig:p2_n_T_evolution_10K}. It is clear that at T=10~K, CO is depleted more in the form pf other grain species, i.e. GCH$_4$., while it is frozen up in T=15~K and depleted in the form of GCO. This model succeeds to reproduce CO observed abundance. When T is declined to 10~K, abundance of HCO$+$ rises with respect to T=15~K, but then it decreases faster and more. As time evolution of H$_{3}^+$ is plotted in the panel of HCO$^+$ in Figure~\ref{fig:p2_n_T_evolution_10K} with dashed-dotted lines, in the models with T=10~K, abundances of H$_{3}^+$ is higher rather than the model with T=15~k. On the other side, since the main reaction of HCO$+$ production, is combination of H$_{3}^+$ and CO, abundance of HCO$+$ increase at early times when T=10~K. Then, due to CO depletion to the grain species, HCO$+$ abundance is also decreased. In the case of N$_2$H$^+$, decreasing temperature, results in decreasing N$_2$H$^+$ abundance. In this panel gas-phase molecular nitrogen abundances is potted with dashed line which shows that at T=10~K, since N mostly is found in the form of grain particles (GN$_2$), gas-phase N$_2$ is declined which consequently leads to lower abundance of N$_2$H$^+$. In the model with T=10~K, the main uncertainty of $\chi^2$ comes from HCO$+$ abundance.


\subsubsection{20 K}

Time evolution of the species plotted in Figure~\ref{fig:p2_n_T_evolution_20K} shows that whereas at T=15~K, CO starts to be frozen out and depleted before 1.0e5 years, when T increases and rises up to T=20~K, CO remains in gas phase and it is depleted in the form of other grain species (GC$_2$H$_6$) after 1.0e7 years. This model is able to reproduce CO and N$_2$H$^+$, but it fails to predict HCO$^+$ observed abundance. As it has been indicated in Figure~\ref{fig:p2_n_T_evolution_20K}, when T=20~K, abundance of H$_{3}^+$ which is one of the reactants of HCO$^+$ formation, is declined. But on the other side, since CO is not depleted and can be found in gas phase, HCO$^+$ abundance evolution goes up with respect to the model with T=15~K. But then at later time, due to CO depletion, HCO$^+$ abundance is also decreases. 

In the model with T=20~K, in spite of existing higher amount of molecular Nitrogen in gas phase, due to less amount of H$_{3}^+$, abundances of N$_2$H$^+$ gets down with respect to the T=15~K. Then in later time, it rises and is declined very fast, because of N$_2$ gas phase depletion.



\subsubsection{Variation of CRIR}
Comparing evolution of the main species in the best model, as well as the models with higher and lower CRIR, demonstrated in Figure\ref{fig:p2_n_T_evolution_high_low_CRIR} shows that as CRIR decreases, the solution moves to later times. Although variation of CRIR parameter, when T=15~K, makes not much different in CO time history, but as $\zeta$ increases, CO is depleted more and reaches the equilibrium state later in time. Higher CRIR creates higher amount of H$_3^+$ due to ionization which leads a growth in HCO$+$ which can be seen in the middle panel of Figure~\ref{fig:p2_n_T_evolution_high_low_CRIR}. The same scenario can be applied to interpret the time evolution of N$_2$H$^+$.


\subsection{Astrochemical Implications for Cosmic Ray IonizationRate and Cloud Age, utilizing all observed species}


We have presented extracted best model parameters using abundances of the key species for $\zeta$, CO, HCO$^+$ and N$_2$H$^+$ at P2. Now we will show the influence of other species on the parameters of the best models.

Figure~\ref{fig:p2_n_T_case2} shows that when we add other species to perform the fitting and finding the best model, contributing only 5$\%$ of total $\chi^2$, in spite of the very decent $\zeta$ extracted at later time after 1Myr (central panel of Figure~\ref{fig:p2_n_T_case2}), due to high $\chi^2$ ($\sim$ 60), the fitting does not seem good. By adding other species, the extracted models fails to predict all observed abundances. 

Evolution of the species shown in Figure~\ref{fig:p2_n_T_evolution_case2} indicates that, the best models with minimum $\chi^2$ marked with black crosses in the middle panels of Figure~\ref{fig:p2_n_T_case2}, as well as the models with higher and lower $\zeta$ compared to the best models indicated in central panel of Figure~\ref{fig:p2_n_T_case2}, fails seriously to reproduce other abundances. The models are far below the observed abundance of CH$_3$OH, or far above the observed abundances of HNC, HCN and H$_2$CO. Amongst these models, the best matching has been extracted in the model with T=10~K, the value of $\chi^2$ is still high enough though (>40), to be called the best match.



\subsection{Astrochemical Implications for Cosmic Ray Ionization Rate and Cloud Age, at p6, the most quiescent region}

Extracted $\chi^2$ landscape in the $\zeta$ versus $t$ plane are shown in Figure~\ref{fig:p6_n_T_case1} for UR fitting of [CO], [HCO$^+$] and [N$_2$H$^+$] of the P6 position, which is the most quiescent region. These nine panels are centered around the case with $n_{\rm H}=4.6\times10^4\:{\rm cm}^{-3}$ and $T=15\:$K (with the other main variable of $A_V$ set equal to 7~mag for all nine panels). Then in each panel we see which values of $\zeta$ and $t$ give relatively low values of $\chi^2$, with values of $\chi^2<30$ illustrated via the color scale.

Several main features in the results of Figure~\ref{fig:p6_n_T_case1} can be noticed. First, the best result in the central panel that is best matched to the physical conditions of P6 has $\zeta=4.6\times 10^{-18}\:{\rm s}^{-1}$ and $t=2.88\times10^5\:$yr and yields a value of $\chi^2=2.47$. These values are listed in Table~\ref{tab:gen_table}, along with those obtained for UR and R cases, using observed abundances of main and all species separately as case 1 and case 2, for all positions.\\

One of the reasons that the estimated $\zeta$ at P6 (4.6e-18 s$^{-1}$), is bigger than that obtained at P2 (2.2e-18 s$^{-1}$), is the higher estimated abundances of main species at this position, which yields to match a model with higher $\zeta$, specially due to HCO$^+$ and N$_2$H$^+$ (Figure~\ref{fig:p2_n_T_evolution_high_low_CRIR} and \ref{fig:CO_evolution_fD_15K}). But since at the same time the density at this position is lower than that estimated at P2, as shown before in Figure~\ref{fig:CO_evolution_fD_15K}, as density reduces, the time history of the abundances tend to go up which is resulted in higher $\chi^2$ at P6, with respect to P2. Due to lower density, the later time and higher $\zeta$ solution in the central panel of Figure~\ref{fig:p6_n_T_case1} has became worse with $\chi^2$>25, which is no longer can be considered as a solution, compared to P2. Evolution of the species in the best models marked with white and black crosses in central panel of Figure~\ref{fig:p6_n_T_case1} has been shown in Figure~\ref{fig:p6_n_T_evolution_case1}. It can be noticed a similarity between the evolution of the species at P2 and P6, except the perfect matching at p2, and getting worse at P6.

\subsubsection{10K, at P6}

we can notice some bright features from Figure~\ref{fig:p6_n_T_case1}, central panel at T=10~K. Even though there can be seen common characteristics between the P2 and P6, but some differences are also noticeable. For both positions, the best solution has been appeared before 1Myrs, with higher $\zeta$, with higher $\zeta$ though. At both positions, we can see a very late time solution with higher $\zeta$, with better and lower $\chi^2$ at P6. Also, a very high $\zeta$ solution is detectable at both positions, which is a result of the oscillatory evolution of the species for the models with lower density with respect to CRIR, which we exclude these kinds of the models from our investigation, due to their uncertainties.


Figure~\ref{fig:p6_n_T_evolution_case1_10K} shows the evolution of the species in the vest models at T=15 and 10~K, at P6. As it has been discussed before for P2 (Figure~\ref{fig:p2_n_T_evolution_10K}), although there is not much changes in CO evolution at earlier times, but when T=10~K, HCO$^+$ abundances rises up and then declines very fast, whereas N$_2$H$^+$ abundances stays below those at T=15K, at all the times.  The very late time solution at T=10~K, which is marked with a black cross in the central left panel of Figure~\ref{fig:p6_n_T_case1}, comes from the model at which CO is deleted less and reached the equilibrium state (Figure~\ref{fig:p6_n_T_evolution_case1_10K}). 



\subsubsection{20K, at P6}

Very similar to the result extracted at P2 for the case T=20~K, evolution of the species in the best models presented in the central panels of Figure~\ref{fig:p6_n_T_case1}, is shown in Figure~\ref{fig:p6_n_T_evolution_case1_20K}, for the models with T=15 and 20 K. At p2, the best model at T=15 and 20~K, have identical $\zeta$, but at P6, the best model when T=20~K, has been estimated to have higher $\zeta$, by the factor of approximately 1 order of magnitude. Since estimated observed abundances of CO, HCO$^+$ and N$_2$H$^+$ at P6 are the highest values, we can see a red island containing $\chi^2$>25 before 10Myrs, in the panels of T=20~K at P6, which is the result of observed abundances and evolutionary path of the species.


\subsubsection{Estimated $\zeta$ and age of the cloud at P6, using all observed abundances}





\subsection{16 K}

\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/TH_T_var.pdf}
     \vspace*{-6mm}
     \caption{Evolution of the CO, HCO$^+$ and N$_2$H$^+$, in the models with $n_{\rm H}$ =1.0e5 cm$^{-3}$, $\zeta$=2.2e-17 s$^{-1}$, $A_{\rm v}$ =100 mag and for different temperatures. The horizontal band shows the observed abundances together with corresponding uncertainties, at p2.}
     \label{fig:TH_T_var_p2}
 \end{figure*}  
 

We presented the results extracted by fitting and using abundances of all species for P2 which is the position with the highest density and P6 which seems to be the quiescent region. In spite our expectation, the predicted $\zeta$ at these two positions are approximately in the same range. At P2, the region known with the highest star formation activities, which means it collapsed before and is still evolving, the age of the cloud has been estimated approximately 2.0e5 years, even slightly younger than P6. Thus, extracting almost similar results at two completely different regions, motivated us to investigate late time solution (>1Myr). Also, since the estimated temperature being approximately 15 K at each position, have been extracted from the dust temperature, we decided to look at the models with the temperatures above 15 K, because the gas temperature can be slightly higher. Hence, zooming in to the temperature range and looking at the models with different temperatures, between 15 and 20 K which are shown in Figure~\ref{fig:TH_T_var_p2}, indicates that the model with T=16 K could be the best alternative model for late time solution. In this Figure, the horizontal band shows observed abundances of species at P2, at which the minimum values have been estimated. Thus, for example at position 6 at which the highest amount of CO, HCO$^+$ and N$_2$H$^+$ has been observed, T=16 K will be matched even better than P2. As it is seen in the figure, there is noticeable changing in CO abundance between 15 and 16 K. Looking at the top rates of CO producing reactions show that when T=16 K, thermal desorption rate is approximately 100 times bigger than that of T=15k, whereas the same ratio between rates at T=20 and 16 K, is less than 10 times. Hence, the very fast increasing in CO abundance at T=16 K with respect to T=15 K, is due to the sudden changing in thermal desorption rates. 


\subsubsection{Time history of main species at 16 K}

\begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-1.2cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/TH_CR_var.pdf}
     \vspace*{-6mm}
     \caption{Evolution of the CO, HCO$^+$ and N$_2$H$^+$, in the models with $n_{\rm H}$ =1.0e5 cm$^{-3}$, T=16 K , $A_{\rm v}$ =100 mag and for different $\zeta$. The horizontal band shows the observed abundances together with corresponding uncertainties, at p2.}
     \label{fig:TH_CR_var_p2}
 \end{figure*}
 
 
 Figure~\ref{fig:TH_CR_var_p2} shows the evolution of CO, HCO$^+$ and N$_2$H$^+$ in the models with T=16 K, whereas all physical parameters are constant and they differ only in $\zeta$. Comparing the models with identical parameters with the evolution of the species at T=15 and 20 K shown in Figures~\ref{fig:CO_evolution_fD_15K} and \ref{fig:CO_evolution_fD_20K} respectively, shows that as T rises, CO depletion is declined and CO reaches the equilibrium whereas it has been depleted less. Investigation the reaction rates which produces or destructs CO shows that by raising temperature, thermal desorption rate increases as well which makes CO to get free from the surface of the grains and go back to the gas phase.\\
 
 
 Unlike the time history of the species when T=15 K (shown in Figure~\ref{fig:CO_evolution_fD_15K} which as $\zeta$ decreases, CO is depleted more and stabilized later, in the models with T=16 K, as $\zeta$ is increasing up to $\zeta$=1.0e-15 s$^{-1}$, CO depletion rises as well. When $\zeta$=1.0e-15 s${-1}$, CO depletion reduces again. These results is similar to the models with T=20 K, shown in Figure~\ref{fig:CO_evolution_fD}.
 
 When T=15 K, thermal desorption rate is not high enough to be the main reaction producing CO gas phase and the reaction below has the highest rate:
 
\begin{equation}
%\begin{split}
    \rm {HCO^{+} + e^{-} \longrightarrow CO + H}\\
%\end{split}
\label{eq:HCOP+e}
\end{equation}

And since production of both e$^{-}$ and HCO$^{+}$ depends on photons including cosmic ray photons, so as $\zeta$ is higher, it produces more e$^{-}$ and HCO$^{+}$ and CO gas phase consequently. 

When T=16 K, thermal desorption rate raises by the factor of approximately 2 orders of magnitude, making it to be the dominant reaction producing CO gas phase. At lower $\zeta$, GCO is not destroyed by photons, including comic ray photons. Hence, when T=16 K and $\zeta$ is lower and thermal desorption is the main mechanism producing CO gas phase, there is more GCO to be converted to CO gas phase. As $\zeta$ increases, CO grain phases are dissociated by photons which makes thermal desorption rate to be declined, resulting in more depletion of CO.

After $\zeta$=1.0e-15 s$^{-1}$, again reaction~\ref{eq:HCOP+e} becomes the dominant one and as $\zeta$ goes up, it produces more CO gas phase.


In all models with T=15,16 and 20 K, the main reaction producing HCO$^+$ and N$_2$H$^+$ contains H$_3^{+}$ and its abundance increases by increasing cosmic ray photons. Hence in all three models, abundance of HCO$^+$ and N$_2$H$^+$ increases when cosmic ray ionization rate raises up.


\subsubsection{Estimated $\zeta$ and age of the cloud at T=16 K, using main species}

\begin{figure*}[htb!]
    \centering
     \includegraphics[width=\textwidth]
     {chapters/images/p2_global_16K.pdf}
     \vspace*{-5mm}
     \caption{\tiny Distribution of $\zeta$ associated with $\chi^2$, using observed abundances at P2;XR)$n_{\rm H}$ =1.0e5 cm$^{-3}$ and $A_{\rm v}$ =20 mag, UR)$n_{\rm H}$ =2.2e5, 1.0e5, 4.6e4 cm$^{-3}$, $A_{\rm v}$ =10, 20, 50 mag, R)$n_{\rm H}$ =1.0e4-1.0e6 cm$^{-3}$, $A_{\rm v}$ =5-100 mag. In all panels T=16 K and white crosses show the location of minimum $\chi^2$ at each panel.}
     \label{fig:p2_glob_16K}
 \end{figure*}


\begin{figure*}[htb!]
    \centering
     \includegraphics[width=\textwidth]
     {chapters/images/p6_global_16K.pdf}
     \vspace*{-5mm}
     \caption{\tiny Distribution of $\zeta$ associated with $\chi^2$, using observed abundances at P6;XR)$n_{\rm H}$ =4.6e4 cm$^{-3}$ and $A_{\rm v}$ =7 mag, UR)$n_{\rm H}$ =1.0e5, 4.6e4, 2.2e4 cm$^{-3}$, $A_{\rm v}$ =5, 7, 10 mag, R)$n_{\rm H}$ =1.0e4-1.0e6 cm$^{-3}$, $A_{\rm v}$ =5-100 mag. In all panels T=16 K and white crosses show the location of minimum $\chi^2$ at each panel.}
     \label{fig:p6_glob_16K}
 \end{figure*}


Investigating through 16 K models at P2 and P6 using the abundances of main species CO, HCO$^+$ and N$_2$H$^+$ to find the best matched model, are shown in Figures~\ref{fig:p2_glob_16K} and \ref{fig:p6_glob_16K} respectively. These panels indicate that in both positions, the minimum $\chi^2$ tends to be before 1Myrs, associating to $\zeta$ $\approx$ 1.0e-18 s$^{-1}$, alike the results of T=15 K. As it has been indicated before for T=15 K, the impact of density variation is same when T=16 K. At higher densities, $\zeta$ increase as well, but the age gets younger and vice versa. 

These panels also show some later time solutions, specially for P2 in panels UR and R. But as it has been mentioned before, these solution come from the models with lower densities. For example, in panel R at Figure~\ref{fig:p2_glob_16K}, the later time solution marked with green cross, belongs to the model with $n_{\rm H}$ =1.0e4 cm$^{-3}$, which is approximately 10 times lower than that estimated at P2 ($n_{\rm H}$ =1.0e5 cm$^{-3}$).



\subsubsection{Estimated $\zeta$ and age of the cloud at T=16 K, using all species}

\begin{figure*}[htb!]
    \centering
     \includegraphics[width=\textwidth]
     {chapters/images/p2_global_all_16K.pdf}
     \vspace*{-5mm}
     \caption{\tiny Distribution of $\zeta$ associated with $\chi^2$, using all observed abundances at P2;XR)$n_{\rm H}$ =1.0e5 cm$^{-3}$ and $A_{\rm v}$ =20 mag, UR)$n_{\rm H}$ =2.2e5, 1.0e5, 4.6e4 cm$^{-3}$, $A_{\rm v}$ =10, 20, 50 mag, R)$n_{\rm H}$ =1.0e4-1.0e6 cm$^{-3}$, $A_{\rm v}$ =5-100 mag. In all panels T=16 K and crosses show the location of minimum $\chi^2$ at each panel.}
     \label{fig:p2_all_glob_16K}
 \end{figure*}


\begin{figure*}[htb!]
    \centering
     \includegraphics[width=\textwidth]
     {chapters/images/p6_global_all_16K.pdf}
     \vspace*{-5mm}
     \caption{\tiny Distribution of $\zeta$ associated with $\chi^2$, using all observed abundances at P6;XR)$n_{\rm H}$ =4.6e4 cm$^{-3}$ and $A_{\rm v}$ =7 mag, UR)$n_{\rm H}$ =1.0e5, 4.6e4, 2.2e4 cm$^{-3}$, $A_{\rm v}$ =5, 7, 10 mag, R)$n_{\rm H}$ =1.0e4-1.0e6 cm$^{-3}$, $A_{\rm v}$ =5-100 mag. In all panels T=16 K and crosses show the location of minimum $\chi^2$ at each panel.}
     \label{fig:p6_all_glob_16K}
 \end{figure*}


}








%obtained form their actual velocity range, with all the models in our grid i.e, considering the full parameter space. Thereafter, we will refer to this as \textit{Weighted-unrestricted fitting} method. We have selected the three species as first instance since ions are key tracers of $\zeta$ \citep{2020MNRAS.495L...7B} and their abundance depend on CO directly and indirectly \citep{2002P&SS...50.1133C}. 
%The parameters of the model that best reproduces our data are reported in tables~\ref{tab:p1_different_fittings}-\ref{tab:p10_different_fittings}.\\

%These best models obtained by \textit{Weighted-unrestricted fitting}, fail to reproduce the parameters of density, temperature and visual extinction, as measured in section~\ref{observations}, and the extracted values are not consistent with what we have obtained before. Hence, we have restricted the range of variation for Hydrogen nuclei density, temperature and visual extinction, in accordance to our estimates. We will refer to this as the \textit{Restricted} method for which density is allowed to vary in the range 1.0e4-1.0e6 cm$^{-3}$, temperature in the range 10-50 K and visual extinction in the range 5-100 mag.\\


%We have applied the \textit{Restricted} method on the CO, HCO$^+$ and N$_2$H$^+$ abundances. Note that, H$^{13}$CO$^+$ seems to be optically thick so that HCO$^+$ abundances obtained from H$^{13}$CO$^+$ can be underestimated. Hence, looking at all extracted spectra and choosing a narrower velocity range associated with the narrowest lines which is mostly based on N$_2$H$^+$ (77-82~km.s$^{-1}$) transition, and using HC$^{18}$O$^+$ to estimate HCO$^+$ abundances, we performed \textit{Restricted} fitting method to fit with the abundances in narrow range (\ref{tab:landscape-tab} in restricted region of parameters.\\

%Since we were worried about the estimated column density of Hydrogen obtained from Herschel map, and consequently the estimated abundances of the species, we used ratio abundances of the HCO$^+$ and N$_2$H$^+$ with respect to CO instead of absolute abundances with respect to Hydrogen, to avoid being affected by Hydrogen column density uncertainties. Thus, we tried to find the best model using the ratio abundances of narrow velocity range, and HCO$^+$ abundances obtained from HC$^{18}$O$^+$, in restricted region. Despite expecting to extract the same model obtained by using absolute abundances of the molecules, the matched models are not consistent with our expectations and varies from position to position. \\

%In continue, thinking about the contamination of CO, made us to use only the abundances of ions to see how the best model is far from the estimated CO abundance. Only at P10, the model is the same with the one obtained by using absolute abundances of CO, HCO$^+$ and N$_2$H$^+$, which means that the model extracted by using abundances of only positive charges, can reproduce observed abundance of CO, at P10.\\

%Since HCO$^+$ and N$_2$H$^+$ emissions may arise from different regions along the line of sight in the IRDCs, we have used their abundances separately together with CO to find the matched model. As it is shown in tables~\ref{tab:p1_different_fittings}-\ref{tab:p10_different_fittings}, we have obtained different models for either of the fitting methods.\\

%We proceeded by further restricting the range of parameters (\textit{Ultra restricted region}), allowing the n(H) density to cover the estimated value (Table~\ref{tab:physical_parameters_IRDC}) in the middle of three output, the temperature in the range 10-15 K and A$_v$ in a selected range based on our estimates at each position. We have repeated the fittings with the abundances of CO, HCO$^+$ and N$_2$H$^+$, for both broad and narrow velocity range. We refer to these as the weighted Ultra restricted method (\textit{WUR}) for the broad velocity range and the weighted Ultra restricted Narrow method (\textit{WURN}) for the narrow velocity range. We have used HCO$^+$ abundance obtained from both H$^{13}$CO$^+$ and HC$^{18}$O$^+$ in \textit{WUR} and \textit{WURN18} respectively. Extracted models in restricted and ultra-restricted region generally do not show identical parameters which shows that estimating accurate n(H) and choosing the best range of density is so important. Although we have obtained the same model with \textit{WRN18} and \textit{WURN18} at p1, p5 and p10, for the rest of the positions the solution with \textit{WURN18} method appears earlier times (<1 Myr).\\

%We have applied five more fitting methods by progressively including more species i.e. Carbon (C) and Nitrogen (N) bearing species to fit the data separately. The obtained high $\sim$ $\chi^2$ (>10) with these methods, show that the models are not in good match with the observed real data. Since CH$_3$OH is optically thick and may cause the major error in the fitting, we removed it from the list of the C-bearing species and performed the fitting without it as well. The lower $\chi^2$ values of the extracted models with this method, indicate that the models can reproduce the observed abundances better than those found by using both H$_2$CO and CH$_3$OH.\\



%Reviewing all fitting methods, we believe that using absolute narrow abundances of CO, HCO$^+$ obtained from HC$^18$O$^+$ and N$_2$H$^+$ in restricted region which is more sensitive to the estimated density at each position, leads to constrain physical properties of the cloud with high accuracy. Thus, based on the best models obtained by the \textit{Restricted} fitting method, the estimated CRIR toward all positions is in the range 1.0e-19-4.6e-18 s$^{-1}$. 

%In particular, we obtained $\zeta$ $\simeq$ 1.0e-19 s$^{-1}$ at p8, 2.2e-19 s$^{-1}$ at p2, p3, p4, p10, 4.6e-19 s$^{-1}$ at p7, 1.0e-18 s$^{-1}$ at p9, 4.6e-18 s$^{-1}$ at p1, p5 and 1.0e-15 s$^{-1}$ at p6 as the highest value. The age of the cloud has been estimated to be younger than 1.0e5 years at p1, in the period of 1.0e5 years at p5, p7, p9, after 1.0e6 years at p2, p3, p4, p6, p10 and even after 1.0e7 years at p8 (Tables~\ref{tab:p1_different_fittings}-\ref{tab:p10_different_fittings}).\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Discussion}\label{discussion}

The physical and chemical conditions of IRDCs are believed to be strictly linked to those required for the formation of massive stars \citep{hernandez2012virialized,2012MNRAS.423.2342F,2009Ap&SS.324..155R}. Comparing observational estimates of IRDC properties with state-of-the-art model predictions, can help us advancing in understanding of the star formation ignition in IRDCs. In particular, by studying regions at different levels of star formations, we can infer how the IRDCs properties vary with the star formation activity.\\


By using IRAM30m and NIR and MIR data obtained toward the IRDCs G028.37+00.07, we have measured the properties of density, temperature, visual extinction and molecular abundances toward ten positions across the cloud, believed to be at different levels of star formation. Hence, by comparing observations with a grid of astrochemical models we have estimated the CRIR and constrained the cloud dynamical age.\\



\subsection{Estimated CRIR using CO, HCO$^+$ and N$_2$H$^+$}

As it has been described in the previous section, we tried to find the best models using multiple abundances and different ways. Using the models matched with the minimum $\chi^2$ shows in Tables~\ref{tab:p1_different_fittings}-\ref{tab:p10_different_fittings}, we can extract the range of cosmic ray ionization rate at each position, depending on the chosen method. We set all parameters except $\zeta$ of the best model, to be held fixed and change only cosmic ray ionization rate of the models to estimate $\chi^2$ for each data point. At the end, we have the distribution of cosmic ray ionization rate based on the variation of $\chi^2$, from which we are able pick up the acceptable range for cosmic ray ionization rate ($\chi^2$ < 3).\\ 

%The extracted dot-plots based on the selected fitting method are demonstrated for all positions in Figures~\ref{fig:restricted}-\ref{fig:R+N-group+h2co}. \\

Since the lower $\chi^2$ value of the best fitted model, using CO, HCO$^+$ and N$_2$H$^+$ observed abundances, is the indication of the perfect match between the model and observational data, and on the other hand these three species have key roles to estimate CRIR, we believe that the predicted CRIR range using these three species will be the most plausible value for this quantity.\\ 

Using the parameters of the best fitted models and keeping them fixed and changing $\zeta$ of the models to extract CRIR range,$\zeta$ associated with $\chi^2$<3 has been estimated 1.0e-19-2.2e-19 s$^{-1}$ at p8, 1.0e-19-4.6e-19 s$^{-1}$ at p2,p3,p4,p10, 2.2e-19-4.6e-19 s$^{-1}$ at p6, 2.2e-19-1.0e-18 s$^{-1}$ at p7, 4.6e-19-2.2e-18 s$^{-1}$ at p9, 1.0e-18-1.0e-17 s$^{-1}$ at p5, and 2.2e-18-2.2e-17 s$^{-1}$ at p1. The results are shown in panel a of Figures~\ref{fig:p2_glob} and \ref{fig:p6_glob} for P2 and P6 and figures~\ref{fig:p1_global_cr}-\ref{fig:p10_global_cr} for the rest of the positions.

\subsubsection{Gloabl CRIR using CO, HCO$^+$ and N$_2$H$^+$}

We have seen the CRIR range, predicted by using the best fitted mode, for which we only searched through models with different $\zeta$. Now, we need to understand what happens if the other parameters, i.e., density, temperature and visual extinction are varied.\\

 Figure~\ref{fig:p2_n_T} shows how variation of temperature and density affects on the estimated range of CRIR. In this figure, it is obvious that when the density decreases, $\zeta$ decreases as well, the age of the cloud grows up. Whereas raising temperature, makes CRIR to be reduced, while the age of cloud gets either older or younger, depending on the temperature. In Figure~\ref{fig:p2_n_av}, it has been indicated that CRIR has less sensitivity on A$_v$ (A$_v$ > 5 mag).\\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[htb!]
    \centering
    \addtolength{\leftskip} {-1.2cm}
    \addtolength{\rightskip}{-1cm}
     \includegraphics[width=20cm, height=16cm]
     {chapters/images/p2_n_av.pdf}
     \vspace*{-14mm}
     \caption{$\chi^2$ landscape in the $n_{\rm H}$ versus $t$ plane for Extra-restricted (XR) fitting of the abundances of CO, HCO$^+$ and N$_2$H$^+$ at the P2 position. For these models, T has been set to be 15~K and the location of the minimum $\chi^2$ has been marked with a white cross.}
     \label{fig:p2_n_av}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_global.pdf}
     \vspace*{-5mm}
     \caption{\tiny Distribution of $\zeta$ associated with $\chi^2$,a) using the best fitted model at P2 and keep all parameters to be held fixed and change $\zeta$, b) extracted global CRIR from models with n(H)=1.0e4,2.2e4,4.6e4 cm$^{-3}$, T=10,15,20 K, and A$_v$=20,50 and 100 mag, c) extracted global CRIR from models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T=10-50 K and A$_v$=5-100 mag.}
     \label{fig:p2_glob}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p6_global.pdf}
     \vspace*{-5mm}
     \caption{\tiny Distribution of $\zeta$ associated with $\chi^2$,a) using the best fitted model at P6 and keep all parameters to be held fixed and change $\zeta$, b) extracted global CRIR from models with n(H)=1.0e4,2.2e4,4.6e4 cm$^{-3}$, T=10,15,20 K, and A$_v$=5,7 and 10 mag, c) extracted global CRIR from models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T=10-50 K and A$_v$=5-100 mag.}
     \label{fig:p6_glob}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_gobal_evo.pdf}
     \vspace*{-5mm}
     \caption{\tiny Evolution of three main species: The horizontal band shows the observed abundances at P2, the red line belongs to the model with n(H)=1.0e6 cm$^{-3}$, T=10 K, $\zeta$=1.0e-14 and A$_v$=5 mag, the black line belongs to the model with n(H)=1.0e4 cm$^{-3}$, T=15 K, $\zeta$=2.2e-19 and A$_v$=100 mag, the best fitted model by \textit{Restricted} method at p2, indicated in table~\ref{tab:p2_different_fittings}, the green line belongs to the model with n(H)=1.0e6 cm$^{-3}$, T=20 K, $\zeta$=1.0e-17 and A$_v$=5 mag and the blue line belongs to the model with n(H)=1.0e6 cm$^{-3}$, T=30 K, $\zeta$=1.0e-17 and A$_v$=100 mag. The dotted colored lines in the panel of CO, shows the evolution of the top C-bearing species in the same model and the dashed vertical lines, shows the time location at which the models is fitted with observed data.}
     \label{fig:p2_glob_evo}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[htb!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p6_global_evo.pdf}
     \vspace*{-5mm}
     \caption{\tiny Evolution of three main species: The horizontal band shows the observed abundances at P6, the black line belongs to the model with n(H)=1.0e4 cm$^{-3}$, T=15 K, $\zeta$=4.6e-19 and A$_v$=5 mag, the best fitted model by \textit{Restricted} method at p6, indicated in table~\ref{tab:p2_different_fittings} and the red line belongs to the model with n(H)=2.2e4 cm$^{-3}$, T=15 K, $\zeta$=1.0e-18 and A$_v$=5 mag. The dotted colored lines in the panel of CO, shows the evolution of the top C-bearing species in the same model and the dashed vertical lines, shows the time location at which the models is fitted with observed data.}
     \label{fig:p6_glob_evo}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


It is clear that CRIR is very sensitive to density and temperature. Thus, depending on the best fitted model and considering the grids of the models we have created before, we tried to extract a relatively-global CRIR, by searching through models with T = 10,15,20 K and adjacent densities and visual extinctions, covering only three values of the associated parameter, to calculate minimum $\chi^2$ at each data point. The results have been indicated in panel b of the figures~\ref{fig:p2_glob} and \ref{fig:p6_glob}.\\ 

At the end, we need to extract a global CRIR range which is the result of minimum $\chi^2$ at each time step and coming from any slice of density in the range 1.0e4-1.0e6 cm$^{-3}$, temperature between 10 and 50 K and A$_v$ in the range 5-100 K which is shown in panel c of Figures~\ref{fig:p2_glob} and \ref{fig:p6_glob} for P2 and P6 and Figures~\ref{fig:p1_global_cr}-\ref{fig:p10_global_cr} for the remaining regions. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In these images, we see a similarity of CRIR distribution for all position, that is CRIR starts from very low value which comes from the models with lower densities with T=15 K and is expanded upwards, towards earlier time which is the result of the models with higher densities and same temperature. Although we see also some other purple areas which belongs to different models with different parameters.\\





In Figure~\ref{fig:p2_glob}, we see couple of purple islands which belong to $\chi^2$<4 and show the good mach between observed and theoretical abundances. The very high $\zeta\simeq$ 4.6e-16-1.0e-14 s$^{-1}$, comes from the models with T=10 K, and relatively higher densities. Evolution of CO, HCO$^+$ and N$_2$H$^+$ for one of these models with T=10 K, has been indicated with red lines in Figure~\ref{fig:p2_glob_evo} which shows CO has been reached to the equilibrium.

For $\zeta$=1.0e-17 s$^{-1}$, we see three different regions, one before 1Myrs which belongs to the models with T=15 K, and two regions after 1Myrs. The first one after 1Myrs comes from the models with T=20 K and the second one belong to the models with T=30 K, with very high density for both (n(H)=1.0e6 cm$^{-3}$). Evolution of the species has been shown with green and blue lines in Figure~\ref{fig:p2_glob_evo}, for these models respectively. The very late time solution for $\zeta$=2.2e-18 and 4.6e-18 s$^{-1}$, also have been extracted from the models with T=20 K. At $\zeta$=2.2e-19 s$^{-1}$, we see a very good match with very low $\chi^2$, after 1.0e7 years, which also belongs to T=20 model.\\

Figure~\ref{fig:p2_glob} shows that the area of the minimum $\chi^2$ in which the best fitted models is included, starts from $\zeta$=1.0e-19 s$^{-1}$ with lower densities, and is expanded up to 1.0e-16 s$^{-1}$ with higher densities, comes from models with T=15 K, which is in consistent with our estimation (T=13 K). The black line of molecular evolution in Figure~\ref{fig:p2_glob_evo}, has been plotted for the best fitted model which shows CO is reaching to the equilibrium state. Looking at the evolution of the CO, in different models with different temperatures, indicates that as T increases, CO depletion starts later in time, and C is found in different grain species.\\

At p6, with the most abundant CO and N$_2$H$^+$ and estimated lowest density, the extracted relatively-global and global CRIR has been shown in Figure~\ref{fig:p6_glob}, panel b and c respectively. It is obvious from figure that due the very specific condition of p6, a Short interval for $\zeta$ has been estimated. This results which comes from the models with T=15 K, predicts CRIR to be in the range of 2.2e-19-2.2e-18 s$^{-1}$. We see a very small set of data point at $\zeta$=2.2e-19 s$^{-1}$, after 1.0e7 years, which is due to the models with higher temperature T=20 K. Figure~\ref{fig:p6_glob_evo} shows how increasing density, leads to estimate higher CRIR, and younger age of the cloud.\\

Considering the estimated temperature (T$\simeq$ 13 K) towards all positions, estimated CRIR obtained from models with T=10 and 15 K can be acceptable. But since the predicted density of the models with T=10 K, is higher ($\simeq$ 1.0e6 cm$^{-3}$) than what we have obtained before from the Hydrogen density map (n(H)$\simeq$1.0e4-1.0e5 cm$^{-3}$), we accept the results coming the models with T=15 K. Thus $\zeta$ is predicted to be 1.0e-19-1.0e-17 s$^{-1}$ at p10, 1.0e-19-2.2e-17 s$^{-1}$ at p7,p8,p9, 1.0e-19-4.6e-17 s$^{-1}$ at p4, 1.0e-19-1.0e-16 s$^{-1}$ at p1,p2,p3,p5, and 2.2e-19-2.2e-18 s$^{-1}$ at p6 as the lowest range of CRIR. The age of the cloud is expanded since 1.0e5 yr up to after 1Myrs. The results predict that starless positions p7-p10 and p6, have relatively lower CRIR with respect to active regions. It should be mentioned that at p1, the higher CRIR $\zeta$>1.0e-16 s$^{-1}$, has been extracted from the models with T= 10 K with very high density (1.0e6 cm$^{-3}$).\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Estimated CRIR adding C-bearing species}

To find the best model matched with observed abundances, we added other species to the main group of CO, HCO$^+$ and N$_2$H$^+$. We divided the species to two C-bearing and N-bearing species. Tables~\ref{tab:p1_different_fittings}-\ref{tab:p10_different_fittings} shows that adding H$_2$CO, with or without CH$_3$OH, makes the $\chi^2$ to get worst which means the models struggles to reproduce the observed data, although it is obvious that the main error is due to the abundance of CH$_3$OH. Since the highest abundance of H$_2$CO has been estimated at p2, and CH$_3$OH abundance at p2 is also higher with the respect to the most of the positions, we investigate the effect of adding C-bearing species to the final estimated global CRIR.\\

The estimated CRIR using C-bearing species at P2 indicated in Figure~\ref{fig:main+h2co+ch3oh}, shows lower $\zeta \simeq$ 1.0e-19 s$^{-1}$, which comes from the lower densities of the models with T=20 K. Figure~\ref{fig:main+h2co} shows the evolution of the species in the model extracted using abundances of main group together with H$_2$CO. This model fails to reproduce observed abundances of other species, specially HNCO and CH$_3$OH and it even gets worst if the $\zeta$ is increased. Similarly, the matched model extracted using abundances of the main group together with CH$_3$OH, fails to reproduce observed abundances of H$_2$CO and N-bearing species, but with higher uncertainties rather than H$_2$CO. This result makes us to add only abundance of H$_2$CO to the main group and extract global CRIR and exclude CH$_3$OH from the list of the species.\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_h2co-ch3oh.pdf}
     \vspace*{-4mm}
     \caption{\tiny Estimated CRIR from the models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T = 5-50 K and A$_v$ = 5-100 mag, using abundances of CO, HCO$^+$, N$_2$H$^+$ (main), together with H$_2$CO and CH$_3$OH at p2.}
     \label{fig:main+h2co+ch3oh}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p6_h2co-ch3oh.pdf}
     \vspace*{-4mm}
     \caption{\tiny Estimated CRIR from the models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T = 5-50 K and A$_v$ = 5-100 mag, using abundances of CO, HCO$^+$, N$_2$H$^+$ (main), together with H$_2$CO and CH$_3$OH at p6.}
     \label{fig:main+h2co+ch3oh-p6}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/1_p2.pdf}
     \vspace*{-4mm}
     \caption{\tiny Evolution of the species in the best model with n(H)=1.0e4 cm$^{-3}$, T=20 K, $\zeta$=1.0e-19 s$^{-1}$ and A$_v$=5 mag, found by using abundances of CO, HCO$^+$, N$_2$H$^+$ and H$_2$CO at p2. The vertical dashed line shows the time at which the minimum $\chi^2$ has been found. The horizontal bands are observed abundances at p2. The dashed evolutionary path at each panel shows the evolution of the associated species, in the model with higher $\zeta$=1.0e-17 s$^{-1}$.}
     \label{fig:main+h2co}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Estimated CRIR adding N-bearing species}

Since the highest abundances of HNC and HCN have been estimated at p6, we try to understand the influence of their abundances in the final global CRIR. Figure~\ref{fig:main+hnc+hcn} shows that using these abundances leads to extract very low CRIR $\simeq$ 2.2e-19 s$^{-1}$, which comes from the models with lower densities, i.e., n(H) = 1.0e4 cm$^{-3}$, T=20 K, A$_v$= 5 mag and the same model only with different temperature T=15 K, using HCN and HNC respectively, where as the age of the cloud has been estimated older than 1Myrs. The evolution diagram of the species in the best matched models found by using HCN and HNC abundances (Figure~\ref{fig:main+hcn} and \ref{fig:main+hnc}), shows that where as these two models can relatively reproduce observed abundances of HCN and HNC, fails to reproduce other species i.e., HNCO, H$_2$CO and CH$_3$OH. This result make us to use only abundances of HCN and HNC, together with the main group to estimate global CRIR.\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p6_hnc-hcn.pdf}
     \vspace*{-4mm}
     \caption{\tiny Estimated CRIR from the models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T = 5-50 K and A$_v$ = 5-100 mag, using abundances of CO, HCO$^+$, N$_2$H$^+$ (main), together with HCN and HNC at p6.}
     \label{fig:main+hnc+hcn}
 \end{figure*}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2_hnc-hcn.pdf}
     \vspace*{-4mm}
     \caption{\tiny Estimated CRIR from the models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T = 5-50 K and A$_v$ = 5-100 mag, using abundances of CO, HCO$^+$, N$_2$H$^+$ (main), together with HCN and HNC at p2.}
     \label{fig:main+hnc+hcn_p2}
 \end{figure*}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/1.pdf}
     \vspace*{-6mm}
     \caption{\tiny Evolution of the species in the best model found using abundances of CO, HCO$^+$, N$_2$H$^+$ and HCN at p6. The vertical dashed line shows the time at which the minimum $\chi^2$ has been found. The horizontal bands are observed abundances at p6.}
     \label{fig:main+hcn}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/2.pdf}
     \vspace*{-6mm}
     \caption{\tiny Evolution of the species in the best model found using abundances of CO, HCO$^+$, N$_2$H$^+$ and HNC at p6. The vertical dashed line shows the time at which the minimum $\chi^2$ has been found. The horizontal bands are observed abundances at p6.}
     \label{fig:main+hnc}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Global CRIR by adding more species to the main group}
In this section, we show the final estimated CRIR, when we add other species to the main group of CO, HCO$^+$ and N$_2$H$^+$.


\subsubsection{Global CRIR using abundances of CO, HCO$^+$, N$_2$H$^+$, HCN and HNC}

Since we have noticed that adding HCN and HNC abundances to the main group of the species and perform fitting, leads to extract a model which can predict the abundances of HCN and HNC with good estimates, we decided to extract the global CRIR, by adding abundances of HCN and HNC to the main group and exclude other species. We weight them unequally, in a way that HCN together with HNC contain 25$\%$ of total $\chi^2$. Figure\ref{fig:main+hnc+hcn} shows that CRIR has been estimated $\zeta \simeq$ 2.2e-19 s$^{-1}$ at p2 the densest region and at p6, with the highest abundances of HCN and HNC. These estimation for both regions comes from the lower densities of the models with T = 20 K. Thus, adding other species to the main group, leads to find the models which actually fail to predict the estimated temperature at the positions.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2-p6_hnc+hcn.pdf}
     \vspace*{-6mm}
     \caption{\tiny Estimated CRIR from the models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T = 5-50 K and A$_v$ = 5-100 mag, using abundances of CO, HCO$^+$, N$_2$H$^+$ (main), together with HCN and HNC at p2 and P6.}
     \label{fig:main+hcn+hnc}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Global CRIR using abundances of CO, HCO$^+$, N$_2$H$^+$, HCN, HNC and H$_2$CO}

Since we have noticed that adding H$_2$CO to the main group to estimate global CRIR, makes to achieve lower uncertainty, rather than CH$_3$OH, it would be helpful if we investigate the influence of H$_2$CO on the global CRIR.\\

Figure~\ref{fig:main+hcn+hnc+h2co} shows that when we add H$_2$CO to the main group and using HCN and HNC as well and weighting in a way that the added species contain only 25$\%$ of total $\chi^2$, lower CRIR $\zeta$ = 2.2e-19 s$^{-1}$ is estimated which comes from the same models, as when we use only HCN and HNC abundances, i.e., lower densities with T = 20 K. The only difference is that since we added H$_2$CO, the value of $\chi^2$ gets worse.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2-p6_hnc+hcn+h2co.pdf}
     \vspace*{-6mm}
     \caption{\tiny Estimated CRIR from the models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T = 5-50 K and A$_v$ = 5-100 mag, using abundances of CO, HCO$^+$, N$_2$H$^+$ (main), together with HCN, HNC and H$_2$CO, at p2 and P6.}
     \label{fig:main+hcn+hnc+h2co}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Global CRIR using abundances of all species}

We have noticed that using HNCO, and C-bearing species, specially CH$_3$OH leads to extract a model that actually fails to reproduce observe abundances and consequently the matching gets worse ($\chi^2$ > 10). But to see the final estimated global CRIR, we try to use all observe abundances and weight them in a way that all added species, i.e., HCN, HNC, HNCO, H$_2$CO and CH$_3$OH contain 25$\%$ of total $\chi^2$. Using this method, the best fitted model with n(H) = 1.0e6 cm$^{-3}$, T = 30 and A$_v$ = 50 mag, predicts CRIR $\zeta$ = 4.6e-18 s$^{-1}$, for both P2 and P6, which completely differ each other, from properties and estimated abundances point of view. The estimated parameters, i.e., density and temperature are not consistent with the measured quantities shown in table~\ref{tab:landscape-tab}.
The global CRIR using all observed abundances has been shown in Figure~\ref{fig:all_global}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[ht!]
    \centering
    %\addtolength{\leftskip} {-2.3cm}
    %\addtolength{\rightskip}{-1cm}
     \includegraphics[width=\textwidth]
     {chapters/images/p2-p6_all.pdf}
     \vspace*{-6mm}
     \caption{\tiny Estimated CRIR from the models with n(H)=1.0e4-1.0e6 cm$^{-3}$, T = 5-50 K and A$_v$ = 5-100 mag, using abundances of all observed species, at p2 and P6.}
     \label{fig:all_global}
 \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






==> chapters/tables/fiducial_parameters.tex <==

\begingroup
\setlength{\tabcolsep}{15pt} % horizontal space
\renewcommand{\arraystretch}{1.3} % vertical space


\begin{table}[H]
\centering
\begin{tabular}{c c}
      \hline
      \hline
      Parameter & Value \\
      \hline
      n$_H$ &  1.0e5~~cm$^{-3}$ \\
      T & 20~~K \\
      A$_V$ & 100~~mag \\
      $\zeta$ & 1.0e-16~~s$^{-1}$ \\
    \hline 
    \end{tabular}
    \vspace{2mm}
    \caption{Fiducial Parameter Values}
    \label{tab:fiducial_parameters}
\end{table}





























































==> chapters/tables/gen_table.tex <==
%\begin{landscape}
\setlength{\tabcolsep}{8pt} % horizontal space
\renewcommand{\arraystretch}{2} % vertical space

\Large
\begin{table*}[htpb!]\centering
 \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{c c c c c}
  \hline
  \hline
  & & XR & UR & R\\
  \hline
 P1 & main & 1.0e-18/1.70e5/1.0e5/15/20/0.107 & 1.0e-18/1.70e5/1.0e5/15/50/0.107 & 1.0e-19/2.00e7/2.2e4/20/5/0.070 \\
  & all & 1.0e-13/9.33e3/1.0e5/15/20/43.015 & 1.0e-18/1.00e8/2.2e5/20/10/37.754 & 4.6e-18/1.00e8/1.0e6/30/50/8.555\\
  \hline
  P2 & main & 2.2e-18/2.00e5/1.0e5/15/20/0.692 & 1.0e18/4.17e5/4.6e4/15/50/0.173 & 2.2e-19/2.24e6/1.0e4/15/5/0.020\\
 & all & 1.0e-13/2.88e3/1.0e5/15/20/52.752 & 1.0e-16/1.45e5/2.2e5/10/10/42.640 & 1.0e-17/5.62e7/1.0e6/30/50/16.256\\
  \hline
P3 & main & 2.2e-18/1.95e5/1.0e5/15/20/0.970 & 1.0e-18/3.98e5/4.6e4/15/10/0.494 & 2.2e-19/2.09e6/1.0e4/15/5/0.166\\
 & all & 1.0e-13/9.33e3/1.0e5/15/20/55.295 & 2.2e-18/5.25e7/2.2e5/20/10/47.706 & 4.6e-18/1.00e8/1.0e6/30/50/18.559\\
  \hline
  P4 & main & 2.2e-18/1.91e5/1.0e5/15/20/0.858 & 1.0e-18/3.89e5/4.6e4/15/10/0.312 & 2.2e-19/2.00e6/1.0e4/15/5/0.027\\
 & all & 1.0e-13/7.24e3/1.0e5/15/20/50.513 & 2.2e-18/5.13e7/2.2e5/20/10/43.412 & 4.6e-18/1.00e8/1.0e6/30/50/15.679\\
  \hline
  P5 & main & 2.2e-18/1.74e5/1.0e5/15/20/0.483 & 1.0e-18/3.55e5/4.6e4/15/10/0.208 & 4.6e-19/7.59e5/2.2e4/15/5/0.125\\
 & all & 1.0e-13/9.33e3/1.0e5/15/20/46.611 & 2.2e-18/5.13e7/2.2e5/20/10/43.081 & 4.6e-18/1.00e8/1.0e6/30/50/12.579\\
  \hline
  P6 & main & 4.6e-18/2.88e5/4.6e4/15/7/2.474 & 1.0e-18/7.24e5/2.2e4/15/5/1.730 & 4.6e-19/1.66e6/1.0e4/15/5/1.334\\
 & all & 4.6e-14/6.17e3/4.6e4/15/7/34.657 & 4.6e-19/1.48e7/2.2e4/20/5/13.309 & 4.6e-19/1.48e7/2.2e4/20/5/13.309\\
  \hline
  P7 & main & 1.0e-18/3.31e5/4.6e4/15/10/0.723 & 2.2e-19/8.32e5/2.2e4/15/20/0.392 & 1.0e-19/2.00e6/1.0e4/15/7/0.211 \\
 & all & 4.6e-14/2.45e4/4.6e4/15/10/40.362 & 1.0e-18/1.00e8/1.0e5/20/7/39.321 & 4.6e-18/1.00e8/1.0e6/30/50/11.610 \\
  \hline
  P8 & main & 4.6e-19/3.80e5/4.6e4/15/10/0.434 & 2.2e-19/8.13e5/2.2e4/15/7/0.271 & 1.0e-19/1.95e6/1.0e4/15/5/0.041\\
 & all & 4.6e-14/2.45e4/4.6e4/15/10/39.054 & 1.0e-19/7.76e6/2.2e4/15/7/37.034 & 4.6e-18/1.00e8/1.0e6/30/50/12.060 \\
  \hline
  P9 & main & 2.2e-18/1.78e5/1.0e5/15/20/0.483 & 1.0e-18/3.63e5/4.6e4/15/10/0.271 & 1.0e-19/2.34e6/1.0e4/15/100/0.117\\
 & all & 1.0e-13/9.33e3/1.0e5/15/20/49.929 & 2.2e-18/5.13e7/2.2e5/20/10/44.473 & 4.6e-18/1.00e8/1.0e6/30/50/13.954\\
  \hline
  P10 & main & 2.2e-18/3.16e5/4.6e4/15/10/0.507 & 4.6e-19/7.94e5/2.2e4/15/20/0.200 & 2.2e-19/1.91e6/1.0e4/15/100/0.055\\
 & all & 4.6e-14/1.00e3/4.6e4/15/10/44.001 & 2.2e-17/5.01e5/4.6e4/10/7/38.312 & 4.6e-18/1.00e8/1.0e6/30/50/14.364\\

        \hline
        \hline
    \end{tabular}
  \end{adjustbox}
  \vspace*{1mm}
  \caption{Extracted Astrochemical parameters of the best models by applying observed abundances in Restricted (R), Ultra restricted (UR) and Extra restricted (XR) regions, using main species, [CO],[HCO$^+$] and [N$_2$H$^+$] (A) and all observed abundances (B). The extracted parameters are $\zeta$ [s$^{-1}$], Time [year], $\mathrm{n}_H$ [cm$^{-3}$], T [K], $\mathrm{A}_v$ [mag] and $\chi^2$, respectively from left to right.}
  \label{tab:gen_table}
  
\end{table*}
%\end{landscape}


==> chapters/tables/initial_abundances.tex <==

\begingroup
\setlength{\tabcolsep}{10pt} % horizontal space
\renewcommand{\arraystretch}{1.3} % vertical space


\begin{table}[H]
\caption{Fiducial Initial Abundances}
\centering
\begin{tabular}{c c}
      \hline
      \hline
      Species & Abundance ($n_{\rm X}/n_{\rm H}$)\\
      \hline
      H$_2$ & 5.00e-01\\
      H & 5.00e-05 \\
      He & 9.75e-02 \\
      CO & 1.40e-04 \\
      O & 1.80e-04 \\
      N & 7.50E-05 \\
      S &  8.00e-08 \\
      F & 2.00e-08 \\
      Si & 8.00e-09 \\
      Cl & 4.00e-09 \\
      P & 3.00e-09 \\
      GRAIN & 1.30e-12\\
    \hline 
    \end{tabular}
    %\vspace{2mm}
    %\caption{Fiducial initial elemental abundances.}
    \label{tab:initial_abundances}
\end{table}

%\endgroup




























==> chapters/tables/initial_parameters.tex <==

\begingroup
\setlength{\tabcolsep}{10pt} % horizontal space
\renewcommand{\arraystretch}{1.3} % vertical space


\begin{table}[H]
\caption{Model Grid Parameter Space}
\centering
\begin{tabular}{c c c}
      \hline
      \hline
      Parameter & Explored Range \\
      \hline
      $n_{\rm H}$ (cm$^{-3}$) & 10 - $10^9$\\
      $T$ (K) & 5 - 1000\\
      $\zeta$ (s$^{-1}$) & $10^{-19}$ - $10^{-13}$\\
      $A_V$ (mag) & 1 - 100\\
%      t & time & 1.0e3-1.0e8~~year \\
      $G_0$ (Habings) & 4\\
%      a$_0$ & dust particle radius & 0.1 $\mu$m \\
    \hline 
    \end{tabular}
    \label{tab:initial_parameters}
\end{table}

%\endgroup




























































==> chapters/tables/landscape.tex <==
\begin{landscape}
\setlength{\tabcolsep}{9pt} % horizontal space
\renewcommand{\arraystretch}{1.8} % vertical space

\begin{table}[htpb!]\centering
 \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{c c c c c c c c c c c c c c c c c c c c c c}
  \hline
  \hline
          position & R.A. & Dec. &  $\Sigma$ & $N_H$ & $n_H$ & $A_{V,{\rm tot}}$ & $\bar{A}_V$ & T & [C$^{18}$O] & [CO] & [H$^{13}$CO$^{+}$] & [HCO$^+$] & [HC$^{18}$O$^{+}$] & [HCO$^+$] & [N$_2$H$^+$] & [HNCO] & [HN$^{13}$C] & [HNC] & [HCN] & [H$_2$CO] & [CH$_3$OH] \\
           & (J2000) & (J2000) & [gcm$^{-2}$] & [10$^{23}$ cm$^{-2}$] & [10$^{4}$ cm$^{-3}$] & [mag] & [mag] & [K] & [10$^{-8}$] & [10$^{-5}$] & [10$^{-11}$] & [10$^{-10}$] & [10$^{-12}$] & [10$^{-10}$] & [10$^{-10}$] & [10$^{-10}$] & [10$^{-11}$] &  [10$^{-10}$] & [10$^{-11}$] & [10$^{-11}$] & [10$^{-9}$] \\
         \hline
         \rule{0pt}{2ex}
         P1 & 18:42:46.687 & -4:04:08.830 & 0.394 & 1.68 & 10.50 & 88.4 & 22.1 & 11.8 & $4.77\pm$1.47 & $1.52\pm$0.56 & $1.02\pm$0.31 & $4.11\pm$1.51 & $1.96\pm$0.69 & $6.23\pm$2.54 & $0.55\pm$0.17 & $2.17\pm$0.74 & $1.41\pm$0.43 & $5.65\pm$2.08 & $11.10\pm$3.44 & $3.89\pm$1.26 & $0.52\pm$0.18\\
         & & & 0.270 & 1.15 & 7.19 & 60.7 & 15.2 & \\
         \hline
         P2 & 18:42:50.709 & -4:03:14.763 & 0.438 & 1.87 & 11.70 & 98.4 & 24.6 & 13.1 & $4.31\pm$1.33 & $1.37\pm$0.51 & $1.11\pm$0.34 & $4.48\pm$1.64 &$1.84\pm$0.67 & $5.84\pm$2.43 & $1.79\pm$0.56 & $4.29\pm$1.45 & $1.61\pm$0.50 & $6.47\pm$2.37 & $10.30\pm$3.22 & $10.40\pm$3.33 & $1.73\pm$0.60\\
         & & & 0.296 & 1.26 & 7.88 & 66.6 & 16.6\\
         \hline
        P3 & 18:42:49.490 & -4:02:21.514 & 0.330 & 1.41 & 8.84 & 74.2 & 18.6 & 13.5 & $4.86\pm$1.50 & $1.54\pm$0.57 & $0.87\pm$0.27 & $3.49\pm$1.28 &$1.88\pm$0.74 & $5.96\pm$2.64 & $1.53\pm$0.47 & $4.15\pm$1.41 & $1.85\pm$0.57 & $7.43\pm$2.73 & $5.86\pm$1.88 & $7.33\pm$2.37 & $1.74\pm$0.61\\
        & & & 0.265 & 1.13 & 7.06 & 59.6 & 14.9 \\
        \hline
        P4 & 18:42:52.583 & -4:02:44.647 & 0.322 & 1.38 & 8.65 & 72.6 & 18.2 & 13.4 & $5.19\pm$1.60 & $1.65\pm$0.61 & $0.97\pm$0.30 & $3.89\pm$1.43 &$1.64\pm$0.65 & $5.23\pm$2.31 & $1.52\pm$0.47 & $3.45\pm$1.18 & $1.64\pm$0.51 & $6.59\pm$2.43 & $8.16\pm$2.57 & $7.66\pm$2.47 & $1.33\pm$0.46\\
        & & & 0.267 & 1.14 & 7.12 & 60.1 & 15.0\\
        \hline
        P5 & 18:42:53.970 & -4:02:31.320 & 0.336 & 1.44 & 9.02 & 75.8 & 19.0 & 13.8 & $5.58\pm$1.72 & $1.77\pm$0.65 & $1.02\pm$0.32 & $4.10\pm$1.52 &$2.19\pm$0.78 & $6.98\pm$2.86 & $1.10\pm$0.34  & $2.74\pm$0.94 & $1.24\pm$0.39 & $4.97\pm$1.84 & $8.53\pm$2.69 & $6.98\pm$2.25 & $1.26\pm$0.44\\
        & & & 0.259 & 1.11 & 6.94 & 58.3 & 14.6\\
        \hline
        P6 & 18:43:00.610 & -4:01:32.639 & 0.130 & 0.56 & 3.48 & 29.2 & 7.3 & 14.1 & $11.00\pm$3.40 & $3.51\pm$1.29 & $1.52\pm$0.48 & $6.11\pm$2.27 & & & $2.62\pm$0.81 & $1.91\pm$0.72 & $2.85\pm$0.89 & $11.40\pm$4.24 & $26.60\pm$8.29 & $3.31\pm$1.19 & $0.49\pm$0.18 \\
        & & & 0.187 & 0.80 & 4.99 & 42.1 & 10.5\\
        \hline
        P7 & 18:42:54.636 & -4:00:52.451 & 0.239 & 1.02 & 6.39 & 53.7 & 13.4 & 14.9 & $6.68\pm$2.06 & $2.12\pm$0.78 & $0.84\pm$0.26 & $3.37\pm$1.25 & & & $0.91\pm$0.28 & $1.78\pm$0.64 & $0.94\pm$0.30 & $3.79\pm$1.43 & $10.10\pm$3.28 & $2.76\pm$0.94 & $0.45\pm$0.16\\
        & & & 0.193 & 0.83 & 5.16 & 43.4 & 10.9\\
        \hline
        P8 & 18:42:55.289 & -4:01:21.835 & 0.270 & 1.15 & 7.21 & 60.5 & 15.1 & 13.6 & $5.79\pm$1.79 & $1.84\pm$0.68 & $0.69\pm$0.22 & $2.77\pm$1.04 & & & $0.80\pm$0.25 & $1.40\pm$0.51 & $0.91\pm$0.29 & $3.67\pm$1.38 & $10.50\pm$3.33 & $2.19\pm$0.73 & $0.33\pm$0.12\\
         & & & 0.195 & 0.83 & 5.21 & 43.9 & 11.0\\
        \hline
        P9 & 18:42:50.591 & -4:02:47.469 & 0.315 & 1.35 & 8.46 & 71.1 & 17.8 & 13.3 & $5.13\pm$1.58 & $1.63\pm$0.60 & $0.96\pm$0.30 & $3.84\pm$1.41 & & & $1.14\pm$0.35 & $3.47\pm$1.18 & $1.41\pm$0.44 & $5.66\pm$2.09 & $7.66\pm$2.40 & $9.16\pm$2.95 & $1.54\pm$0.54\\
        & & & 0.164 & 0.70 & 4.38 & 36.9 & 9.2\\
        \hline
        P10 & 18:42:47.860 & -4:03:08.458 & 0.171 & 0.73 & 4.58 & 38.5 & 9.6 & 13.6 & $6.43\pm$1.98 & $2.05\pm$0.75 & $1.36\pm$0.42 & $5.45\pm$2.01 & $1.40\pm$0.36 & $4.45\pm$1.45 & $1.47\pm$0.46 & $4.32\pm$1.49 & $1.88\pm$0.59 & $7.54\pm$2.80 & $10.00\pm$3.32 & $9.94\pm$3.21 & $1.93\pm$0.67\\
        & & & 0.116 & 0.50 & 3.11 & 26.1 & 6.5\\
        \hline
        \hline
    \end{tabular}
  \end{adjustbox}
  \vspace*{1mm}
  \caption{Estimated physical properties and molecular abundances observed by IRAM 30m towards IRDC G28.37+00.0, at 10 different positions.}
  \label{tab:landscape-tab}
  
\end{table}
\end{landscape}

==> chapters/tables/p10_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
     %Unweighted-unrestricted & 1.0e+07 & 600 & 1 & 1.0e-13 & 1.23e+03 & 8.65e-05\\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 1.0e+07 & 600 & 1 & 1.0e-13 & 1.23e+03 & 4.69e-03 \\
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 1.0e+04 & 15 & 20 & 4.6e-19 & 1.35e+06 & 1.13e-02 \\
    \hline
    \hline
    %\rule{0pt}{3ex}
   % Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 4.6e-19 & 1.38e+06 & 6.07e-01 \\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%15-25K
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 4.6e-19 & 1.38e+06 & 6.07e-01 \\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%10-20K
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 1.0e+04 & 15 & 100 & 2.2e-19 & 1.91e+06 & 4.14e-02 \\
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR18) & 1.0e+04 & 15 & 20 & 4.6e-19 & 1.35e+06 & 2.50e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 2.2e+04 & 15 & 20 & 4.6e-19 & 8.13e+05 & 7.16e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 2.2e-17 & 2.51e+04 & 2.58e+01 \\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 2.2e-17 & 2.57e+04 & 2.30e+01 \\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 2.2e+04 & 15 & 20 & 2.2e-14 & 5.25e+04 & 1.83e+01 \\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 100 & 4.6e-18 & 5.01e+07 & 2.05e+01 \\
    %\rule{0pt}{2ex}
    %WR + H2CO & 1.0e+04 & 25 & 20 & 1.0e-14 & 3.80e+04 & 3.96e+00 \\
    %\rule{0pt}{2ex}
    %\textcolor{magenta}{WRN18 + H2CO} & 1.0e+04 & 15 & 50 & 1.0e-19 & 3.02e+07 & 5.02e+00 \\
    %\rule{0pt}{4ex}
    %WR+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.28e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.25e+01 \\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 2.2e+04 & 20 & 100 & 2.2e-18 & 2.95e+06 & 2.55e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.71e+01 \\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 4.6e+04 & 15 & 100 & 1.0e-19 & 4.79e+05 & 5.72e-02 \\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 2.2e+05 & 15 & 20 & 1.0e-18 & 4.77e+04 & 2.72e-05 \\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 4.6e+05 & 15 & 20 & 1.0e-19 & 6.92e+04 & 1.94e-04 \\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 1.0e+05 & 15 & 50 & 4.6e-18 & 1.55e+05 & 4.74e-03 \\
    %\rule{0pt}{4ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 2.2e+05 & 15 & 50 & 1.0e-16 & 1.78e+06 & 1.25e-02 \\
    %\rule{0pt}{2ex}
    %ions(WR18) & 1.0e+05 & 15 & 100 & 4.6e-17 & 3.31e+06 & 6.95e-04 \\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 1.0e-17 & 3.31e+04 & 1.98e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 1.0e+05 & 15 & 50 & 1.0e-13 & 1.12e+04 & 2.09e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 1.0e+06 & 20 & 100 & 2.2e-18 & 4.79e+07 & 8.66e-01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 2.2e+04 & 20 & 100 & 2.2e-18 & 2.82e+06 & 2.67e+01\\
    %\rule{0pt}{5ex}
    %\hline
   % Weighted, ultra restricted (WUR) & 2.2e+04 & 15 & 20 & 1.0e-18 & 6.17e+05 & 6.45e-01\\
    %(2.2e4-1.0e5[cm$^{-3}$])\\
    %(20,50[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 2.2e+04 & 15 & 50 & 4.6e-19 & 7.94e+05 & 1.76e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 2.2e+04 & 15 & 20 & 1.0e-18 & 6.17e+05 & 3.15e-01\\
    %\rule{0pt}{2ex}
    %WURN18 & 2.2e+04 & 15 & 20 & 4.6e-19 & 8.13e+05 & 7.16e-01\\
    
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 2.2e+04 & 15 & 20 & 4.6e-19 & 8.51e+05 & 5.68e-01\\
    %\rule{0pt}{4ex}
   % WURN18 + HNCO,HNC,HCN & 1.0e+05 & 10 & 50 & 1.0e-17 & 2.24e+05 & 2.42e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 2.2e+04 & 15 & 50 & 2.2e-14 & 5.25e+04 & 2.34e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 2.2e+04 & 15 & 50 & 1.0e-19 & 9.77e+06 & 6.53e+00\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 2.2e+04 & 15 & 50 & 1.0e-19 & 2.14e+06 & 3.73e+01\\
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 2.2e+04 & 15 & 50 & 1.0e-19 & 1.07e+06 & 5.76e-03\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 1.0e+05 & 15 & 20 & 1.0e-18 & 3.39e+07 & 4.58e-02\\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 1.0e+05 & 15 & 20 & 1.0e-18 & 1.45e+05 & 1.03e-03\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 4.6e+04 & 15 & 20 & 2.2e-18 & 3.16e+05 & 1.49e-03\\
    %\hline
    Restricted & 1.0e+04 & 15 & 5 & 2.2e-19 & 1.86e+06 & 1.23e-01\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 2.2e+05 & 15 & 5 & 4.6e-19 & 1.15e+05 & 4.40e-04\\
    ions (R) & 1.0e+04 & 15 & 5 & 2.2e-19 & 2.00e+06 & 1.31e-04\\
    CO+ HCO$^+$ & 2.2e+04 & 25 & 100 & 4.6e-14 & 1.86e+03 & 5.70e-04\\
    CO+ N$_2$H$^+$ & 4.6e+04 & 15 & 5 & 2.2e-18 & 3.16e+05 & 2.83e-04\\
    \rule{0pt}{5ex}
     R+ CH$_3$OH,H$_2$CO & 1.0e+05 & 25 & 5 & 2.2e-19 & 1.00e+08 & 1.32e+01\\
    R+ H$_2$CO & 1.0e+04 & 20 & 5 & 1.0e-19 & 2.19e+07 & 8.12e-01\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 2.2e-15 & 1.05e+04 & 1.25e+01\\
    R+ N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 2.30e+01\\
    R+ N-group + H$_2$CO & 1.0e+06 & 10 & 100 & 2.2e-15 & 1.07e+04 & 1.67e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p10. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p10_different_fittings}
\end{table*}

==> chapters/tables/p1_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
    % Unweighted-unrestricted & 1.0e+04 & 900 & 3 & 1.0e-16 & 1.00e+06 & 1.37e-05\\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 1.0e+04 & 900 & 3 & 1.0e-16 & 1.00e+06 & 7.34e-04\\
    \hline
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 2.2e+04 & 15 & 50 & 2.2e-19 & 7.08e+05 & 1.41e-03 \\
    %\hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 2.2e+04 & 15 & 50 & 2.2e-19 & 7.08e+05 & 7.64e-02\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\ %(15-25K)
    %Weighted-restricted(WR) & 2.2e+04 & 15 & 50 & 2.2e-19 & 7.08e+05 & 7.64e-02\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\ %10-20 K
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 1.0e+05 & 15 & 100 & 1.0e-18 & 1.74e+05 & 1.02e-01 \\
    %\rule{0pt}{3ex}
    %WR18 & 1.0e+05 & 15 & 50 & 2.2e-18 & 1.41e+05 & 1.63e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 2.2e+05 & 15 & 100 & 4.6e-18 & 7.76e+04 & 7.14e-03\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{4ex}
    %WR + HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 1.0e-17 & 2.75e+04 & 1.81e+01\\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 1.0e-17 & 2.75e+04 & 1.65e+01\\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 1.42e+01\\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 1.44e+01\\
    %\rule{0pt}{2ex}
    %WR + H2CO & 2.2e+04 & 25 & 50 & 2.2e-14 & 3.24e+04 & 2.73e+00\\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 1.0e+06 & 20 & 100 & 1.0e-18 & 9.33e+07 & 2.92e+00\\
    %\rule{0pt}{4ex}
    %WR+N+C & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.35e+01\\
     %\rule{0pt}{2ex}
    %WRN+N+C & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.37e+01\\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.17e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.19e+01\\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 1.0e+05 & 15 & 20 & 1.0e-18 & 1.62e+05 & 4.06e-03\\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 1.0e+06 & 15 & 50 & 2.2e-18 & 2.45e+04 & 5.12e-04\\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 1.0e+05 & 15 & 20 & 2.2e-18 & 1.51e+05 & 2.74e-03\\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 2.2e+04 & 15 & 20 & 4.6e-18 & 3.72e+05 & 2.90e-03\\
    %\rule{0pt}{4ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 4.6e+05 & 20 & 50 & 4.6e-18 & 2.95e+07 & 1.25e-02\\
    %\rule{0pt}{2ex}
    %ions(WR18) & 2.2e+05 & 25 & 20 & 1.0e-13 & 1.23e+05 & 1.25e-03\\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.16e+04 & 1.47e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45e+04 & 1.67e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 1.0e+06 & 20 & 100 & 1.0e-18 & 9.77e+07 & 4.90e-01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 1.0e+05 & 20 & 100 & 4.6e-18 & 2.75e+06 & 1.75e+01\\
    %\hline
    %\rule{0pt}{5ex}
    %Weighted,Ultra restricted (WUR) & 4.6e+04 & 15 & 50 & 4.6e-19 & 3.31e+05 & 1.16e-01 \\
    %(4.6e4-2.2e5[cm$^{-3}$])\\
    %(50,100[mag], 10-15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 1.0e+05 & 15 & 100 & 1.0e-18 & 1.74e+05 & 1.02e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 1.0e+05 & 15 & 50 & 2.2e-18 & 1.41e+05 & 1.63e-01\\
    %\rule{0pt}{2ex}
    %WURN18 & 2.2e+05 & 15 & 100 & 4.6e-18 & 7.76e+04 & 7.14e-03\\%15-25K
    %WURN18 & 2.2e+05 & 15 & 100 & 4.6e-18 & 7.76e+04 & 7.14e-03\\%10-20K
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 2.2e+05 & 15 & 100 & 4.6e-18 & 7.76e+04 & 5.17e-03\\
    %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 1.0e+05 & 10 & 100 & 4.6e-18 & 2.57e+05 & 1.78e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.51e+04 & 1.76e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.57e+04 & 1.11e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 4.6e+04 & 15 & 100 & 2.2e-19 & 1.05e+06 & 4.05e+01\\
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 1.0e+05 & 15 & 50 & 4.6e-18 & 1.32e+05 & 1.44e-02\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 2.2e+05 & 15 & 100 & 4.6e-18 & 7.76e+04 & 6.35e-03 \\
    %\rule{0pt}{2ex}
   % CO + HCO$^+$ (WURN18) & 1.0e+05 & 15 & 50 & 2.2e-18 & 1.66e+05 & 1.23e-03\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 2.2e+05 & 15 & 100 & 4.6e-18 & 7.76e+04 & 8.32e-03\\
    \hline
    Restricted(R) & 2.2e+05 & 15 & 50 & 4.6e-18 & 7.59e+04 & 7.23e-02\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 1.0e+06 & 5 & 50 & 4.6e-16 & 2.24e+05 & 1.82e-05\\
    ions (R) & 1.0e+05 & 10 & 7 & 2.2e-17 & 4.17e+05 & 1.47e-04\\
    CO+ HCO$^+$ & 1.0e+06 & 10 & 50 & 1.0e-15 & 1.95e+04 & 2.38e-03\\
    CO+ N$_2$H$^+$ & 4.6e+05 & 10 & 5 & 2.2e-16 & 6.17e+04 & 1.89e-03\\
    \rule{0pt}{5ex}
    R+ CH$_3$OH,H$_2$CO & 2.2e+05 & 25 & 5 & 2.2e-19 & 1.00e+08 & 3.92e+00\\
    R+ H$_2$CO & 2.2e+04 & 20 & 5 & 1.0e-19 & 2.00e+07 & 6.45e-01\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 1.0e-15 & 1.20e+04 & 6.26e+00\\
    R + N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 9.12e+07 & 1.46e+01\\
    R+ N-group + H$_2$CO & 1.0e+06 & 30 & 50 & 4.6e-18 & 9.12e+07 & 1.50e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p1. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p1_different_fittings}
\end{table*}

==> chapters/tables/p2_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    %\rule{0pt}{2ex}
     %Unweighted-unrestricted & 1.0e+04 & 15 & 4 & 1.0e-19 & 1.66e+06 & 5.52e-04\\
    %\rule{0pt}{2ex}
    %Weighted-unrestricted & 1.0e+04 & 15 & 4 & 1.0e-19 & 1.66e+06 & 3.42e-02\\
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 1.0e+04 & 15 & 100 & 2.2e-19 & 2.04e+06 & 4.72e-03\\
    %\hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 50 & 2.2e-19 & 2.09e+06 & 2.96e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\ %15-25 K
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 50 & 2.2e-19 & 2.09e+06 & 2.96e-01\\ %10-20K
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 2.2e+04 & 15 & 20 & 4.6e-19 & 9.33e+05 & 3.09e-02 \\
    %\rule{0pt}{3ex}
    %WR18 & 2.2e+04 & 15 & 20 & 1.0e-18 & 7.08e+05 & 2.43e-02\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 1.0e+04 & 15 & 20 & 2.2e-19 & 2.34e+06 & 1.12e-02 \\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 2.2e-17 & 2.63e+04 & 2.54e+01\\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.09e+04 & 2.29e+01\\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 2.2e+04 & 15 & 20 & 2.2e-14 & 5.25e+04 & 2.16e+01\\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 100 & 4.6e-18 & 5.37e+07 & 2.08e+01\\
    %\rule{0pt}{2ex}
    %WR + H2CO & 1.0e+04 & 15 & 50 & 1.0e-19 & 2.75e+07 & 5.02e+00\\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 1.0e+04 & 15 & 50 & 1.0e-19 & 3.63e+07 & 2.99e+00\\
    %\rule{0pt}{4ex}
    %WR+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.44e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.46e+01\\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.96e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.98e+01 \\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 4.6e+04 & 15 & 20 & 1.0e-19 & 5.50e+05 & 1.89e-03  \\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.80e+05 & 1.01e-03  \\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 2.2e+04 & 15 & 20 & 4.6e-19 & 9.33e+05 & 2.04e-03 \\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 1.0e+04 & 15 & 20 & 1.0e-18 & 1.55e+06 & 2.10e-03 \\
    %\rule{0pt}{4ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 2.34e+06 & 1.46e-03 \\
    %\rule{0pt}{2ex}
    %ions(WR18) & 2.2e+05 & 15 & 100 & 1.0e-17 & 9.77e+04 & 8.30e-04\\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.47e+04 & 1.98e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 1.0e+04 & 15 & 100 & 1.0e-14 & 1.12e+05 & 2.18e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 1.0e+06 & 20 & 20 & 2.2e-18 & 4.79e+07 & 1.20e+00\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 1.0e+04 & 25 & 100 & 1.0e-18 & 2.09e+07 & 2.65e+01\\
    %\hline
    %Weighted, ultra restricted(WUR) & 4.6e+04 & 15 & 50 & 2.2e-18 & 3.39e+05 & 7.46e-01  \\
    %(4.6e4-2.2e5[cm$^{-3}$])\\
    %(50,100[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 4.6e+04 & 15 & 50 & 1.0e-18 & 4.17e+05 & 1.66e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 4.6e+04 & 15 & 100 & 2.2e-18 & 3.39e+05 & 9.75e-02\\
    %\rule{0pt}{2ex}
    %WURN18 & 4.6e+04 & 15 & 50 & 1.0e-18 & 4.17e+05 & 1.70e-01\\%15-25, 10-15K
    %\rule{0pt}{2ex}
   % WURN18(higher $\sigma$) & 4.6e+04 & 15 & 50 & 1.0e-18 & 4.27e+05 & 9.55e-02\\
    %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 2.2e+05 & 10 & 100 & 2.2e-17 & 1.10e+05 & 2.48e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.00e+04 & 2.62e+01 \\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 4.6e+04 & 15 & 100 & 2.2e-19 & 4.68e+06 & 1.25e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 2.2e+05 & 15 & 50 & 1.0e-18 & 1.78e+05 & 3.78e+01 \\
    
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 2.2e+05 & 15 & 100 & 4.6e-19 & 1.26e+05 & 2.19e-03\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 1.0e+05 & 15 & 50 & 2.2e-17 & 4.17e+06 & 3.17e-03\\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 1.0e+05 & 15 & 50 & 2.2e-18 & 1.74e+05 & 9.89e-04\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 4.6e+04 & 10 & 100 & 2.2e-16 & 6.03e+05 & 4.77e-03\\
    \hline
    Restricted & 1.0e+04 & 15 & 100 & 2.2e-19 & 2.29e+06 & 5.72e-02\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 1.0e+04 & 15 & 20 & 4.6e-19 & 1.86e+06 & 6.73e-04\\
    ions (R) & 4.6e+04 & 15 & 10 & 4.6e-19 & 6.92e+07 & 3.49e-03\\
    CO+ HCO$^+$ & 2.2e+04 & 10 & 5 & 1.0e-18 & 9.77e+05 & 3.11e-03\\
    CO+ N$_2$H$^+$ & 4.6e+05 & 25 & 10 & 1.0e-17 & 1.82e+07 & 6.18e-04\\
    \rule{0pt}{5ex}
     R+ CH$_3$OH,H$_2$CO & 1.0e+04 & 20 & 5 & 2.2e-19 & 3.63e+07 & 1.26e+01\\
    R+ H$_2$CO & 1.0e+04 & 20 & 5 & 1.0e-19 & 2.24e+07 & 9.15e-01\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 2.2e-15 & 1.02e+04 & 1.49e+01\\
    R+ N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 2.27e+01 \\
    R+ N-group + H$_2$CO & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 1.80e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p2. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag}
    \label{tab:p2_different_fittings}
\end{table*}

==> chapters/tables/p3_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
     %Unweighted-unrestricted & 2.2e+06 & 500 & 2 & 2.2e-14 & 1.58e+04 & 5.64e-04\\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 2.2e+06 & 500 & 2 & 2.2e-14 & 1.55e+04 & 3.24e-02 \\
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.91e+06 & 7.83e-03 \\
    \hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.96e+06 & 4.25e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\ %15-25K,10-20K
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.96e+06 & 4.28e-01\\%10-20K
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 1.0e+04 & 15 & 100 & 1.0e-19 & 2.82e+06 & 3.89e-01 \\
    %\rule{0pt}{3ex}
    %WR18 & 1.0e+04 & 15 & 100 & 2.2e-19 & 1.91e+06 & 1.03e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 1.0e+04 & 15 & 100 & 2.2e-19 & 2.09e+06 & 5.16e-02\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.02e+04 & 2.78e+01 \\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.09e+04 & 2.56e+01\\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 2.2e+04 & 15 & 100 & 2.2e-14 & 5.25e+04 & 2.17e+01 \\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 100 & 4.6e-18 & 5.25e+07 & 2.15e+01\\
    %\rule{0pt}{2ex}
    %WR + H2CO & 4.6e+05 & 20 & 50 & 1.0e-18 & 1.00e+08 & 6.79e+00 \\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 4.6e+05 & 20 & 50 & 1.0e-18 & 1.00e+08 & 4.62e+00\\
    %\rule{0pt}{4ex}
    %WR+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.70e+01\\
    %\rule{0pt}{2ex}
    %WRN+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.71e+01\\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.27e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.27e+01\\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 4.6e+04 & 15 & 20 & 1.0e-19 & 5.13e+05 & 2.58e-01\\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 1.0e+04 & 15 & 100 & 2.2e-19 & 1.86e+06 & 4.00e-04 \\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 4.6e+04 & 15 & 20 & 1.0e-19 & 5.62e+05 & 8.15e-03 \\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 1.0e+04 & 15 & 50 & 4.6e-19 & 1.70e+06 & 1.50e-03\\
    %\rule{0pt}{5ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 4.6e+05 & 15 & 20 & 1.0e-17 & 6.03e+04 & 2.52e-04 \\
    %\rule{0pt}{2ex}
    %ions(WR18) & 1.0e+06 & 15 & 20 & 4.6e-17 & 2.88e+04 & 2.28e-03\\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.47e+04 & 2.20e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 1.0e+05 & 15 & 50 & 1.0e-13 & 1.12e+04 & 2.25e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 1.0e+05 & 15 & 100 & 4.6e-19 & 6.76e+07 & 1.03e+00\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 1.0e+04 & 25 & 100 & 1.0e-18 & 1.91e+07 & 2.88e+01\\
    %\rule{0pt}{5ex}
    %\hline
    %Weighted, ultra restricted(WUR) & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.72e+05 & 8.15e-01\\
    %(4.6e4-2.2e5[cm$^{-3}$])\\
    %(50,100[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.98e+05 & 4.95e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 4.6e+04 & 15 & 100 & 2.2e-18 & 3.16e+05 & 2.26e-01\\
    %\rule{0pt}{2ex}
    %WURN18 & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.89e+05 & 1.91e-01\\%15-25, 10-15 K
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.98e+05 & 1.37e-01\\
     %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 2.2e+05 & 10 & 100 & 2.2e-17 & 1.10e+05 & 3.01e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45e+04 & 2.72e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 4.6e+04 & 15 & 100 & 2.2e-19 & 2.25e+06 & 1.38e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 4.6e+04 & 15 & 100 & 2.2e-19 & 9.77e+05 & 4.47e+01\\
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 2.2e+05 & 15 & 100 & 1.0e-18 & 1.12e+05 & 1.05e-02\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 4.6e+04 & 15 & 50 & 4.6e-19 & 7.24e+07 & 1.24e-02 \\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 2.2e+05 & 15 & 50 & 4.6e-18 & 7.59e+04 & 2.84e-02\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 1.0e+05 & 15 & 50 & 4.6e-18 & 1.66e+05 & 1.97e-03\\
    \hline
    Restricted & 1.0e+04 & 15 & 50 & 2.2e-19 & 2.04e+06 & 5.68e-02\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 1.0e+04 & 15 & 20 & 4.6e-19 & 1.70e+06 & 1.81e-04\\
    ions (R) & 1.0e+06 & 5 & 7 & 1.0e-13 & 1.91e+04 & 7.74e-04\\
    CO+ HCO$^+$ & 2.2e+04 & 10 & 5 & 1.0e-18 & 9.12e+05 & 1.55e-03\\
    CO+ N$_2$H$^+$ & 1.0e+04 & 15 & 5 & 2.2e-19 & 2.04e+06 & 3.63e-04\\
    \rule{0pt}{5ex}
    R+ CH$_3$OH,H$_2$CO & 1.0e+05 & 25 & 5 & 2.2e-19 & 1.00e+08 & 1.33e+01\\
    R+ H$_2$CO & 1.0e+04 & 20 & 5 & 1.0e-19 & 2.19e+07 & 7.53e-01\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 2.2e-15 & 1.05e+04 & 1.65e+01\\
    R + N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 2.64e+01 \\
    R+ N-group + H$_2$CO & 1.0e+04 & 30 & 100 & 1.0e-18 & 2.19e+07 & 2.09e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p3. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p3_different_fittings}
\end{table*}

==> chapters/tables/p4_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
     %Unweighted-unrestricted & 1.0e+07 & 500 & 1 & 1.0e-13 & 6.03e+04 & 7.19e-04\\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 2.2e+06 & 500 & 2 & 2.2e-14 & 1.17e+04 & 3.89e-02 \\
    %\rule{0pt}{2ex}
    %unweighted-restricted & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.86e+06 & 6.03e-03 \\
    \hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.91e+06 & 3.55e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%15-25K
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.91e+06 & 3.55e-01\\%10-20K
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 2.2e+04 & 15 & 20 & 4.6e-19 & 8.51e+05 & 1.66e-01\\
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR18) & 2.2e+04 & 15 & 20 & 1.0e-18 & 6.61e+05 & 2.28e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 2.2e+04 & 15 & 20 & 4.6e-19 & 8.51e+05 & 1.70e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 2.95e+04 & 2.56e+01\\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.02e+04 & 2.31e+01\\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 2.2e+04 & 15 & 100 & 2.2e-14 & 5.25e+04 & 1.97e+01 \\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 100 & 4.6e-18 & 5.25e+07 & 1.95e+01\\
    %\rule{0pt}{2ex}
    %WR + H2CO & 1.0e+04 & 25 & 20 & 1.0e-14 & 3.80e+04 & 6.57e+00\\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 4.6e+05 & 20 & 50 & 1.0e-18 & 1.00e+08 & 5.23e+00\\
    %\rule{0pt}{4ex}
    %WR+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.21e+01\\
    %\rule{0pt}{2ex}
    %WRN+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.20e+01\\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.84e+01\\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.84e+01 \\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 4.6e+04 & 15 & 20 & 1.0e-19 & 5.13e+05 & 8.69e-02\\
    %\rule{0pt}{2ex}
    %Ratio(WR18) &  2.2e+05 & 15 & 20 & 2.2e-19 & 1.23e+05 & 1.83e-03\\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 1.0e+04 & 15 & 100 & 1.0e-19 & 2.63e+06 & 3.68e-04\\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 2.2e+04 & 15 & 20 & 1.0e-18 & 7.24e+05 & 1.22e-02\\
    %\rule{0pt}{5ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 1.0e+05 & 15 & 100 & 2.2e-18 & 2.09e+05 & 2.93e-03\\
    %\rule{0pt}{2ex}
    %ions(WR18) & 4.6e+04 & 15 & 50 & 4.6e-19 & 7.24e+07 & 1.36e-03\\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.47e+04 & 1.87e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 1.0e+05 & 15 & 50 & 1.0e-13 & 1.12e+04 & 2.06e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 2.2e+04 & 15 & 20 & 1.0e-19 & 2.19e+07 & 1.17e+00\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 1.0e+04 & 25 & 100 & 1.0e-18 & 1.66e+07 & 2.55e+01\\
    %\rule{0pt}{5ex}
    %\hline
    %Weighted, ultra restricted (WUR) & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.72e+05 & 1.03e+00\\
    %(4.6e4-2.2e5[cm$^{-3}$])\\
    %(50,100[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.89e+05 & 3.01e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 4.6e+04 & 15 & 100 & 2.2e-18 & 3.16e+05 & 2.78e-01\\
    %\rule{0pt}{2ex}
    %WURN18 & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.89e+05 & 3.06e-01\\%15-25, 10-15K
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 4.6e+04 & 15 & 100 & 1.0e-18 & 4.07e+05 & 1.83e-01\\
    %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 1.0e+05 & 10 & 100 & 1.0e-17 & 2.24e+05 & 2.70e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45e+04 & 2.37e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 4.6e+04 & 15 & 100 & 2.2e-19 & 4.17e+06 & 1.35e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 4.6e+04 & 15 & 100 & 2.2e-19 & 9.77e+05 & 3.91e+01\\
    
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 1.0e+05 & 15 & 50 & 1.0e-19 & 2.75e+05 & 7.16e-03\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 1.0e+05 & 15 & 50 & 1.0e-18 & 3.31e+07 & 1.72e-02\\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 2.2e+05 & 10 & 100 & 4.6e-18 & 8.91e+04 & 2.03e-02\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 2.2e+05 & 15 & 50 & 2.2e-17 & 7.24e+04 & 7.17e-03\\
    \hline
    Restricted & 1.0e+04 & 15 & 7 & 2.2e-19 & 2.04e+06 & 1.17e-03\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 4.6e+05 & 15 & 5 & 2.2e-19 & 6.76e+04 & 1.39e-05\\
    ions (R) & 1.0e+05 & 5 & 10 & 1.0e-14 & 2.00e+05 & 7.86e-05\\
    CO+ HCO$^+$ & 1.0e+04 & 15 & 7 & 2.2e-19 & 2.04e+06 & 6.81e-04\\
    CO+ N$_2$H$^+$ & 1.0e+06 & 10 & 5 & 4.6e-15 & 2.88e+04 & 1.72e-06\\
    \rule{0pt}{5ex}
     R+ CH$_3$OH,H$_2$CO & 1.0e+05 & 25 & 5 & 2.2e-19 & 1.00e+08 & 1.16e+01\\
    R+ H$_2$CO & 1.0e+04 & 20 & 5 & 1.0e-19 & 2.19e+07 & 6.02e-01\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 2.2e-15 & 1.05e+04 & 1.39e+01\\
    R+ N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 2.17e+01 \\
    R+ N-group + H$_2$CO & 1.0e+04 & 30 & 20 & 1.0e-18 & 2.19e+07 & 1.85e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p4. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p4_different_fittings}
\end{table*}

==> chapters/tables/p5_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
     %Unweighted-unrestricted & 4.6e+03 & 500 & 5 & 4.6e-17 & 1.15e+07 & 1.15e-04\\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 4.6e+03 & 500 & 5 & 4.6e-17 & 1.17e+07 & 6.18e-03 \\
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 2.2e+04 & 15 & 20 & 4.6e-19 & 7.24e+05 & 5.64e-03 \\
    \hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 2.2e+04 & 15 & 20 & 4.6e-19 & 7.24e+05 & 3.02e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%15-25K
    %Weighted-restricted(WR) & 2.2e+04 & 15 & 20 & 4.6e-19 & 7.24e+05 & 3.02e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%10-20K
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 1.0e+04 & 15 & 100 & 1.0e-19 & 2.24e+06 & 1.88e-01\\
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR18) & 1.0e+04 & 15 & 50 & 2.2e-19 & 1.62e+06 & 7.88e-02\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 1.0e+05 & 15 & 20 & 4.6e-18 & 1.48e+05 & 5.69e-02\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 2.88e+04 & 2.33e+01\\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 2.88e+04 & 2.16e+01 \\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45e+04 & 1.78e+01\\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 100 & 4.6e-18 & 4.90e+07 & 1.84e+01\\
    %\rule{0pt}{2ex}
    %WR + H2CO & 1.0e+05 & 25 & 100 & 1.0e-13 & 6.76e+03 & 5.23e+00 \\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 4.6e+05 & 20 & 100 & 1.0e-18 & 1.00e+08 & 3.61e+00 \\
    %\rule{0pt}{4ex}
    %WR+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.91e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.90e+01\\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.50e+01\\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.50e+01\\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](ratio)$_{(WR)}$ & 4.6e+04 & 15 & 20 & 1.0e-19 & 4.79e+05 & 5.18e-02\\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 1.0e+06 & 15 & 20 & 1.0e-19 & 3.39e+04 & 3.75e-03\\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 1.0e+04 & 15 & 20 & 1.0e-19 & 2.19e+06 & 4.58e-03\\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 1.0e+06 & 15 & 50 & 4.6e-19 & 3.09e+04 & 3.93e-04\\
    %\rule{0pt}{4ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 1.0e+05 & 15 & 100 & 1.0e-18 & 3.55e+07 & 4.21e-03\\
    %\rule{0pt}{2ex}
    %ions(WR18) & 4.6e+04 & 20 & 100 & 2.2e-18 & 8.32e+07 & 6.48e-03\\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.39e+04 & 1.76e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 2.2e+04 & 15 & 20 & 2.2e-14 & 5.25e+04 & 1.92e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 1.0e+06 & 20 & 100 & 2.2e-18 & 4.68e+07 & 1.04e+00\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 1.0e+04 & 25 & 100 & 1.0e-18 & 1.32e+07 & 2.23e+01\\
    %\rule{0pt}{5ex}
    %\hline
    %Weighted, ultra restricted (WUR) & 4.6e+04 & 15 & 100 & 1.0e-18 & 3.39e+05 & 4.71e-01\\
    %(4.6e4-2.2e5[cm$^{-3}$])\\
    %(50,100[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 4.6e+04 & 15 & 100 & 1.0e-18 & 3.55e+05 & 2.13e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 4.6e+04 & 15 & 100 & 2.2e-18 & 2.82e+05 & 1.97e-01\\
    %\rule{0pt}{2ex}
    %WURN18 & 1.0e+05 & 15 & 50 & 4.6e-18 & 1.48e+05 & 5.69e-02\\%15-25, 10-15 K
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 1.0e+05 & 15 & 100 & 4.6e-18 & 1.48e+05 & 3.87e-02\\
    %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 4.6e+04 & 10 & 100 & 4.6e-18 & 4.68e+05 & 2.50e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45e+04 & 2.21e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 1.0e+05 & 15 & 50 & 1.0e-13 & 1.17e+04 & 1.38e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 4.6e+04 & 15 & 100 & 2.2e-19 & 1.00e+06 & 3.99e+01\\
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 2.2e+05 & 15 & 50 & 4.6e-18 & 8.51e+04 & 9.69e-03\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 4.6e+04 & 15 & 50 & 1.0e-18 & 3.98e+07 & 1.70e-03\\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 4.6e+04 & 15 & 100 & 2.2e-18 & 3.47e+05 & 1.44e-02\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 4.6e+04 & 15 & 100 & 1.0e-18 & 3.55e+05 & 2.72e-02\\
    \hline
    Restricted & 1.0e+05 & 15 & 5 & 4.6e-18 & 1.48e+05 & 8.12e-02\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 1.0e+06 & 5 & 50 & 2.2e-16 & 1.86e+05 & 2.79e-03\\
    ions (R) & 4.6e+05 & 25 & 50 & 4.6e-17 & 6.03e+06 & 1.56e-03\\
    CO+ HCO$^+$ & 4.6e+04 & 10 & 10 & 2.2e-18 & 3.98e+05 & 1.81e-03\\
    CO+ N$_2$H$^+$ & 1.0e+06 & 10 & 7 & 2.2e-15 & 2.75e+04 & 1.25e-03\\
    \rule{0pt}{5ex}
    R+ CH$_3$OH,H$_2$CO & 1.0e+05 & 25 & 5 & 2.2e-19 & 1.00e+08 & 8.93e+00\\
    R+ H$_2$CO & 1.0e+04 & 20 & 5 & 1.0e-19 & 2.14e+07 & 7.53e-01\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 1.0e-15 & 1.15e+04 & 1.14e+01\\
    R+ N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 1.88e+01\\
    R+ N-group + H$_2$CO & 1.0e+04 & 30 & 100 & 1.0e-18 & 2.19e+07 & 1.54e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p5. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p5_different_fittings}
\end{table*}

==> chapters/tables/p6_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [$s^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
     %Unweighted-unrestricted & 2.2e+03 & 450 & 7 & 2.2e-17 & 6.46e+06 & 5.86e-04\\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 2.2e+03 & 450 & 7 & 2.2e-17 & 6.46e+06 & 3.15e-02\\
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 1.0e+04 & 15 & 20 & 1.0e-18 & 1.15e+06 & 3.55e-02 \\
    \hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 1.0e-18 & 1.17e+06 & 1.93e+00\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%15-25K
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 1.0e-18 & 1.17e+06 & 1.93e+00\\%10-20K
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 1.0e+04 & 15 & 20 & 4.6e-19 & 1.66e+06 & 1.32e+00\\
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR18) & 1.0e+04 & 15 & 20 & 4.6e-19 & 1.48e+06 & 2.41e+00\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 1.0e+04 & 15 & 20 & 2.2e-19 & 2.14e+06 & 3.68e+00\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 1.0e+04 & 20 & 100 & 1.0e-18 & 6.31e+06 & 1.71e+01\\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 4.6e+05 & 15 & 100 & 1.0e-17 & 5.01e+04 & 1.77e+01 \\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45e+04 & 2.54e+01\\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45e+04 & 2.64e+01 \\
    %\rule{0pt}{2ex}
    %WR + H2CO & 1.0e+04 & 25 & 20 & 1.0e-14 & 6.76e+04 & 9.77e+00 \\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 1.0e+04 & 25 & 20 & 1.0e-14 & 6.76e+04 & 1.08e+01 \\
    %\rule{0pt}{4ex}
    %WR+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.60e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.52e+01 \\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 1.0e+05 & 20 & 100 & 1.0e-17 & 3.98e+05 & 1.86e+01\\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 1.0e+05 & 20 & 100 & 1.0e-17 & 3.98e+05 & 1.99e+01\\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 4.6e+04 & 15 & 20 & 1.0e-19 & 4.79e+05 & 5.96e-01 \\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.62e+06 & 1.12e-02\\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 2.2e+04 & 15 & 20 & 1.0e-19 & 1.05e+06 & 3.64e-02\\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 1.0e+06 & 15 & 100 & 2.2e-19 & 3.31e+04 & 4.35e-03\\
    %\rule{0pt}{5ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 1.0e+04 & 15 & 20 & 1.0e-19 & 2.75e+07 & 3.25e-03 \\
    %\rule{0pt}{2ex}
    %ions(WR18) & 4.6e+04 & 15 & 20 & 1.0e-18 & 3.47e+07 & 1.82e-03 \\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.39e+04 & 1.09e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 1.0e+06 & 25 & 100 & 4.6e-18 & 5.89e+07 & 2.94e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 2.2e+04 & 15 & 100 & 1.0e-19 & 3.72e+07 & 3.22e+00\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 1.0e+05 & 20 & 50 & 1.0e-17 & 3.89e+05 & 2.16e+01\\
    %\rule{0pt}{5ex}
    %\hline
    %Weighted, ultra restricted (WUR) & 2.2e+04 & 15 & 20 & 2.2e-18 & 5.37e+05 & 2.19e+00\\
    %(2.2e4-1.0e5[cm-3])\\
    %(20,50[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 2.2e+04 & 15 & 20 & 1.0e-18 & 7.24e+05 & 1.70e+00\\
    %\rule{0pt}{2ex}
    %WUR18 & 2.2e+04 & 15 & 20 & 2.2e-18 & 5.50e+05 & 3.00e+00\\
    %\rule{0pt}{2ex}
    %WURN18 & 2.2e+04 & 15 & 20 & 4.6e-19 & 8.71e+05 & 4.29e+00\\%15-25, 10-15 K
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 2.2e+04 & 15 & 20 & 4.6e-19 & 1.02e+06 & 1.97e+00\\
    %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 1.0e+05 & 15 & 50 & 1.0e-18 & 2.75e+05 & 2.03e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 4.6e+04 & 15 & 50 & 4.6e-14 & 2.45e+04 & 2.41e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 2.2e+04 & 15 & 50 & 1.0e-19 & 2.19e+07 & 1.40e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 2.2e+04 & 15 & 50 & 1.0e-19 & 2.40e+06 & 3.32e+01\\
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 4.6e+04 & 15 & 20 & 2.2e-19 & 4.68e+05 & 1.14e-02\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 4.6e+04 & 15 & 20 & 1.0e-18 & 5.50e+05 & 3.74e-03\\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 1.0e+05 & 15 & 20 & 1.0e-18 & 1.05e+05 & 2.16e-02\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 4.6e+04 & 15 & 20 & 1.0e-17 & 2.29e+05 & 8.32e-03\\
    \hline
    Restricted & 1.0e+04 & 5 & 7 & 1.0e-15 & 2.04e+06 & 2.01e+00\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow) & 1.0e+04 & 15 & 5 & 4.6e-19 & 1.66e+06 & 2.35e+00\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 2.2e+04 & 5 & 100 & 1.0e-18 & 2.45e+07 & 1.85e-03\\
    ions (R) & 1.0e+05 & 15 & 5 & 2.2e-17 & 5.50e+06 & 2.05e-03\\
    CO+ HCO$^+$ & 2.2e+05 & 10 & 7 & 4.6e-18 & 5.75e+04 & 9.52e-06\\
    CO+ N$_2$H$^+$ & 4.6e+05 & 10 & 7 & 2.2e-15 & 4.17e+04 & 1.94e-03\\
    \rule{0pt}{5ex}
    R+ CH$_3$OH,H$_2$CO & 1.0e+04 & 20 & 5 & 2.2e-19 & 2.82e+07 & 1.65e+01\\
    R+ H$_2$CO & 1.0e+04 & 20 & 5 & 1.0e-19 & 2.19e+07 & 7.28e+00\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 4.6e-15 & 9.33e+03 & 8.23e+00\\
    R+ N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 1.79e+01\\
    R+ N-group + H$_2$CO & 1.0e+04 & 30 & 10 & 1.0e-18 & 1.91e+07 & 1.87e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p6. The restricted fitting have been performed through the models with n(H) in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p6_different_fittings}
\end{table*}

==> chapters/tables/p7_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
     %Unweighted-unrestricted & 4.6e+04 & 15 & 2 & 1.0e-17 & 1.00e+08 & 1.43e-03\\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 2.2e+03 & 600 & 5 & 2.2e-17 & 7.59e+06 & 7.79e-02 \\
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.45e+06 & 5.31e-03\\
    \hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.45e+06 & 2.85e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%15-25K
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.45e+06 & 2.85e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%10-20K
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 1.0e+04 & 15 & 20 & 1.0e-19 & 2.00e+06 & 2.09e-01 \\
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR18) & 4.6e+04 & 15 & 20 & 2.2e-18 & 2.57e+05 & 1.64e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 1.0e+04 & 15 & 100 & 1.0e-19 & 2.00e+06 & 1.72e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 4.6e+05 & 25 & 100 & 2.2e-18 & 1.00e+08 & 2.08e+01 \\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 1.0e-17 & 2.75e+04 & 1.92e+01\\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 2.2e+04 & 15 & 100 & 2.2e-14 & 5.37e+04 & 1.72e+01 \\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 1.78e+01 \\
    %\rule{0pt}{2ex}
    %WR + H2CO & 1.0e+04 & 25 & 20 & 1.0e-14 & 6.92e+04 & 3.74e+00 \\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 2.2e+04 & 25 & 100 & 2.2e-14 & 3.16e+04 & 6.18e+00 \\
    %\rule{0pt}{4ex}
    %WR+N+C & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.36e+01\\
    %\rule{0pt}{2ex}
    %WRN+N+C & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.35e+01\\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.28e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.28e+01\\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 4.6e+04 & 15 & 20 & 1.0e-19 & 4.37e+05 & 7.56e-02\\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 1.0e+05 & 15 & 20 & 1.0e-18 & 1.66e+05 & 4.55e-03\\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 1.0e+04 & 15 & 50 & 1.0e-19 & 1.91e+06 & 2.93e-03 \\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 4.6e+04 & 15 & 20 & 2.2e-18 & 2.75e+05 & 3.66e-03\\
    %\rule{0pt}{5ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 1.0e+06 & 15 & 20 & 2.2e-17 & 2.82e+04 & 5.36e-03 \\
    %\rule{0pt}{2ex}
    %ions(WR18) & 2.2e+05 & 25 & 100 & 2.2e-17 & 1.23e+07 & 7.86e-04 \\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.16e+04 & 1.61e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45e+04 & 2.06e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 1.0e+06 & 20 & 100 & 1.0e-18 & 1.00e+08 & 1.88e+00\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 2.2e+05 & 20 & 100 & 1.0e-17 & 8.32e+05 & 2.17e+01\\
    %\rule{0pt}{5ex}
    %\hline
   % Weighted, ultra restricted (WUR) & 2.2e+04 & 15 & 20 & 4.6e-19 & 6.46e+05 & 3.27e-01\\
    %(2.2e4-1.0e5[cm$^{-3}$])\\
    %(20,50,100[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 2.2e+04 & 15 & 100 & 2.2e-19 & 8.32e+05 & 3.85e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 4.6e+04 & 15 & 20 & 2.2e-18 & 2.57e+05 & 1.62e-01\\
    %\rule{0pt}{2ex}
    %WURN18 & 2.2e+04 & 15 & 100 & 2.2e-19 & 8.32e+05 & 3.76e-01\\%15-25, 10-15 K
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 2.2e+04 & 15 & 50 & 2.2e-19 & 8.51e+05 & 1.65e-01\\
    %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 2.2e+04 & 10 & 20 & 1.0e-18 & 1.23e+06 & 2.49e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 2.2e+04 & 15 & 100 & 2.2e-14 & 5.37e+04 & 1.92e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 2.2e+04 & 15 & 50 & 1.0e-19 & 1.70e+07 & 1.37e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 2.2e+04 & 15 & 100 & 1.0e-19 & 2.34e+06 & 3.87e+01\\
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 2.2e+04 & 15 & 20 & 4.6e-19 & 6.92e+05 & 1.56e-02\\
    %\rule{0pt}{2ex}
    %ions (WUR18) & 2.2e+04 & 15 & 100 & 2.2e-19 & 8.91e+05 & 2.29e-02\\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 1.0e+05 & 15 & 20 & 1.0e-18 & 1.41e+05 & 1.91e-03\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 1.0e+05 & 15 & 100 & 4.6e-18 & 1.38e+05 & 1.93e-02\\
    \hline
    Restricted & 2.2e+04 & 15 & 5 & 4.6e-19 & 6.92e+05 & 6.78e-02\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 4.6e+04 & 10 & 5 & 1.0e-19 & 1.07e+06 & 1.70e-03\\
    ions (R) & 1.0e+05 & 15 & 7 & 4.6e-18 & 1.15e+07 & 8.36e-05\\
    CO+ HCO$^+$ & 1.0e+04 & 25 & 7 & 2.2e-14 & 3.98e+03 & 5.31e-05\\
    CO+ N$_2$H$^+$ & 4.6e+04 & 10 & 5 & 1.0e-17 & 3.63e+05 & 6.45e-04\\
    \rule{0pt}{5ex}
     R+ CH$_3$OH,H$_2$CO & 2.2e+05 & 25 & 5 & 2.2e-19 & 1.00e+08 & 7.23e+00\\
    R+ H$_2$CO & 2.2e+04 & 20 & 5 & 1.0e-19 & 2.04e+07 & 1.81e+00\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 1.0e-15 & 1.20e+04 & 9.02e+00\\
    R+ N-group + C-group & 1.0e+06 & 30 & 20 & 4.6e-18 & 9.33e+07 & 1.72e+01\\
    R+ N-group + H$_2$CO & 1.0e+04 & 30 & 10 & 4.6e-19 & 3.47e+07 & 1.82e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p7. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p7_different_fittings}
\end{table*}

==> chapters/tables/p8_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
     %Unweighted-unrestricted & 4.6e+04 & 15 & 2 & 2.2e-19 & 2.88e+05 & 1.13e-04 \\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 4.6e+04 & 15 & 2 & 2.2e-19 & 2.88e+05 & 5.80e-03 \\
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 1.0e+04 & 15 & 100 & 1.0e-19 & 1.78e+06 & 4.16e-03 \\
    \hline
    \hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 100 & 1.0e-19 & 1.82e+06 & 2.57e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%15-25K
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 100 & 1.0e-19 & 1.82e+06 & 2.57e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%10-20K
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 2.2e+04 & 15 & 20 & 2.2e-19 & 8.13e+05 & 2.81e-01 \\
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR18) & 1.0e+05 & 15 & 20 & 4.6e-18 & 1.29e+05 & 1.49e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 1.0e+04 & 15 & 20 & 1.0e-19 & 1.95e+06 & 4.62e-03\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 4.6e+05 & 25 & 100 & 2.2e-18 & 1.00e+08 & 1.71e+01\\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 1.0e-17 & 2.69e+04 & 1.57e+01 \\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 1.82e+01 \\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 1.82e+01 \\
    %\rule{0pt}{2ex}
    %WR + H2CO & 1.0e+04 & 25 & 50 & 1.0e-14 & 6.92e+04 & 4.19e+00\\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 1.0e+06 & 20 & 100 & 1.0e-18 & 9.33e+07 & 6.62e+00 \\
    %\rule{0pt}{4ex}
    %WR+N+C & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.12e+01\\
    %\rule{0pt}{2ex}
    %WRN+N+C & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.12e+01\\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.11e+01\\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.11e+01 \\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 1.0e+05 & 15 & 20 & 1.0e-19 & 2.29e+05 & 4.27e-02 \\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 4.6e+05 & 15 & 20 & 2.2e-19 & 5.89e+04 & 4.79e-03 \\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 2.2e+05 & 15 & 50 & 1.0e-19 & 1.26e+05 & 4.70e-03\\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 1.0e+06 & 15 & 20 & 4.6e-19 & 2.95e+04 & 3.75e-03\\
    %\rule{0pt}{4ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 1.0e+05 & 15 & 50 & 1.0e-18 & 3.72e+07 & 1.31e-04 \\
    %\rule{0pt}{2ex}
    %ions(WR18) & 1.0e+05 & 15 & 20 & 4.6e-17 & 3.89e+06 & 9.91e-04 \\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 4.6e-18 & 3.55e+04 & 1.37e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 1.0e+06 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.09e+01\\
    
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 1.0e+06 & 20 & 50 & 1.0e-18 & 1.00e+08 & 3.28e+00\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 2.2e+05 & 20 & 100 & 1.0e-17 & 6.76e+05 & 1.94e+01\\
    %\rule{0pt}{5ex}
    %\hline
    %Weighted, ultra restricted (WUR) & 2.2e+04 & 15 & 20 & 4.6e-19 & 6.46e+05 & 3.49e-01\\
    %(2.2e4-1.0e5[cm$^{-3}$])\\
    %(20,50,100[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 2.2e+04 & 15 & 50 & 2.2e-19 & 8.13e+05 & 2.81e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 1.0e+05 & 15 & 20 & 4.6e-18 & 1.29e+05 & 1.48e-01\\
    %\rule{0pt}{2ex}
    %WURN18 & 2.2e+04 & 15 & 50 & 2.2e-19 & 8.13e+05 & 5.21e-02\\%15-25, 10-15K
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 2.2e+04 & 15 & 100 & 2.2e-19 & 8.32e+05 & 2.65e-02\\
    %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 1.0e+05 & 10 & 100 & 4.6e-18 & 2.40e+05 & 2.38e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.51e+04 & 1.89e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 2.2e+04 & 15 & 50 & 1.0e-19 & 1.78e+07 & 1.49e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 2.2e+04 & 15 & 100 & 1.0e-19 & 2.40e+06 & 3.76e+01\\
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 2.2e+04 & 15 & 20 & 4.6e-19 & 6.92e+05 & 1.25e-02\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 2.2e+04 & 15 & 50 & 2.2e-19 & 8.32e+05 & 5.75e-03\\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 1.0e+05 & 15 & 50 & 1.0e-18 & 1.51e+05 & 2.92e-04\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 1.0e+05 & 15 & 50 & 2.2e-18 & 1.58e+05 & 5.98e-02\\
    %\hline
    Restricted & 1.0e+04 & 20 & 5 & 1.0e-19 & 2.04e+07 & 2.95e-02\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
    \rule{0pt}{2ex}
    Ratio (R) & 2.2e+04 & 5 & 100 & 1.0e-18 & 1.95e+07 & 7.62e-04\\
    ions (R) & 1.0e+05 & 15 & 5 & 1.0e-17 & 1.55e+07 & 2.14e-04\\
    CO+ HCO$^+$ & 1.0e+06 & 10 & 50 & 4.6e-16 & 1.82e+04 & 1.49e-03\\
    CO+ N$_2$H$^+$ & 1.0e+06 & 10 & 100 & 2.2e-15 & 1.74e+04 & 7.43e-05\\
    \rule{0pt}{5ex}
     R+ CH$_3$OH,H$_2$CO & 2.2e+05 & 25 & 5 & 2.2e-19 & 2.88e+07 & 6.06e+00\\
    R+ H$_2$CO & 4.6e+04 & 20 & 5 & 1.0e-19 & 2.09e+07 & 1.89e+00\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 1.0e-15 & 1.35e+04 & 8.33e+00\\
    R+ N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 9.12e+07 & 1.67e+01\\
    R+ N-group + H$_2$CO & 1.0e+04 & 30 & 10 & 4.6e-19 & 3.47e+07 & 1.78e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p8. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p8_different_fittings}
\end{table*}

==> chapters/tables/p9_fittings.tex <==
\begin{table*}[ht]
    \centering
    \addtolength{\leftskip} {-2cm}
    \addtolength{\rightskip}{-2cm}
    \begin{tabular}{p{0.26\linewidth}p{0.09\linewidth}p{0.06\linewidth}p{0.07\linewidth}p{0.08\linewidth}p{0.08\linewidth}p{0.1\linewidth}}
    \hline
    \hline
     Fitting & n(H) & T & A$_v$ & $\zeta$ & Time & $\chi^2$\\
     & [cm$^{-3}$] & [K] & [mag] & [s$^{-1}$] & [year] &\\
    \hline
    \rule{0pt}{2ex}
     %Unweighted-unrestricted & 2.2e+04 & 500 & 4 & 2.2e-16 & 3.02e+06 & 2.04e-04\\
    %\rule{0pt}{2ex}
    Weighted-unrestricted & 2.2e+04 & 500 & 4 & 2.2e-16 & 3.16e+06 & 1.16e-02 \\
    %\rule{0pt}{2ex}
    %Unweighted-restricted & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.66e+06 & 4.94e-03\\
    \hline
    \hline
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.70e+06 & 2.67e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%15-25K
    %Weighted-restricted(WR) & 1.0e+04 & 15 & 20 & 2.2e-19 & 1.70e+06 & 2.67e-01\\
    %(CO,HCO$^+$(C13),N$_2$H$^+$)\\%10-20K
    %\rule{0pt}{3ex}
    %Narrower velocity range(WRN) & 1.0e+04 & 15 & 100 & 1.0e-19 & 2.34e+06 & 1.06e-01\\
    %\rule{0pt}{3ex}
    %Weighted-restricted(WR18) & 4.6e+04 & 15 & 20 & 2.2e-18 & 2.88e+05 & 1.27e-01\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{3ex}
    %WRN18 & 1.0e+04 & 15 & 100 & 1.0e-19 & 2.34e+06 & 9.42e-02\\
    %(CO,HCO$^+$(O18),N$_2$H$^+$)\\
    %\rule{0pt}{5ex}
    %WR + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 2.95e+04 & 2.65e+01\\
    %\rule{0pt}{2ex}
    %WRN + HNCO,HNC,HCN & 1.0e+06 & 15 & 100 & 1.0e-17 & 3.02e+04 & 2.36e+01 \\
    %\rule{0pt}{4ex}
    %WR + CH3OH,H2CO & 2.2e+04 & 15 & 100 & 2.2e-14 & 5.25e+04 & 1.79e+01\\
    %\rule{0pt}{2ex}
    %WRN + CH3OH,H2CO & 1.0e+06 & 25 & 100 & 4.6e-18 & 5.01e+07 & 1.84e+01\\
    %\rule{0pt}{2ex}
    %WR + H2CO & 1.0e+04 & 25 & 20 & 1.0e-14 & 3.80e+04 & 4.96e+00 \\
    %\rule{0pt}{2ex}
    %WRN18 + H2CO & 4.6e+05 & 20 & 50 & 1.0e-18 & 1.00e+08 & 3.36e+00  \\
    %\rule{0pt}{4ex}
    %WR+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.29e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 3.29e+01 \\
    %\rule{0pt}{2ex}
    %WR+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.88e+01 \\
    %\rule{0pt}{2ex}
    %WRN+N+C-(CH3OH) & 4.6e+05 & 25 & 50 & 2.2e-18 & 1.00e+08 & 2.88e+01\\
    %\rule{0pt}{4ex}
    %[HCO$^+$/CO],[N$_2$H$^+$/CO](Ratio)$_{(WR)}$ & 4.6e+04 & 15 & 20 & 1.0e-19 & 4.79e+05 & 6.85e-02 \\
    %\rule{0pt}{2ex}
    %Ratio(WR18) & 1.0e+05 & 15 & 100 & 1.0e-19 & 2.45e+05 & 5.57e-03\\
    %\rule{0pt}{2ex}
    %Ratio(WRN) & 1.0e+05 & 15 & 100 & 4.6e-19 & 2.19e+05 & 2.77e-02 \\
    %\rule{0pt}{2ex}
    %Ratio(WRN18) & 4.6e+05 & 15 & 100 & 2.2e-19 & 6.46e+04 & 8.27e-04\\
    %\rule{0pt}{4ex}
    %[HCO$^+$],[N$_2$H$^+$](ions)(WR) & 4.6e+05 & 15 & 20 & 1.0e-17 & 5.50e+04 & 2.32e-03 \\
    %\rule{0pt}{2ex}
    %ions(WR18) & 4.6e+05 & 25 & 20 & 4.6e-17 & 5.89e+06 & 1.30e-03 \\
    %\rule{0pt}{2ex}
    %ions(WR18)+HNCO,HNC,HCN & 1.0e+06 & 15 & 50 & 1.0e-17 & 3.31e+04 & 2.18e+01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO,CH$_3$OH & 1.0e+05 & 15 & 50 & 1.0e-13 & 1.12e+04 & 1.92e+01\\
    
    %\rule{0pt}{2ex}
    %ions(WR18) + H$_2$CO & 1.0e+06 & 20 & 100 & 2.2e-18 & 4.68e+07 & 7.79e-01\\
    %\rule{0pt}{2ex}
    %ions(WR18) + N-group + H$_2$CO & 2.2e+04 & 20 & 100 & 2.2e-18 & 2.40e+06 & 2.84e+01\\
    %\rule{0pt}{5ex}
    %\hline
    %Weighted, ultra restricted (WUR) & 4.6e+04 & 15 & 100 & 1.0e-18 & 3.47e+05 & 6.39e-01\\
    %(2.2e4-1.0e5[cm-3])\\
    %(20,50[mag], 10,15[K]) \\
    %\rule{0pt}{2ex}
    %WURN & 4.6e+04 & 15 & 100 & 1.0e-18 & 3.63e+05 & 2.79e-01\\
    %\rule{0pt}{2ex}
    %WUR18 & 4.6e+04 & 15 & 100 & 2.2e-18 & 2.88e+05 & 1.26e-01\\
    %\rule{0pt}{2ex}
    %WURN18 & 4.6e+04 & 15 & 100 & 1.0e-18 & 3.72e+05 & 5.29e-01\\%15-25, 10-15K
    %\rule{0pt}{2ex}
    %WURN18(higher $\sigma$) & 4.6e+04 & 15 & 50 & 4.6e-19 & 4.37e+05 & 3.49e-01\\
    %\rule{0pt}{4ex}
    %WURN18 + HNCO,HNC,HCN & 1.0e+05 & 10 & 50 & 4.6e-18 & 3.02e+05 & 2.72e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + CH$_3$OH,H$_2$CO & 4.6e+04 & 15 & 100 & 4.6e-14 & 2.45+04 & 2.21e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + H$_2$CO & 1.0e+05 & 15 & 50 & 1.0e-13 & 1.17+04 & 1.06e+01\\
    %\rule{0pt}{2ex}
    %WURN18 + N-group + H$_2$CO & 4.6e+04 & 15 & 100 & 2.2e-19 & 9.55+05 & 3.92e+01\\
    %\rule{0pt}{4ex}
    %Ratio (WURN18) & 1.0e+05 & 15 & 100 & 1.0e-19 & 2.63+05 & 6.73e-03\\
    %\rule{0pt}{2ex}
    %ions (WURN18) & 2.2e+05 & 15 & 50 & 4.6e-17 & 2.57+06 & 2.97e-02\\
    %\rule{0pt}{2ex}
    %CO + HCO$^+$ (WURN18) & 2.2e+05 & 15 & 100 & 2.2e-18 & 7.41+04 & 1.19e-05\\
    %\rule{0pt}{2ex}
    %CO + N$_2$H$^+$ (WURN) & 4.6e+04 & 15 & 100 & 1.0e-18 & 3.63+05 & 4.09e-03\\
    %\hline
    Restricted & 4.6e+04 & 15 & 5 & 1.0e-18 & 3.63e+05 & 4.63e-02\\
    (CO,HCO$^+$(O18),N$_2$H$^+$)(Narrow)\\
    (1.0e4-1.0e6[cm$^{-3}$] \\
    (5-100[mag], 5-50[K]) \\
     \rule{0pt}{2ex}
    Ratio (R) & 1.0e+04 & 15 & 5 & 1.0e-19 & 2.24e+06 & 1.52e-03\\
    ions (R) & 4.6e+05 & 5 & 20 & 1.0e-13 & 3.89e+04 & 5.75e-04\\
    CO+ HCO$^+$ & 1.0e+04 & 20 & 20 & 2.2e-14 & 5.01e+03 & 1.49e-04\\
    CO+ N$_2$H$^+$ & 4.6e+05 & 10 & 20 & 2.2e-16 & 4.37e+04 & 1.01e-03\\
    \rule{0pt}{5ex}
    R+ CH$_3$OH,H$_2$CO & 1.0e+05 & 25 & 5 & 2.2e-19 & 3.72e+07 & 1.00e+01\\
    R+ H$_2$CO & 1.0e+04 & 20 & 5 & 1.0e-19 & 2.14e+07 & 1.31e-01\\
    R+ HNCO,HNC,HCN & 1.0e+06 & 10 & 100 & 1.0e-15 & 1.17e+04 & 1.36e+01\\
    R+ N-group + C-group & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 2.19e+01\\
    R+ N-group + H$_2$CO & 1.0e+06 & 30 & 50 & 4.6e-18 & 1.00e+08 & 1.79e+01\\
    \hline
    \end{tabular}
    \vspace*{2mm}
    \caption{The best models found with different solutions at p9. The restricted fitting have been performed through the models with Hnuc in the range of 1.0e4-1.0e6 cm-3, temperature in the range of 5-50 K and and visual extinction in the range of 5-100 mag.}
    \label{tab:p9_different_fittings}
\end{table*}

==> chapters/tables/table1.tex <==

%\begin{landscape}
\begin{table*}[ht]
\caption{Selected IRDC positions and their physical properties. The $\Sigma$ values and derived quantities in the first line for each position are based on the sub-mm dust continuum emission observed by {\it Herschel} \citep{lim2016distribution}, while values in the second line for each position are derived from the MIREX map \citep{2013A&A...549A..53K}.}
    \centering
    \addtolength{\leftskip} {-1cm} % increase (absolute) value if needed
    \addtolength{\rightskip}{-1cm}
    \begin{tabular}{p{0.01\linewidth}p{0.11\linewidth}p{0.11\linewidth}p{0.07\linewidth}p{0.10\linewidth}p{0.08\linewidth}p{0.04\linewidth}p{0.04\linewidth}p{0.04\linewidth}}\hline\hline
     & R.A. & Dec. & $\Sigma$ & $N_{\rm H}$ & $n_{\rm H}$ & $A_{V,{\rm tot}}$ & $\bar{A}_V$ & $T$\\
     &(J2000) & (J2000) & [$\rm g\:cm^{-2}$] & [$10^{23}\:\rm cm^{-2}$] & [$10^4\:\rm cm^{-3}$] & [mag] & [mag] & [K]\\
    \hline
    P1 & 18:42:46.687 & -4:04:08.830 & 0.394 & 1.68 & 10.50 & 88.4 & 22.1 & 11.8\\
    & & & 0.270 & 1.15 & 7.19 & 60.7 & 15.2 & \\
    \hline
    P2 & 18:42:50.709 & -4:03:14.763 & 0.438 & 1.87 & 11.70 & 98.4 & 24.6 & 13.1\\
     & & & 0.296 & 1.26 & 7.88 & 66.6 & 16.6\\
    \hline
    P3 & 18:42:49.490 & -4:02:21.514 & 0.330 & 1.41 & 8.84 & 74.2 & 18.6 & 13.5\\
     & & & 0.265 & 1.13 & 7.06 & 59.6 & 14.9 \\
    \hline
    P4 & 18:42:52.583 & -4:02:44.647 & 0.322 & 1.38 & 8.65 & 72.6 & 18.2 & 13.4\\
     & & & 0.267 & 1.14 & 7.12 & 60.1 & 15.0\\
    \hline
    P5 & 18:42:53.970 & -4:02:31.320 & 0.336 & 1.44 & 9.02 & 75.8 & 19.0 & 13.8\\
     & & & 0.259 & 1.11 & 6.94 & 58.3 & 14.6\\
    \hline
    P6 & 18:43:00.610 & -4:01:32.639 & 0.130 & 0.56 & 3.48 & 29.2 & 7.3 & 14.1\\
     & & & 0.187 & 0.80 & 4.99 & 42.1 & 10.5\\
    \hline
    P7 & 18:42:54.636 & -4:00:52.451 & 0.239 & 1.02 & 6.39 & 53.7 & 13.4 & 14.9\\
     & & & 0.193 & 0.83 & 5.16 & 43.4 & 10.9\\
    \hline
    P8 & 18:42:55.289 & -4:01:21.835 & 0.270 & 1.15 & 7.21 & 60.5 & 15.1 & 13.6\\
     & & & 0.195 & 0.83 & 5.21 & 43.9 & 11.0\\
    \hline
    P9 & 18:42:50.591 & -4:02:47.469 & 0.315 & 1.35 & 8.46 & 71.1 & 17.8 & 13.3\\
     & & & 0.164 & 0.70 & 4.38 & 36.9 & 9.2\\
    \hline
    P10 & 18:42:47.860 & -4:03:08.458 & 0.171 & 0.73 & 4.58 & 38.5 & 9.6 & 13.6\\
     & & & 0.116 & 0.50 & 3.11 & 26.1 & 6.5\\
    \hline
    \end{tabular}
    \label{tab:physical_parameters_IRDC}
\end{table*}
%\end{landscape}


==> chapters/tables/table2.tex <==


%\begingroup
%\begin{landscape}
\setlength{\tabcolsep}{7pt} % horizontal space
\renewcommand{\arraystretch}{1.4} % vertical space

\begin{table*}[t]\centering
\caption{Observed molecular species, rest frequencies, rotational quantum numbers of the transitions, rotational constants, rotational partition function, Einstein $A$ coefficients, energy of lower state, degeneracy of upper state, velocity resolution, $B_{\rm eff}$ and HPBWs.}
  \begin{tabular}{c c c c c c c c c c c}
  \hline
  \hline
  molecule & $\nu$ (GHz) & $J$ & $B$~(Hz) & $Q_{\rm rot}$($T_{\rm ex}$=7.5K) & $A$~(s$^{-1}$) & $E_{L}$~(K) & $g_{u}$ & $dv$~(km s$^{-1}$) & $B_{\rm eff}$ & $\theta(\arcsec)$ \\
  \hline
   HC$^{18}$O$^+$ & 85.1621570 & 1-0 & 4.26e10 & 3.90  & 3.6450E-05 & 0.00 & 3 &  0.6876 & 0.81 & 28.89\\
    \hline
    H$^{13}$CO$^+$ & 86.7542884 & 1-0 & 4.34e10 & 3.83 & 3.8539E-05 & 0.00 & 3 &  0.6749 & 0.81 & 28.36 \\
    \hline
    %SiO & 86846.96 & Q($T_{ex}$) = 1.010600$\times T^{0.990020}$ & 2.9275E-05 & 2.08 & 5 & 0.6742 & 83.39\\
    %\hline
     HN$^{13}$C & 87.0908500 & 1-0 & 4.35e10 &  3.82 & 2.3840E-05 & 0.00 & 3 & 0.6723 & 0.81 & 28.25\\
    \hline
     %CCH & 87316.925 & Q($T_{ex}$) = 2.106200$\times T^{0.981580}$ & 1.5314E-06 & 0.00216 & 3 & 0.6706 & 83.30\\
    %\hline
    HNCO & 87.9250443 & 4-3 & 1.11e10 & 36.90 & 8.7801E-06 & 6.33 & 9 & 0.6659 & 0.81 & 27.98\\
    \hline
    HCN & 88.6304160 & 1-0 & 4.43e10 & 3.88 & 8.0884E-06 & 0.00 & 3 & 0.6606 & 0.81 & 27.76\\
    \hline
    N$_2$H$^+$ & 93.1761300 & 1-0 & 4.66e10 & 3.71 & 3.6300E-05 & 0.00 & 3 & 0.0628 & 0.80 & 26.40\\
    \hline
    C$^{18}$O & 109.7821734 & 1-0 & 5.49e10 & 3.11& 6.2661E-08 & 0.00 & 3 & 0.0533 & 0.78 & 22.41\\
    \hline
     %DCO+ & 144077.2144 & Q($T_{ex}$) = 1.842760$\times T^{0.991545}$ & 2.1184E-04 & 3.46 & 5 & 0.4064 & 72.82 \\
    %\hline
     CH$_3$OH & 145.1031850 & 3-2 & 2.47e10 & 13.25 & 1.2323E-05 & 6.96 & 7 & 0.4035 & 0.73 & 16.95\\
    \hline
    H$_2$CO & 145.6029490 & 2-1 & 3.88e10 & 10.52 & 7.8127E-05 & 3.49 & 5 & 0.4021 & 0.73 & 16.90\\
    \hline
    %\dots & \dots
  \end{tabular}
  \vspace*{1mm}
  
  \label{tab:modelcules_parameters_Ntot}
\end{table*}
%\end{landscape}


































































==> chapters/tables/table2_landscape.tex <==
%\newpage
\afterpage{
\begin{landscape}
After this point, everthing is displayed in landscape format.\\
\ \\
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Year & 2000 & 2001 & 2002 & 2003 & 2004 & 2005 & 2006 & 2007 & 2008 & 2009 & 2010 \\
\hline 
GPD in billions & 235  &  225 bn & 223 bn & 323 & 423  & 523 & 624 & 725 & 826  & 924  & 1022  \\
\hline 
\end{tabular}
\end{landscape}
}

==> chapters/tables/table3_positions_abundances.tex <==
%\begin{landscape}
%\centering
%\begin{table*}[ht]
 %   \centering
  %  \addtolength{\leftskip} {-1cm}
   % \addtolength{\rightskip}{-1cm}
    %\begin{tabular}{p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
    %\hline
    %\hline
    %\begingroup
\setlength{\tabcolsep}{4pt} % horizontal space
\renewcommand{\arraystretch}{1.5} % vertical space

\begin{table*}[htpb!]\centering
 \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{c c c c c c c c c c c}
  \hline
  \hline
          Molecule & p1 & p2 & p3 & p4 & p5 & p6 & p7 & p8 & p9 & p10\\
         \hline
         \rule{0pt}{2ex}
         C$^{18}$O & $4.77\pm$1.47 & $4.31\pm$1.33 & $4.86\pm$1.50 & $5.19\pm$1.60 & $5.58\pm$1.72 & $11.00\pm$3.40 & $6.68\pm$2.06 & $5.79\pm$1.79 & $5.13\pm$1.58 & $6.43\pm$1.98\\
         (E-08)\\ 
         \rule{0pt}{2ex}
         CO & $1.52\pm$0.56 & $1.37\pm$0.51 & $1.54\pm$0.57 & $1.65\pm$0.61 & $1.77\pm$0.65 & $3.51\pm$1.29 & $2.12\pm$0.78 & $1.84\pm$0.68 & $1.63\pm$0.60 & $2.05\pm$0.75\\
         (E-05)\\ 
         %\rule{0pt}{2ex}
         %fD & 7.14 & 6.80 & 6.70 & 5.96 & 6.11 &  2.75 & 4.86 & 5.65 & 5.71 & 4.36 \\
         % & 9.34 & 10.29 & 9.21 & 8.59 & 7.95 & 4.03 & 6.64 & 7.65 & 8.70 & 6.97 \\
         \hline
         \rule{0pt}{2ex}
         H$^{13}$CO$^{+}$ & $1.02\pm$0.31 & $1.11\pm$0.34 & $0.87\pm$0.27 & $0.97\pm$0.30 & $1.02\pm$0.32 & $1.52\pm$0.48 & $0.84\pm$0.26 & $0.69\pm$0.22 & $0.96\pm$0.30 & $1.36\pm$0.42\\
         (E-11)\\
         HCO$^{+}$ & $4.11\pm$1.51 & $4.48\pm$1.64 & $3.49\pm$1.28 & $3.89\pm$1.43 & $4.10\pm$1.52 & $6.11\pm$2.27 & $3.37\pm$1.25 & $2.77\pm$1.04 & $3.84\pm$1.41 & $5.45\pm$2.01\\
         (E-10)\\
         \hline
         \rule{0pt}{2ex}
         HC$^{18}$O$^{+}$ & $1.96\pm$0.69 & $1.84\pm$0.67 &
         $1.88\pm$0.74 & $1.64\pm$0.65 & $2.19\pm$0.78 & &  &  &  & $1.40\pm$0.36\\
         (E-12)\\
         HCO$^{+}$ & $6.23\pm$2.54 & $5.84\pm$2.43 & $5.96\pm$2.64 & $5.23\pm$2.31 & $6.98\pm$2.86 & & & & & $4.45\pm$1.45 \\
         (E-10)\\
         \hline
         \rule{0pt}{2ex}
         N$_2$H$^{+}$ & $0.55\pm$0.17 & $1.79\pm$0.56 & $1.53\pm$0.47 & $1.52\pm$0.47 & $1.10\pm$0.34 & $2.62\pm$0.81 & $0.91\pm$0.28 & $0.80\pm$0.25 & $1.14\pm$0.35 & $1.47\pm$0.46\\
         (E-10) \\
         \hline
         \rule{0pt}{2ex}
         HNCO & $2.17\pm$0.74 & $4.29\pm$1.45 & $4.15\pm$1.41 & $3.45\pm$1.18 & $2.74\pm$0.94 & $1.91\pm$0.72 & $1.78\pm$0.64 & $1.40\pm$0.51 & $3.47\pm$1.18 & $4.32\pm$1.49\\
         (E-10) \\
         \hline
         \rule{0pt}{2ex}
         HN$^{13}$C & $1.41\pm$0.43 & $1.61\pm$0.50 & $1.85\pm$0.57 & $1.64\pm$0.51 & $1.24\pm$0.39 & $2.85\pm$0.89 & $0.94\pm$0.30 & $0.91\pm$0.29 & $1.41\pm$0.44 & $1.88\pm$0.59\\
         (E-11) \\
         HNC & $5.65\pm$2.08 & $6.47\pm$2.37 & $7.43\pm$2.73 & $6.59\pm$2.43 & $4.97\pm$1.84 & $11.40\pm$4.24 & $3.79\pm$1.43 & $3.67\pm$1.38 & $5.66\pm$2.09 & $7.54\pm$2.80 \\
         (E-10) \\
         \hline
         \rule{0pt}{2ex}
         HCN & $11.10\pm$3.44 & $10.30\pm$3.22 & $5.86\pm$1.88 & $8.16\pm$2.57 & $8.53\pm$2.69 & $26.60\pm$8.29 & $10.10\pm$3.28 & $10.50\pm$3.33 & $7.66\pm$2.40 & $10.00\pm$3.32\\
         (E-11) \\
         \hline
         \rule{0pt}{2ex}
         CH$_3$OH & $0.52\pm$0.18 & $1.73\pm$0.60 & $1.74\pm$0.61 & $1.33\pm$0.46 & $1.26\pm$0.44 & $0.49\pm$0.18 & $0.45\pm$0.16 & $0.33\pm$0.12 & $1.54\pm$0.54 & $1.93\pm$0.67\\
          (E-09) \\
          \hline
          \rule{0pt}{2ex}
          H$_2$CO & $3.89\pm$1.26 & $10.40\pm$3.33 & $7.33\pm$2.37 & $7.66\pm$2.47 & $6.98\pm$2.25 & $3.31\pm$1.19 & $2.76\pm$0.94 & $2.19\pm$0.73 & $9.16\pm$2.95 & $9.94\pm$3.21\\
         (E-11)\\
         \hline
         %\hline
         %\hline
         %\\
         
         %HC3N & $2.15\pm$0.67 & $7.31\pm$2.20 & $8.30\pm$2.50 & $5.15\pm$1.59 & $4.25\pm$1.32 & $1.46\pm$0.53 & $1.38\pm$0.53 & $1.10\pm$0.39 & $5.44\pm$1.66 & $5.77\pm$1.79\\
         %(E-10) \\
         %\hline
         %CCS & & $5.17\pm$1.75 & $5.41\pm$1.88 & $5.94\pm$2.25 & $4.88\pm$1.78 & $7.55\pm$3.20 & & &  $7.44\pm$2.52 &  \\
         %(E-11) \\
         %\hline
         %OCS & $1.70\pm$0.66 & $8.98\pm$2.80 & $8.94\pm$2.82 & $5.47\pm$1.79 & $6.27\pm$2.04 & $5.35\pm$1.96 & & & $6.81\pm$2.19 & $11.60\pm$3.68\\
         %(E-10) \\
         %\hline
        % SO & & $2.59\pm$0.85 & & & $1.88\pm$0.72 & & & & $1.57\pm$0.63 & \\
         %(E-10) \\
        % \hline
         %SiO & $1.39\pm$0.43 & $5.92\pm$1.78 & $7.35\pm$2.21 & $5.14\pm$1.55 & $4.43\pm$1.34 & & & $0.35\pm$0.14 & $5.64\pm$1.70 & $6.19\pm$1.87\\
         %(E-11)\\
         %\hline
         %c-C3H2 & $2.11\pm$0.64 & $2.17\pm$0.65 & $2.61\pm$0.79 & $2.07\pm$0.63 & $2.18\pm$0.66 & $3.06\pm$0.94 & $1.31\pm$0.41 & $1.53\pm$0.48 & $2.13\pm$0.64 & $3.29\pm$1.01\\
         %(E-10)\\
        % \hline
         %CH3C2H & $2.65\pm$0.86 & $3.39\pm$1.05 & $3.37\pm$1.10 & $2.84\pm$0.91 & $2.05\pm$0.73 & & $3.07\pm$1.11 & $3.10\pm$1.06 & $3.05\pm$1.00 & \\
         %(E-10) \\
         %\hline
         %CCH & $0.71\pm$0.22 & $1.11\pm$0.33 & $1.02\pm$0.31 & $7.45\pm$2.29 & $0.62\pm$0.19 & $0.65\pm$0.21 & $0.37\pm$0.12 & $0.34\pm$0.11 & $0.94\pm$0.29 & $1.02\pm$0.32\\
         %(E-09)\\
         %\hline
         %CS & $0.89\pm$0.27 & $2.46\pm$0.74 & $1.69\pm$0.51 & $1.83\pm$0.55 & $1.55\pm$0.47 & $1.51\pm$0.46 & $0.69\pm$0.21 & $0.56\pm$0.17 & $2.27\pm$0.68 & $3.35\pm$1.01\\
         %(E-10) \\
         %\hline
         %DCO+ & $7.43\pm$2.40 & $5.05\pm$1.65 & $6.06\pm$2.07 & $7.36\pm$2.32 & $6.23\pm$2.08 & $16.80\pm$5.63 & & $5.45\pm$1.99 & $3.64\pm$1.24 & $8.57\pm$2.92\\
         %(E-12) \\
         %\hline
    %\end{tabular}
     %\vspace*{2mm}
    %\caption{Calculated abundances of molecules observed by IRAM 30m telescope at 10 different positions. Abundances of C18O and CO, have obtained for broad (first row) and narrow range (second row) of velocities.}
    %\label{tab:abundances}
%\end{table*}
  \hline
  \end{tabular}
  \end{adjustbox}
  \vspace*{1mm}
  \caption{Estimated molecular abundances observed by IRAM 30m telescope towards IRDC G28.37+00.07, at 10 different positions within narrow velocity range (77-82 km.s$^{-1}$).}
  \label{tab:abundances}
  
\end{table*}
%\end{landscape}
